Proceedings of the Sixth International Workshop on Multiple Partonic Interactions at the Large Hadron Collider

Multiple Partonic Interactions are often crucial for interpreting results obtained at the Large Hadron Collider (LHC). The quest for a sound understanding of the dynamics behind MPI - particularly at this time when the LHC is due to start its "Run II" operations - has focused the aim of this workshop. MPI@LHC2014 concentrated mainly on the phenomenology of LHC measurements whilst keeping in perspective those results obtained at previous hadron colliders. The workshop has also debated some of the state-of-the-art theoretical considerations and the modeling of MPI in Monte Carlo event generators. The topics debated in the workshop included: Phenomenology of MPI processes and multiparton distributions; Considerations for the description of MPI in Quantum Chromodynamics (QCD); Measuring multiple partonic interactions; Experimental results on inelastic hadronic collisions: underlying event, minimum bias, forward energy flow; Monte Carlo generator development and tuning; Connections with low-x phenomena, diffraction, heavy-ion physics and cosmic rays. In a total of 57 plenary talks the workshop covered a wide range of experimental results, Monte Carlo development and tuning, phenomenology and dedicated measurements of MPI which were produced with data from the LHC's Run I. Recent progress of theoretical understanding of MPI in pp, pA and AA collisions as well as the role of MPI in diffraction and small-x physics were also covered. The workshop forstered close contact between the experimental and theoretical communities. It provided a setting to discuss many of the different aspects of MPI, eventually identifying them as a unifying concept between apparently different lines of research and evaluating their impact on the LHC physics programme.

==> DPS/Baranov/content1b.tex <==
\title{Correlations in $J/\psi$ pair production as SPS versus DPS discriminators}

\author{Sergey Baranov}
\affiliation{P.N.Lebedev Institute of Physics\\Russian Academy of Sciences}
%\author{A.M.Snigirev and  N.P. Zotov}
%\affiliation{Institute of Nuclear Physics\\Moscow State University}
%\author{W. Sch\"{a}fer and A. Szczurek}
%\affiliation{Institute of Nuclear Physics\\Polish Academy of Sciences}

\maketitle

\def\J {$J/\psi$ }
\def\j {J/\psi }
\def\O  {{\cal O}}
\def\qe {quasielastic}
\def\pd {pseudo-diffractive}
\def\ktf {$k_t$-factorization }
\def\ktfa {$k_t$-factorization approach }
\def\plb#1#2#3  {{Phys.\ Lett.\ B }          {\bf#1}, #2 (#3)}
\def\prd#1#2#3  {{Phys.\ Rev.\ D }           {\bf#1}, #2 (#3)}
\def\prl#1#2#3  {{Phys.\ Rev.\ Lett.\ }      {\bf#1}, #2 (#3)}
\section{Motivation and theoretical framework}

We focus on the problem of disentangling the single (SPS) and double (DPS) 
parton scattering modes in the production of \J pairs at the LHC conditions.
We carefully examine the production properties in the different kinematical 
domains paying attention to the different contributing processes and compare 
the shapes of the differential cross sections. 

%\section{Theoretical framework}

Our approach is based on perturbative QCD, 
nonrelativistic bound state formalism, and the \ktf ansatz in the parton model.
On the SPS side, 
we consider the leading-order  ${\cal O}(\alpha_s^4)$ contribution (31 box
diagrams calculated in \cite{B})
and the subleading ${\cal O}(\alpha_s^6)$ contribution from \pd ~gluon-gluon 
scattering represented by one gluon exchange and two gluon exchange mechanisms.
The latter can mimic the DPS mechanism having similar kinematics.
On the DPS side, we consider the prompt \J production including the direct 
$g+g\to\j+g$ contribution and radiative $\chi_c$ decays.
All necessary details of calculations can be found in \cite{BSSSZ}. 
%and references therein.

\section{Results and conclusions}

Naive expectations that the SPS mechanism should result in back-to-back event 
configuration received no support from calculations. Including the initial state 
radiation effects (either in the form of $k_t$-dependent gluon densities \cite{B} 
or by means of simulating parton showers in a phenomenological way \cite{Stirling}) 
washes out the azimuthal correlations, thus making the SPS and DPS samples very 
similar to each other. The correlations get restored at higher $p_t$, but then 
the production rates fall dramatically, and so, the practical discrimination 
of the production mechanisms remains problematic.

Selecting the events with large rapidity difference between \J mesons looks more 
promising. As it was expected, the DPS production leads to broad and relatively 
flat distribution in $\Delta y$. The leading order SPS contribution is localized 
inside the interval $|\Delta{y}|\le 2$ (and continues to fall down steeply with 
increasing $|\Delta{y}|$), while the higher order \pd ~contributions extending 
beyond these limits are heavily suppressed by the color algebra (see \cite{BSSSZ}
for details) and do not constitute significant background for the DPS production.

%\begin{figure}\label{deltay}
\hspace*{-1cm}
\includegraphics[width=8.5cm, height=4.5cm]{jj_dy.eps}
%\end{figure}
\parbox{7.0cm}%
{\vspace*{-4.5cm}
Distributions over the rapidity difference between $J/\psi$ mesons.
Dotted curve, SPS 'box' contribution;
dashed curve, one-gluon exchange contribution multiplied by 1000;
solid curve, two-gluon exchange contribution multiplied by 25;
dash-dotted curve, DPS production.}\\[-1cm]

\begin{thebibliography}{9}
\bibitem{B} S.P. Baranov, \prd{84}{054012}{2011} .
\bibitem{Stirling} C.-H. Kom, A. Kulesza, and W.J. Stirling,
        \prl{107}{082002}{2011} .
%\bibitem{BSZ} S.P. Baranov, A.M. Snigirev, and N.P. Zotov,
%        \plb{705}{116}{2011} .
\bibitem{BSSSZ} S.P. Baranov, A.M. Snigirev, A. Szczurek, 
        W. Sch\"{a}fer, N.P. Zotov, \prd{87}{034035}{2013} .
\end{thebibliography}


==> DPS/Baranov/content2.tex <==
\title{Kinematic corrections to Quarkonium production in NRQCD approach}

\author{Sergey Baranov}
\affiliation{P.N.Lebedev Institute of Physics\\Russian Academy of Sciences}

\maketitle

\def\cc {$c\bar{c}$~}
\def\cj {$\chi_{cJ}$~}
\def\bb {$b\bar{b}$~}
\def\qq {$Q\bar{Q}$~}
%\def\m  {$m_{Octet}$~}
\def\m  {$m_{[8]}$~}
\def\J {$J/\psi$ }   
\def\Js {$J/\psi$'s~}
\def\j { J/\psi  }
\def\pjt {$p_{\psi,T}$~}
\def\ktf {$k_t$-factorization }
\def\ktfa {$k_t$-factorization approach }
\def\dum#1#2#3  {{~}                         {\bf#1}, #2 (#3)}
\def\plb#1#2#3  {{Phys.\ Lett.\ B }          {\bf#1}, #2 (#3)}
\def\prd#1#2#3  {{Phys.\ Rev.\ D }           {\bf#1}, #2 (#3)}
\def\prl#1#2#3  {{Phys.\ Rev.\ Lett.\ }      {\bf#1}, #2 (#3)}
\section{Introduction and motivation}

Quarkonium production in high energy hadrinic collisions is usually expressed 
in terms of non-relativistic QCD (NRQCD) factorization approach \cite{NRQCD}.
In its mathematical aspects, this approach is similar to the classical theory 
of multipole radiation;
in practice, numerical calculations are always accompanied by an exordium that
a \qq pair produced in hard subprocess as color-octet emits 
(a number of) soft gluons changing the quantum numbers of the \qq system without 
changing its energy-momentum. This is in obvious contradiction with confinement 
which prohibits the emission of soft colored quanta. 
Our note represents an attempt to estimate the numerical effect of final state 
radiation on the experimental observables if to replace an 'infinitely soft' 
gluon with a 'real' quantum of nonzero (of order $\Lambda_{QCD}$)
energy-momentum.

\section{Results and conclusions}

The simulation is organized as follows. First, we generate the production 
of a color-octet \cc state in a usual perturbative way, but with a mass \m 
slightly higher than the nominal \J mass in order to preserve some phase space 
for the subsequent decay. As an example we tried \m = 3.4 and 3.7 GeV. After 
that we generate a two-body decay $c\bar{c}[8]\to J/\psi + X$. We do not specify 
the nature of the state $X$, since the only property of importance is its mass 
$m_X$. For illustration we tried $m_X$=0, 150, 300, and 500 MeV.

The $p_t$ of the resulting \J is smaller than that of the originall \cc pair, 
as part of the initial momentum is carried away by the quantum $X$. The visible 
kinematic effect (i.e., the ratio of the cross sections before and after emission
$d\sigma(c\bar{c}[8])/dp_t$ and $d\sigma(J/\psi)/dp_t$)
%and $d\sigma(c\bar{c}[8])/dp_t$)
turned out to be very similar for all intermediate octet states
($^1S_0^{[8]}$, $^3S_1^{[8]}$, $^3P_0^{[8]}$, $^3P_1^{[8]}$, $^3P_2^{[8]}$),
despite the individual spectra on their own may be rather different.
The effect is nearly insensitive to the mass of the emitted quantum $m_X$
and is only sensitive to the mass difference between \m and $m_\psi$. 
The kinematic correction is large and, therefore, cannot be neglected.
On the other hand, it flattens at high $p_t$, and so, can be effectively
included into redefined nonperturbative matrix elements.







%\begin{figure}
\hspace*{-1cm}
\includegraphics[width=8.cm, height=4.5cm]{m34.eps}
\includegraphics[width=8.cm, height=4.5cm]{m37.eps}\\
Kinematic correction factors for $p_t$ spectra due to final state radiation.
The mass of the emitted system $m_X$ is set to 0 (solid curves),
150 MeV (dashed), 300 MeV (dotted), and 500 MeV (dash-dotted).
The octet state mass is set to 3.4 GeV (left panel) and 3.7 GeV (right panel).
%\end{figure}

\begin{thebibliography}{9}
\bibitem{NRQCD} G. T. Bodwin, E. Braaten, and G. P. Lepage,
                       \prd{51}{1125}{1995} ; \dum{55}{5853(E)}{1997} .
\end{thebibliography}


==> DPS/Baranov/content_Baranov.tex <==
\title{Correlations in $J/\psi$ pair production as SPS versus DPS discriminators}

\author{Sergey Baranov}
\affiliation{P.N.Lebedev Institute of Physics\\Russian Academy of Sciences}
%\author{A.M.Snigirev and  N.P. Zotov}
%\affiliation{Institute of Nuclear Physics\\Moscow State University}
%\author{W. Sch\"{a}fer and A. Szczurek}
%\affiliation{Institute of Nuclear Physics\\Polish Academy of Sciences}

\maketitle

\def\J {$J/\psi$ }
\def\j {J/\psi }
\def\O  {{\cal O}}
\def\qe {quasielastic}
\def\pd {pseudo-diffractive}
\def\ktf {$k_t$-factorization }
\def\ktfa {$k_t$-factorization approach }
\def\plb#1#2#3  {{Phys.\ Lett.\ B }          {\bf#1}, #2 (#3)}
\def\prd#1#2#3  {{Phys.\ Rev.\ D }           {\bf#1}, #2 (#3)}
\def\prl#1#2#3  {{Phys.\ Rev.\ Lett.\ }      {\bf#1}, #2 (#3)}
\section*{Motivation and theoretical framework}

We focus on the problem of disentangling the single (SPS) and double (DPS) 
parton scattering modes in the production of \J pairs at the LHC conditions.
We carefully examine the production properties in the different kinematical 
domains paying attention to the different contributing processes and compare 
the shapes of the differential cross sections. 

%\section{Theoretical framework}

Our approach is based on perturbative QCD, 
nonrelativistic bound state formalism, and the \ktf ansatz in the parton model.
On the SPS side, 
we consider the leading-order  ${\cal O}(\alpha_s^4)$ contribution (31 box
diagrams calculated in \cite{B})
and the subleading ${\cal O}(\alpha_s^6)$ contribution from \pd ~gluon-gluon 
scattering represented by one gluon exchange and two gluon exchange mechanisms.
The latter can mimic the DPS mechanism having similar kinematics.
On the DPS side, we consider the prompt \J production including the direct 
$g+g\to\j+g$ contribution and radiative $\chi_c$ decays.
All necessary details of calculations can be found in \cite{BSSSZ}. 
%and references therein.

\section*{Results and conclusions}

Naive expectations that the SPS mechanism should result in back-to-back event 
configuration received no support from calculations. Including the initial state 
radiation effects (either in the form of $k_t$-dependent gluon densities \cite{B} 
or by means of simulating parton showers in a phenomenological way \cite{Stirling}) 
washes out the azimuthal correlations, thus making the SPS and DPS samples very 
similar to each other. The correlations get restored at higher $p_t$, but then 
the production rates fall dramatically, and so, the practical discrimination 
of the production mechanisms remains problematic.

Selecting the events with large rapidity difference between \J mesons looks more 
promising. As it was expected, the DPS production leads to broad and relatively 
flat distribution in $\Delta y$. The leading order SPS contribution is localized 
inside the interval $|\Delta{y}|\le 2$ (and continues to fall down steeply with 
increasing $|\Delta{y}|$), while the higher order \pd ~contributions extending 
beyond these limits are heavily suppressed by the color algebra (see \cite{BSSSZ}
for details) and do not constitute significant background for the DPS production.

%\begin{figure}\label{deltay}
\hspace*{-1cm}
\includegraphics[width=8.5cm, height=4.5cm]{DPS/Baranov/jj_dy.eps}
%\end{figure}
\parbox{7.0cm}%
{\vspace*{-4.5cm}
Distributions over the rapidity difference between $J/\psi$ mesons.
Dotted curve, SPS 'box' contribution;
dashed curve, one-gluon exchange contribution multiplied by 1000;
solid curve, two-gluon exchange contribution multiplied by 25;
dash-dotted curve, DPS production.}\\[-1cm]

\begin{thebibliography}{9}
\bibitem{B} S.P. Baranov, \prd{84}{054012}{2011} .
\bibitem{Stirling} C.-H. Kom, A. Kulesza, and W.J. Stirling,
        \prl{107}{082002}{2011} .
%\bibitem{BSZ} S.P. Baranov, A.M. Snigirev, and N.P. Zotov,
%        \plb{705}{116}{2011} .
\bibitem{BSSSZ} S.P. Baranov, A.M. Snigirev, A. Szczurek, 
        W. Sch\"{a}fer, N.P. Zotov, \prd{87}{034035}{2013} .
\end{thebibliography}


==> DPS/Baranov/content_Baranov2.tex <==
\title{Correlations in $J/\psi$ pair production as SPS versus DPS discriminators}

\author{S.P. Baranov$^1$, 
A.M. Snigirev$^2$, W. Sch\"{a}fer$^3$, A. Szczurek$^3$, N.P. Zotov$^2$}
\affiliation{$^1$P.N.Lebedev Institute of Physics, Russian Academy of Sciences\\
             $^2$Institute of Nuclear Physics, Moscow State University\\
             $^3$Institute of Nuclear Physics, Polish Academy of Sciences}
%\author{A.M.Snigirev and  N.P. Zotov}
%\affiliation{Institute of Nuclear Physics\\Moscow State University}
%\author{W. Sch\"{a}fer and A. Szczurek}
%\affiliation{Institute of Nuclear Physics\\Polish Academy of Sciences}

\maketitle

\def\J {$J/\psi$ }
\def\j {J/\psi }
\def\O  {{\cal O}}
\def\qe {quasielastic}
\def\pd {pseudo-diffractive}
\def\ktf {$k_t$-factorization }
\def\ktfa {$k_t$-factorization approach }
\def\plb#1#2#3  {{Phys.\ Lett.\ B }          {\bf#1}, #2 (#3)}
\def\prd#1#2#3  {{Phys.\ Rev.\ D }           {\bf#1}, #2 (#3)}
\def\prl#1#2#3  {{Phys.\ Rev.\ Lett.\ }      {\bf#1}, #2 (#3)}
\section{Motivation and theoretical framework}
\vspace*{-1mm}

We focus on the problem of disentangling the single (SPS) and double (DPS) 
parton scattering modes in the production of \J pairs at the LHC conditions.
We carefully examine the production properties in the different kinematical 
domains paying attention to the different contributing processes and compare 
the shapes of the differential cross sections. 

%\section{Theoretical framework}

Our approach is based on perturbative QCD, 
nonrelativistic bound state formalism, and the \ktf ansatz in the parton model.
On the SPS side, 
we consider the leading-order  ${\cal O}(\alpha_s^4)$ contribution (31 box
diagrams calculated in \cite{B})
and the subleading ${\cal O}(\alpha_s^6)$ contribution from \pd ~gluon-gluon 
scattering represented by one gluon exchange and two gluon exchange mechanisms.
The latter can mimic the DPS mechanism having similar kinematics.
On the DPS side, we consider the prompt \J production including
the direct $g+g\to\j+g$ contribution and radiative $\chi_c$ decays.
All necessary details of calculations can be found in \cite{BSSSZ}.\\[-6mm]
%and references therein.

\section{Results and conclusions}
\vspace*{-1mm}

Naive expectations that the SPS mechanism should result in back-to-back event 
configuration received no support from calculations. Including the initial state 
radiation effects (either in the form of $k_t$-dependent gluon densities \cite{B} 
or by means of simulating parton showers in a phenomenological way \cite{Stirling}) 
washes out the azimuthal correlations, thus making the SPS and DPS samples very 
similar to each other. The correlations get restored at higher $p_t$, but then 
the production rates fall dramatically, and so, the practical discrimination 
of the production mechanisms remains problematic.

Selecting the events with large rapidity difference between \J mesons looks more 
promising. As it was expected, the DPS production leads to broad and relatively 
flat distribution in $\Delta y$. The leading order SPS contribution is localized 
inside the interval $|\Delta{y}|\le 2$ (and continues to fall down steeply with 
increasing $|\Delta{y}|$), while the higher order \pd ~contributions extending 
beyond these limits are heavily suppressed by the color algebra (see \cite{BSSSZ}
for details) and do not constitute significant background for the DPS production.

%\begin{figure}\label{deltay}
\hspace*{-1cm}
\includegraphics[width=8.5cm, height=4.5cm]{DPS/Baranov/jj_dy.eps}
%\end{figure}
\parbox{7.0cm}%
{\vspace*{-4.5cm}
Distributions over the rapidity difference between $J/\psi$ mesons.
Dotted curve, SPS 'box' contribution;
dashed curve, one-gluon exchange contribution multiplied by 1000;
solid curve, two-gluon exchange contribution multiplied by 25;
dash-dotted curve, DPS production.}~\\[-13mm]

\begin{thebibliography}{9}
\bibitem{B} S.P. Baranov, \prd{84}{054012}{2011} .\\[-5mm]
\bibitem{Stirling} C.-H. Kom, A. Kulesza, and W.J. Stirling,
        \prl{107}{082002}{2011} .\\[-5mm]
%\bibitem{BSZ} S.P. Baranov, A.M. Snigirev, and N.P. Zotov,
%        \plb{705}{116}{2011} .
\bibitem{BSSSZ} S.P. Baranov, A.M. Snigirev, A. Szczurek, 
        W. Sch\"{a}fer, N.P. Zotov, \prd{87}{034035}{2013} .
\end{thebibliography}


==> DPS/Cecciopieri/content_Cecciopieri.tex <==
\title{On the longitudinal structure double parton distributions}
\author{Federico Alberto Ceccopieri}
\affiliation{IFPA, Universit\'e de Li\`ege, 4000 Li\`ege, Belgium}

\maketitle

\section*{Open problems}
At high energies, multiple parton scattering may occur within the same hadronic collision.
As long as the scattering processes are characterised by large momentum transfers we may 
try to generalise, as a first approximation, the concepts of hard scattering factorisation derived in the single particle scattering context. In the case of double parton scattering, under the simplifying assumptions of two uncorrelated hard scatterings, measurements have provided so far informations only on $\sigma_{eff}$, the dimensionful parameter which controls the overall relative magnitudo of the double parton scattering contribution, with no strong indications of its energy, hardness and flavour dependence. 
Among channels which have been proposed to study the multiple parton component of the scattering, we mention here the associated production of a particle and a electroweak boson, along the lines described in Ref.~\cite{LHCb_ZD}.
This processes, triggering on particles rather than on jets, can access the low but sill perturbative transverse momentum region of the particle production spectrum, which is expected to be populated by particles generated in additional partonic interactions. Moreover, the possibility to control initial state radiation by properly restricting the transverse momentum of the electroweak boson can give additional handle in the characterisation of the double or multiple parton scattering component.
On the theoretical side, double parton scattering gives access to parton correlations in the hadron structure not accessible in single parton scattering and encoded in novel distributions, double parton distributions.
The factorisation of the relevant cross sections is presently under scrutiny~\cite{DS,Gaunt}
and the relevant issue of the proper scale evolution of these distributions has been already pointed out. Its solution is mandatory if the whole double parton scattering formalism has to be properly validated in different processes at different energies. If the dependence on relative interparton distance is integrated over, one obtains longitudinal 
double parton distributions evolution equations~\cite{snigirev2003,Ceccopieri_DPD}. These distributions however do not appear directly into double parton scattering cross sections and their evolution is characterised by an additional term, responsable for perturbative longitudinal correlation between the interacting partons, which poses a problem of double counting with single parton scattering cross sections. Moreover, when viewed in position space, such term accumulates at zero transverse distance exhibiting a singular behaviour in this limit~\cite{DS}. 
In order to solve these problems, it is therefore necessary to introduce distributions unintegrated over relative transverse parton momenta, addressed as generalised parton distributions, $_{2}\mbox{GPD}s$,
which are directly connected to the value of $\sigma_{eff}^{-1}$~\cite{BDFS} without factorising assumptions.
On the other hand, the inhomogeneous term discussed above is essential to preserve the expected sum rules for longitudinal double parton 
distributions~\cite{Ceccopeiri_sumrules}.  It appears therefore that the road towards a consistent treatment of QCD evolution effects of (generalised) double parton distributions is quite narrow as it must reconcile all these requirements at once.

\section*{Outlook}
We have outlined measurements potentially sensitive to double partonic interactions and some theoretical aspects of the present multiple scattering theory which requires further improvements.

\begin{thebibliography}{9}
\bibitem{LHCb_ZD}R.~Aaij \textit{et al.} (LHCb Collaboration),  \textsl{JHEP} \textbf{1404} (2014) 091\,.
\bibitem{DS}M.~Diehl and A.~Schafer, \textsl{Phys.~Lett.~} \textbf{B698} (2011) 389\,.
\bibitem{Gaunt} J.~Gaunt, \textsl{JHEP} \textbf{1407} (2014) 110\,.
\bibitem{snigirev2003} A.~M.~Snigirev, \textsl{Phys.~Rev.~} \textbf{D68} (2003) 114012\,.
\bibitem{Ceccopieri_DPD} F.~A.~Ceccopieri, \textsl{Phys.~Lett.~} \textbf{B697} (2011) 482.
\bibitem{BDFS} B.~Blok \textit{et al.}, \textsl{Phys.~Rev.~} \textbf{D83} (2011) 071501\,, \textsl{Eur.~Phys.~J.~} \textbf{C72} (2012) 1963\,.
\bibitem{Ceccopeiri_sumrules}F.~A.~Ceccopieri, \textsl{Phys.~Lett.~} \textbf{B734} (2014) 79\,.
\end{thebibliography}




==> DPS/Ciangottini/content_Ciangottini.tex <==
\title{DPS measurements with CMS}
\author{Diego Ciangottini and Livio Fano}
\affiliation{Universit\'a degli Studi di Perugia/INFN, Italy}

\maketitle

\section*{Introduction}
The study of DPS processes is important because it provides valuable information on the transverse distribution of partons in the proton and on the multi-parton correlations in the hadronic wave function. DPS also constitutes a background to new physics searches at the LHC.%~\cite{DelFabbro:1999tf,Hussein:2006xr,Bandurin:2010gn}.

%\begin{figure}[htbp]
%\centering
%\includegraphics[width=0.40\textwidth]{figs/DPS_final.pdf}
 %\includegraphics[width=0.40\textwidth]{figs/SPS_final.pdf}
 %\caption{Feynman diagrams for W + 2-jet production from (left) double parton scattering and (right) single parton scattering.}
%\label{fig:feyn}
%\end{figure}

Various measurements in pp and $p-\bar{p}$ collisions at $\sqrt{s}=63~GeV$%~\cite{UA2}
, 630~GeV
%\cite{AFS}
, and 1.8~TeV
%~\cite{CDF1} 
are consistent with DPS contributions to multijet final states, as well as to $\gamma$ + 3-jet events at $\sqrt{s}=1.8~TeV$
%~\cite{CDF2} 
and 1.96~TeV.%~\cite{D0}.


The summary of DPS measurements at CMS is presented in the following sections.


\section*{DPS in W+2jets process}
The W + 2-jet process is attractive because the muonic decay of the W provides a clean tag and the large dijet production cross section increases the probability of observing DPS.
Events containing a W + 2-jet final state originating from single parton scattering (SPS) constitute an irreducible background.

Events are required to have exactly one muon with $p_T> 35$GeV/c, $|{\eta}| < 2.1$, and missing transverse energy $MET > 30$GeV.
The transverse mass is required to be greater than 50~GeV/$c^2$.
Selected events are required to have exactly two jets with $p_T> $ 20~GeV/c and $|{\eta}| < $ 2.0.
For DPS events, the W and the dijet system are independent of each other, while for SPS events they are highly correlated.
It is thus possible to define several observables that discriminate between DPS and SPS events.


\begin{itemize}
\item
the relative ${p_T}$-balance between the two jets, $\Delta^{rel}~{p_T}$, defined as:
$$
\Delta^{rel}~{p_T} = \frac{  |{\overrightarrow{p_T}({j_{1}}) + \overrightarrow{p_T}({j_{2}}) }| }{|{\overrightarrow{p_T}({j_{1}})}| + |{\overrightarrow{p_T}({j_{2}})}| }
$$

\item
The azimuthal angle between the W-boson and the dijet system, $\Delta S$, defined as:
%The $\DS$ is defined as:

$$
\Delta S = \arccos \left( \frac{\overrightarrow{p_T}(\mu, MET)\cdot\overrightarrow{p_T}(j_1, j_2)}{|{\overrightarrow{p_T}(\mu, MET)}|\cdot |{\overrightarrow{p_T}(j_1, j_2)}| }\right)
$$



\end{itemize}


The fraction of DPS in W + 2-jet events is extracted with the DPS + SPS  template fit to the distribution of the $\Delta ^{rel}~{p_T}$ and $\Delta S$ observables.

The effective cross section, characterizing the effective transverse area of hard partonic interactions in collisions between protons, is calculated to be:

\begin{equation}
\sigma_{eff} = 20.7 \pm 0.8^{stat} \pm  6.6^{syst} mb.
\end{equation}

The measured value of the effective cross section is consistent with the Tevatron and ATLAS results.


\section*{DPS in 4 jets process}
 Scenario with four jets at different transverse momentum ($p_T$) thresholds in the final state has been measured at the CMS detector\cite{ref:4jet}. In particular, the two hardest jets are required to have $p_T$ greater than 50 GeV and they form the "hard-jet pair", while a $p_T$ threshold of 20 GeV is set for the two additional jets, comprising the "soft-jet pair". Additional jets with $p_T > $20 GeV are
vetoed. All the jets are selected in the pseudorapidity region $|\eta|<$4.7.
Single jet $p_T$ and spectra are measured and data are compared to different Monte Carlo predictions, which use a different matrix element in the perturbative QCD framework.

The $p_T$ spectrum of the hard jets is well reproduced by all the compared models at high $p_T$, while at low $p_T$, where a contribution coming from MPI is expected, the predictions start to exhibit greater differences. 

The predictions including MPI need to be validated with underlying event measurements before a
direct extraction of the DPS contribution can be performed via template fit. However, an alternative way to extrapolate $\sigma_{eff}$ using a MC tuning procedure has been investigated and it produces coherent results \cite{ref:4jet2}.


\section*{DPS in double $J/\psi$ production}
The measurement of the cross section for prompt double $J/\psi$ production in pp interactions at $\sqrt{s}=7\mathrm{TeV}$ has been performed independently from production
models \cite{ref:jpsi}.

A signal yield of 446$\pm$23 events for the production of two prompt $J/\psi$ mesons originating from a common vertex has been observed in a sample corresponding to an integrated luminosity of 4.73~$\mathrm{fb}^{-1}$. 
The differential cross section in bins of $|\Delta y|$ is sensitive to DPS contribution. The data show
evidence for excess at $|\Delta y|>$2.6, a region that current models suggest to be exclusively populated by DPS production. 

\begin{thebibliography}{9}
\bibitem{ref:w2jets}{The CMS Collaboration}, 
				{10.1007/JHEP03(2014)032},
            			{Study of double parton scattering using W + 2-jet events in proton-proton collisions at $\sqrt{s}$ = 7 TeV}
\bibitem{ref:4jet} PhysRevD.89.092010, CMS Collaboration, Measurement of four-jet production in proton-proton collisions at $\sqrt{s}=7\mathrm{TeV}$
\bibitem{ref:4jet2} {Underlying Event Tunes and Double Parton Scattering}, {CMS Collaboration, PAS-GEN-14-001}
\bibitem{ref:jpsi}  JHEP 1409, CMS Collaboration, Measurement of prompt $J/\psi$ pair production in pp collisions at $\sqrt{s}=7\mathrm{TeV}$
\end{thebibliography}



==> DPS/Gaunt/content_Gaunt_2v1.tex <==
\title{Conventional versus single-ladder-splitting contribution to double gluon-gluon initiated
processes}
\author{Jonathan R.~Gaunt$^1$, Rafa{\l} Maciu{\l}a$^2$ and Antoni Szczurek$^{2,3}$}
\affiliation{$^1$DESY Hamburg, Germany, $^2$Cracow, INP, Poland \& $^3$Rzesz\'ow U.,Poland
}

\maketitle

It is known that there are (at least) two different types of contribution to the double parton
scattering (DPS) cross section. One of these is the well-known `conventional'/2v2 contribution in 
which two separate ladders emerge from both protons and interact in two separate hard interactions.
The other type of process is the `perturbative 
ladder splitting'/2v1 contribution, which is similar to the 2v2 process except that one proton 
initially provides one ladder, which later perturbatively splits into two. In \cite{Gaunt:2014rua} we performed a study of the ladder splitting effects in
several DPS processes in which gluon-gluon fusion is the dominant mechanism for both subprocesses
-- namely double quarkonium, $HH$, and $c\bar{c}c\bar{c}$ production (see also \cite{Blok:2013bpa}
for a similar study in the context of four-jet, $\gamma
+ 3j$, $W+jj$ and $W^+W^-$ production).

In order to calculate the 2v2 and 2v1 DPS cross sections one needs values for both the `independent
ladder pair' (ILP) and `ladder splitting' (LS) double PDFs (dPDFs). Schematically, $\sigma(2v2) \propto
\text{ILP dPDF} \otimes \text{ILP dPDF} \times 1/\sigma_{eff,2v2}$ and $\sigma(2v1) \propto \text{ILP dPDF} 
\otimes \text{LS dPDF} \times 1/\sigma_{eff,2v1}$, with $1/\sigma_{eff,2v1}$ and $1/\sigma_{eff,2v2}$
geometrical prefactors. We took a simple
product of MSTW2008LO PDFs to be the ILP dPDF. The LS dPDFs were calculated using MSTW2008LO PDFs for
the initial single ladder, and permitting splitting starting at $Q_0 = 1$ GeV. Following simple model 
considerations we took $\sigma_{eff,2v2}/\sigma_{eff,2v1} = 2$ and $\sigma_{eff,2v2} = 30$ mb.

 In the first part of the study the LS and ILP dPDFs were compared directly at scales $\mu_1,\mu_2 
 = 10$ GeV. The ratio of LS/ILP was found to be rather flat for various parton combinations
 %for various parton combinations ($gg$, $gu$,
% %$u\bar{u}$, and $u\bar{d}$) 
 at small $x_1,x_2 \lesssim 10^{-3}$. The reason for this is that the ladder splitting 
 in the LS dPDF tends to occur very early -- this means that the LS and ILP dPDFs to have the same 
 `two-ladder' evolution over most of their evolution range, which causes their low $x$ shapes to converge.
 
Next 2v1 and 2v2 cross sections were compared for the double quarkonium (\& $HH$) process. Values of 
$R = \sigma(2v1)/\sigma(2v2)$ between $0.4 - 1.3$ were obtained varying $\sqrt{s}$ of the $pp$
collision between $0.2-13$ TeV, and $M$ of produced heavy particles between $3-126$ GeV. Increasing
$\sqrt{s}$ decreased $R$, whilst increases in $M$ increased it. Plots of $R$ against the rapidities of
the produced particles for fixed $\sqrt{s},M$ were also produced, and were found to be rather flat as
a result of the similar $x$ shapes of the underlying dPDFs.

\begin{wrapfigure}{r}{5cm}
\centering
\includegraphics[trim = 1cm 2cm -2cm 3cm, scale=0.3]{DPS/Gaunt/sigeff_sqrtS_chi.eps}
\end{wrapfigure}

Another quantity of interest to plot is the empirical $\sigma_{eff} = \sigma_{A,B} (DPS)/[\sigma_A(SPS)
\sigma_B(SPS)]$ (SPS = single scattering) that is often extracted in experiments. If only the 2v2 mechanism were present this
quantity would be approximately constant, whereas with the two components it increases slowly with
$\sqrt{s}$ and decreases slowly with scale (a plot for double quarkonium is given to the right). The
variation of $\sigma_{eff}$ with scale is a key prediction of the two-component DPS framework, and it 
would be interesting to test this if possible at the LHC experiments.

Finally the 2v1 and 2v2 cross sections were compared for the $c\bar{c}c\bar{c}$ process. The results
obtained were broadly similar to those for the double quarkonium process. For this process one can
plot more differential distributions, such as the $p_T$ and rapidity of the charm particles. The 2v1
and 2v2 contributions to these distributions were found to have very similar shapes, making it difficult
to disentangle the 2v1 and 2v2 contributions via these quantities.

\vspace{-0.5cm}



\begin{thebibliography}{9}

% \bibitem{Gaunt:2012dd}
%   J.~R.~Gaunt,
%   %``Single Perturbative Splitting Diagrams in Double Parton Scattering,''
%   JHEP {\bf 1301} (2013) 042
%   [arXiv:1207.0480 [hep-ph]].


\bibitem{Gaunt:2014rua}
  J.~R.~Gaunt, R.~Maciu{\l}a and A.~Szczurek,
  %``Conventional versus single-ladder-splitting contributions to double parton scattering production of two quarkonia, two Higgs bosons and $c \bar c c \bar c$,''
  Phys.\ Rev.\ D {\bf 90} (2014) 054017
  [arXiv:1407.5821].

\bibitem{Blok:2013bpa}
  B.~Blok, Y.~Dokshitzer, L.~Frankfurt and M.~Strikman,
  %``Perturbative QCD correlations in multi-parton collisions,''
  Eur.\ Phys.\ J.\ C {\bf 74} (2014) 2926
  [arXiv:1306.3763].
  

  

  

  
  
  
\end{thebibliography}



==> DPS/Gaunt/content_Gaunt_Glauber.tex <==
\title{Glauber Gluons and Multiple Parton Interactions}
\author{Jonathan R.~Gaunt}
\affiliation{DESY Hamburg, Germany
}

\maketitle

Factorisation formulae are a key tool for making predictions at the LHC. 
%They separate the short 
%distance physics of interest from the long-distance QCD physics (with the latter part not being
%entirely calculable using perturbation theory, but being universal and process-independent). 
Factorisation at the leading power in $\Lambda_{QCD}/Q$ (with $Q$ the hard scale) has only been 
rigorously proven in hadron-hadron collisions for the inclusive cross section for $p + p \to V + X$,
where $V$ is colourless and $X$ can be anything, and for the cross section differential 
in the $p_T$ of the $V$ for this process \cite{Collins:1985ue}.

One important difficulty in obtaining a factorisation formula is the treatment of the so-called
Glauber region. A particle in the Glauber region has momentum $r$ that satisfies $|r^+r^-| \ll 
\mathbf{r}^2$, where $r^\pm = (r^0 \pm r^3)/\sqrt{2}$, $\mathbf{r} = (r^1,r^2)$. A Feynman graph
can have a leading power contribution when some of the particles are in the Glauber region (and 
others are in the so-called central soft $S$, collinear $J$, or hard $H$ regions). However, unlike 
the $S$, $J$ and $H$ contributions, the Glauber contribution cannot readily be disentangled 
from the rest to achieve factorisation. In \cite{Collins:1985ue} it was shown that the
contribution from the Glauber region cancelled for the considered observables.

`Standard' factorisation formulae containing only $S$, $J$ and $H$ contributions have been 
written down for other observables, and some 
partially proven. Here we focus on the observable of hadronic transverse energy, or $E_T$. 
In $p + p \to V + X$, $E_T = \sum_{i \in X} \sqrt{p_{Ti}^2+m_i^2}$. A factorisation (or resummation) 
formula for this observable was written down in \cite{Papaefstathiou:2010bw}. However, when 
comparing the results of this formula to the results from Monte Carlo generators incorporating 
multiple parton interactions (MPI), a noticable discrepancy is seen \cite{Papaefstathiou:2010bw}.
It is interesting to ask whether the effects of MPI on this observable, missing in the standard 
factorisation formula, correspond to a leading power Glauber contribution, or a numerically (very) 
large power correction.

In \cite{Gaunt:2014ska} we addressed this question, investigating the contribution of Glauber 
gluons to the observable $E_T$, when $E_T \ll Q$. This was done using a model set-up
in which each proton is considered to be composed only from a $q\bar{q}$ pair. We focussed
on Glauber gluon exchanges between the `spectator' partons not involved in the `primary' 
$q\bar{q} \to V$ hard process. This is because it is only for these exchanges that the
integral contour is trapped in the Glauber region. 


\begin{wrapfigure}{r}{5cm}
\centering
\includegraphics[trim = 0.5cm 0.5cm 0.5cm 0.5cm, scale=0.4]{DPS/Gaunt/twoglauber.eps}
\end{wrapfigure}


It was found that the leading power Glauber contributions cancelled for one Glauber 
gluon exchanged between spectators, but failed to cancel at the level of two-gluon exchange (see
right). The non-cancellation can be traced to a mismatch in $E_T$ value between the cut passing
between the Glauber gluons (short-dashed line, MPI occurs) and those passing either side of the Glauber 
system (long-dashed lines, absorptive process occurs).

In this way a link between leading power contributions from Glauber gluons to $E_T$ and MPI effects
can be established. For similar reasons one expects leading power Glauber/MPI contributions
to other event shape observables in $pp$, such as beam thrust and transverse thrust. The effect of
these Glauber exchanges/MPI can be suppressed by considering jet-based observables. On the other hand
measurements of these event shape variables can be useful to measure MPI effects and tune Monte Carlo
event generators.

%Our discussion was for $E_T \ll Q$ -- however one also anticipates a problem with applying the standard
%factorisation formula even when $E_T$ is larger. This is because Glauber miscancellations on multiple 
%spectator legs (i.e. many extra interactions) are possible and have a cumulative effect on the observable,
%causing large smearing effects.

\begin{thebibliography}{9}

\bibitem{Collins:1985ue}
  G.~T.~Bodwin,
  %``Factorization of the Drell-Yan Cross-Section in Perturbation Theory,''
  Phys.\ Rev.\ D {\bf 31} (1985) 2616, {\bf 34} (1986) 3932 (E).
  J.~C.~Collins, D.~E.~Soper and G.~F.~Sterman,
  %\emph{``Factorization for Short Distance Hadron - Hadron Scattering}.
  Nucl.\ Phys.\ B {\bf 261} (1985) 104,
  %\emph{Soft Gluons and Factorization}.
  %Nucl.\ Phys.\ B 
  {\bf 308} (1988) 833.

  
  \bibitem{Papaefstathiou:2010bw}
  A.~Papaefstathiou, J.~M.~Smillie and B.~R.~Webber,
  %``Resummation of transverse energy in vector boson and Higgs boson production at hadron colliders,''
  JHEP {\bf 1004} (2010) 084
  [arXiv:1002.4375 [hep-ph]].
    M.~Grazzini, A.~Papaefstathiou, J.~M.~Smillie and B.~R.~Webber,
  %``Resummation of the transverse-energy distribution in Higgs boson production at the Large Hadron Collider,''
  JHEP {\bf 1409} (2014) 056
  [arXiv:1403.3394 [hep-ph]].

\bibitem{Gaunt:2014ska}
  J.~R.~Gaunt,
%  \emph{Glauber Gluons and Multiple Parton Interactions}.
  JHEP {\bf 1407} (2014) 110
  [arXiv:1405.2080 [hep-ph]].
  
%\bibitem{Stewart:2009yx}
%  I.~W.~Stewart, F.~J.~Tackmann and W.~J.~Waalewijn,
%  \emph{Factorization at the LHC: From PDFs to Initial State Jets}.
%  Phys.\ Rev.\ D {\bf 81} (2010) 094035
%  [arXiv:0910.0467 [hep-ph]].
  
  
  
\end{thebibliography}



==> DPS/Gueta/content_Gueta.tex <==
\title{Measurement of hard double-parton interactions in $W (\rightarrow \ell \nu)$~+ 2 jet events at $\sqrt{s}=$~7~TeV with the ATLAS detector}
\author{Orel Gueta {\small (on behalf of the ATLAS collaboration)}}
\affiliation{Tel Aviv University}

\maketitle

\noindent The production of $W$ bosons in association with two jets in $pp$ collisions at a centre-of-mass energy of $\sqrt{s}\,=\,7 \TeV$ has been analysed for the presence of double-parton interactions using data corresponding to an integrated luminosity of 36~$\ipb$, collected with the ATLAS detector at the LHC~\cite{Aad:2013bjm}.
The fraction of events arising from double-parton interactions, $\fDP{D}$, has been measured through the $\pt$~balance between the two jets.
The observable, $\DeltaJn$, defined as 
\[
    \DeltaJn\;=\; \frac{|{\vec{p}_\mathrm{T}}^{J_1}+{\vec{p}_\mathrm{T}}^{J_2}|}{|\vec{p}_\mathrm{T}^{J_1}|+|\vec{p}_\mathrm{T}^{J_2}|}\,, 
\]
was chosen as it shows good discriminating power between the direct production of a $W$ boson with two jets ($W_{2\mathrm{j}}$) and the production of a $W$ boson in association with zero jets in addition to another parton--parton scatter resulting in two jets ($W_{0\mathrm{j}}+2\mathrm{j_{DPI}}$).
A fit is performed to the normalised, detector-level, background-corrected data distribution of \DeltaJn using two normalised templates, denoted by $A$ and $B$. 
The result of the fit of the form $(1 \!-\! \fDP{D}) \!\cdot\! A \!+\! \fDP{D} \!\cdot\! B$ is shown in Figure~\ref{fig:fitDeltaN}. 
Template $A$ represents the expected contribution to the distribution of \DeltaJn from $W_{2\rm{j}}$ events 
and is selected from events generated with the \textsc{Alpgen} Monte Carlo generator, interfaced with \textsc{Herwig} and \textsc{Jimmy} (\AHJ).
Template $B$ represents the expected contribution from $W_{0\mathrm{j}}\!+\!2\rm{j_{DPI}}$ events and is estimated from dijet events in data.
%
%\thisfloatsetup{floatwidth=.6\textwidth,capbesidewidth=sidefil,
%capposition=beside,capbesideposition={right,center}}
%-----------------------------------------------------------------------------
\begin{figure}[!h]
\begin{minipage}{0.47\textwidth}
 \centerline{\includegraphics[width=1.0\textwidth]{DPS/Gueta/figures/fit_DeltaJets_n_Alpgen.eps}}
\end{minipage}
\hspace{0.5cm}
\begin{minipage}{0.47\textwidth}
   \caption{  \label{fig:fitDeltaN}
\small  Distribution of \DeltaJn from background-subtracted data (dots) compared to the result from the best fit for $\fDP{D}$~\cite{Aad:2013bjm}. 
        The result of the fit is shown as the green histogram. 
        The bins to the right of the vertical dash-dotted line were excluded from the fit. 
        Data and the overall fit have been normalised to unity, Template $A$ (dashed line) to $1-\fDP{D}$ and Template $B$ (blue solid line) to $\fDP{D}$.}
\end{minipage}
\end{figure}
%------------------------------------------------------------------------------


For jets with transverse momentum $p_{\rm T} > 20$~GeV and rapidity $|y|<2.8$, a central value of
\[
\fDP{D} = 0.08 \pm 0.01~(\rm{stat.}) \pm 0.02 ~(\rm{sys.}) 
\]
is obtained. 
The result for $\fDP{D}$ is used to extract the parameter $\sigma_\mathrm{eff}$.
In the formalism presented in this measurement, $\sigma_\mathrm{eff}$ is a universal scaling parameter, defined at the parton-level which is process and phase-space independent.
It quantifies the probability for a secondary hard interaction in the same collision.
The value extracted from data is
\[
\sigma_\mathrm{eff}(7~\,\mbox{\rm TeV}) = 15 \pm 3~(\rm{stat.})~^{+5}_{-3} ~(\rm{sys.})~mb. 
\]
This value is consistent with values measured in other experiments at various centre-of-mass energies.

\begin{thebibliography}{9}
        \bibitem{Aad:2013bjm} ATLAS Collaboration, New J. Phys. \textbf{15} (2013) 033038.
\end{thebibliography}


==> DPS/Gunnellini/content_Gunnellini.tex <==
\title{DPS and determinations of $\sigma_{\textrm{\scriptsize{eff}}}$}
\author{Paolo Gunnellini, on behalf of the CMS Collaboration}
\affiliation{DESY, Hamburg (Germany)\\Universiteit Antwerpen (Belgium)}

\maketitle

\section*{Open problems}
Measurements sensitive to double parton scattering (DPS) signals have been carried out in different final states by several experiments \cite{Chatrchyan:2013xxa,Aad:2013bjm,Abazov:2014fha}. The final goal of a DPS analysis is to extract a value for the quantity $\sigma_{\textrm{\scriptsize{eff}}}$. Current methods used for $\sigma_{\textrm{\scriptsize{eff}}}$ extraction rely on the so-called ``template method'', which uses fits to DPS-sensitive observables performed with two different templates, one for the background contribution and one for the signal. The template method has been found to be very solid and reliable but there are some issues connected to the definition of the templates. In particular, it is difficult and sometimes even impossible to define an appropriate background template in a consistent way with different Monte Carlo event generators. This feature consequently brings larger uncertainties due to model dependence and some ambiguity in the $\sigma_{\textrm{\scriptsize{eff}}}$ extraction. 

\section*{Results and Outlook}
A new method for $\sigma_{\textrm{\scriptsize{eff}}}$ determinations, called ``tuning method'', has been developed in order to circumvent the issues related to the definition of the templates. It is based on inclusive fits of measured DPS-sensitive observables with predictions generated with different choices of the Underlying Event (UE) parameters implemented in the simulation. The output of the fit is the tune of UE parameters which provides the best description of the data. The tune defines the corresponding value of $\sigma_{\textrm{\scriptsize{eff}}}$. The extraction of $\sigma_{\textrm{\scriptsize{eff}}}$ with the tuning method can be easily performed with the use of the RIVET \cite{Buckley:2010ar} and the PROFESSOR \cite{Buckley:2009bj} software. RIVET is used to generate predictions by using the corresponding plugin of the DPS-sensitive analysis. PROFESSOR is used to automatically generate random choices of the parameters, to interpolate the response of the predictions and to fit the data with the obtained predictions. The innovative part of the method is that an inclusive fit is taken without the need of dividing the contributions in background and signal.\\
Results have been obtained for the measurement of four-jet final states performed at the CMS experiment \cite{Chatrchyan:2013qza}. The tuning method has been applied  by using the PYTHIA8 event generator \cite{Sjostrand:2007gs} by fitting two DPS-sensitive observables, namely $\Delta$S and $\Delta^{\textrm{\scriptsize{rel}}}_{\textrm{\scriptsize{soft}}}p_{\textrm{\scriptsize{T}}}$. They investigate the relative position of the jets in the transverse plane and they show sensitivity to a possible DPS signal. Values of $\sigma_{\textrm{\scriptsize{eff}}}$ are listed in Table \ref{tablesigma} \cite{CMS:2014sva}, as well as the goodness of the fits, $\chi^2$/NdF. 

\begin{table}[htbp] 
\begin{center}
\begin{tabular}{|r|l|l|}
\hline
Tune & $\chi^2$/NdF & $\sigma_{\textrm{\scriptsize{eff}}}$ (mb)\\
\hline
P8 4C & - &  30.3\\
CDPSP8S1-4j & 0.751 & 21.3$^{+1.2}_{-1.6}$\\
CDPSP8S2-4j & 0.428 & 19.0$^{+4.7}_{-3.0}$\\
\hline
\end{tabular}
\caption{Values of $\sigma_{\textrm{\scriptsize{eff}}}$ obtained for the new tunes compared to the UE-based tune 4C. The goodness of fit, evaluated as $\chi^2$ divided by the number of degrees of freedom, is also indicated for the new tunes.}
\label{tablesigma}
\end{center}
\end{table}

Two different fits have been performed: CDPSP8S1-4j, which considers a variation of only the amount of matter overlap between the two protons and CDPSP8S2-4j which extends the tune to the whole set of UE parameters. The values of $\sigma_{\textrm{\scriptsize{eff}}}$ obtained for the new tunes are found to be compatible between each other around 20 mb. They are smaller than the $\sigma_{\textrm{\scriptsize{eff}}}$ value predicted by the UE-based tune 4C. This indicates that the DPS contribution implemented in the tune 4C needs to be increased in order to improve the description of four-jet observables. \\ The new approach proposed with the tuning method is very useful and efficient to extract $\sigma_{\textrm{\scriptsize{eff}}}$. It is very quick and easy to implement with any MC generator and any model of Multiple Parton Interaction (MPI). The tuning method requires a three-step procedure. First of all, the considered DPS-sensitive observables need to be corrected to the particle level; then the fit is performed on those. Finally the corresponding value of $\sigma_{\textrm{\scriptsize{eff}}}$ can be extracted and can be compared to results obtained with any other Monte Carlo event generator and physics channel. We would like to suggest some points and remarks which should be considered when using the tuning method. They are listed in the following:

\begin{itemize}
\item Investigation of the contribution of different matrix elements used with the same UE simulation;
\item Use more than one MC event generator to study the DPS contribution needed in different models;
\item Use more than one variable for the DPS determination;
\item Check if the new set of parameters spoil description of more inclusive distributions. 
\end{itemize}

We think that the tuning method is very reliable for determinations of $\sigma_{\textrm{\scriptsize{eff}}}$ and may become very important for the next LHC phase where it can be applied to measurements at a new and unexplored collision energy.

\begin{thebibliography}{9}
 
\bibitem{Chatrchyan:2013xxa}
  S.~Chatrchyan {\it et al.},
  ``Study of double parton scattering using W + 2-jet events in proton-proton collisions at $\sqrt{s}$ = 7 TeV,''
  JHEP {\bf 1403} (2014) 032

\bibitem{Aad:2013bjm}
  G.~Aad {\it et al.},
  ``Measurement of hard double-parton interactions in $W(\to l\nu)$+ 2 jet events at $\sqrt{s}$=7 TeV with the ATLAS detector,''
  New J.\ Phys.\  {\bf 15} (2013) 033038

\bibitem{Abazov:2014fha}
  V.~M.~Abazov {\it et al.},
  ``Double parton interactions in photon + 3 jet and photon + $b/c$ jet + 2 jet events in $p\bar{p}$ collisions at $\sqrt{s}=1.96$ TeV,''
  Phys.\ Rev.\ D {\bf 89} (2014) 072006

\bibitem{Buckley:2010ar}
  A.~Buckley, J.~Butterworth, L.~Lonnblad, D.~Grellscheid, H.~Hoeth, J.~Monk, H.~Schulz and F.~Siegert,
  ``Rivet user manual,''
  Comput.\ Phys.\ Commun.\  {\bf 184} (2013) 2803

\bibitem{Buckley:2009bj}
  A.~Buckley, H.~Hoeth, H.~Lacker, H.~Schulz and J.~E.~von Seggern,
  ``Systematic event generator tuning for the LHC,''
  Eur.\ Phys.\ J.\ C {\bf 65} (2010) 331

\bibitem{Chatrchyan:2013qza}
  S.~Chatrchyan {\it et al.},
  ``Measurement of four-jet production in proton-proton collisions at sqrt(s) = 7 TeV,''
  Phys.\ Rev.\ D {\bf 89} (2014) 092010

\bibitem{Sjostrand:2007gs}
  T.~Sjostrand, S.~Mrenna and P.~Z.~Skands,
  ``A Brief Introduction to PYTHIA 8.1,''
  Comput.\ Phys.\ Commun.\  {\bf 178} (2008) 852

\bibitem{CMS:2014sva}
  CMS Collaboration,
  ``Underlying Event Tunes and Double Parton Scattering,''
  CMS-PAS-GEN-14-001.

\end{thebibliography}



==> DPS/Haevermaet/content_Haevermaet.tex <==
\title{The study of QCD in high pile-up environments with Higgs boson and Drell-Yan production}
\author{H. Van Haevermaet}
\affiliation{Deutsches Elektronen Synchrotron, D 22603 Hamburg \\ Universiteit Antwerpen, Elementaire Deeltjes Fysica, B 2020 Antwerpen}

\maketitle

\section*{Open problems}
The study of QCD is typically done using measurements of processes in single proton-proton collisions. With its clean final state, a particular interesting one is the Drell-Yan process, which can be used to precisely measure the quark structure functions, parton showers, and underlying event properties. The properties and structure functions of gluons however, have to be determined indirectly. With the recent discovery \cite{bib:higgs} of the Higgs boson, this picture changes. In the heavy top limit, the Higgs boson directly couples to gluons and can be produced with the gluon fusion process through a colour singlet current \cite{bib:gluonfusion}. The access to this new process opens up a whole new interesting area of possible QCD measurements, where one can directly study gluon induced effects \cite{bib:higgsgluon}. However, due to the small cross sections, current accelerators like the LHC at CERN have to operate at very high beam intensities to collect sufficient statistics. This allows one to measure differential distributions, but it also creates a condition (called pile-up) in which on average much more than one proton-proton collision happens per bunch crossing. This implies that the phase space will be completely filled with extra hadronic activity coming from the pile-up events, which makes a study of QCD in the Higgs or Drell-Yan channels extremely difficult. 

\section*{Outlook}
In this study we presented a novel method that compares Higgs and Drell-Yan production in the same invariant mass and rapidity range to perform a direct measurement of gluon versus quark induced processes. In particular we studied the underlying event activity in Higgs and Drell-Yan processes by looking at the charged particle multiplicity and scalar $\Sigma p_{T}$ in the transverse region. We constructed the subtracted underlying event observable, and comparing pile-up = 0, 20, and 50 scenarios we can conclude that it is stable in high pile-up environments. Thus, by comparing Higgs to Drell-Yan production we can subtract the pile-up contributions, and directly measure the difference in gluon versus quark induced initial state radiation effects, such that one can still access (small-$p_{T}$) QCD physics in high pile-up environments. Furthermore, this method allows for a completely detector independent pile-up subtraction that is not limited to the small experimental tracker ranges where vertex identification can be used. Hence it does not introduce any extra bias or uncertainty due to such complicated corrections, and even allows to measure initial state radiation in more forward regions. Finally, we are in the process of applying the same kind of strategy to vector boson + jet topologies to study the high-$p_{T}$ region of QCD. 

\begin{thebibliography}{9}
\bibitem{bib:higgs} ATLAS Coll. (G. Aad et al.), Phys. Lett. {\bf B716} (2012) 1; CMS Coll. (S. Chatrchyan et al.), Phys. Lett. {\bf B716} (2012) 30.
\bibitem{bib:gluonfusion} H. M. Georgi et al., Phys. Rev. Lett. {\bf 40}, 692 (1978); J. Ellis et al., Nucl. Phys. {\bf B106} (1976) 292; M.A. Shifman et al., Sov. J. Nucl. Phys. {\bf 30} (1979) 711.  
\bibitem{bib:higgsgluon} P. Cipriano et al., Phys. Rev. D {\bf 88}, 097501 (2013), H.~Van Haevermaet et al.,
  %``Higgs boson as a gluon trigger: the study of QCD in high pile-up environments,''
  arXiv:1407.2815 [hep-ph].
\end{thebibliography}



==> DPS/Krasny/content_Krasny.tex <==
\title{DPS and the Higgs signal strength at the LHC }
\author{Mieczyslaw Witold Krasny }
\affiliation{LPNHE, Universit\'{e}s Paris VI et VII and CNRS--IN2P3, Paris, France}

\maketitle

\section*{Purpose}

The principal  purpose of this talk was: (1)  to bring to an attention,  and (2) to 
stimulate discussions, within  the Double Parton Scattering (DPS)  expert 
community,  on the loopholes in our present  theoretical and experimental 
understanding of the vector bosons pair (VV) production at the LHC.  In the 
region in which the transverse momenta of both bosons are small, the kinematical 
characteristics of leptons produced by the  conventional  sources 
mimic very closely those of  the Higgs boson 
decays.  To establish beyond any doubt the evidence of the SM Higgs boson 
and to determine the strength of its coupling to vector bosons additional
calculations are needed. They must merge, so far distinct, efforts
of the "QCD-boxes" and the "DPS" communities to address   the interplay between 
the gluon-gluon scattering box diagrams and the full set of the DPS processes, 
with a special attention to the  DPS collinear singularity region. 



\section*{DDYP and the Higgs searches background}

The specific type of the DPS: the Double Drell-Yan Process (DDYP), and its 
contribution  to the vector boson pair production at the LHC was discussed in \cite{DPS}, 
where the WINHAC generator was adopted to study the DDYP contribution
within the approximation in which the amplitude interferences, colour, spin and flavour 
correlations, correlations between the  longitudinal momenta of participants 
(beyond the momentum conservation constraints) were neglected. Already within 
such an approximation the DDYP contribution was found to mimic rather closely the Higgs boson 
decay signals, both in the $4l$ and $2l2\nu$ channels, provided that the $\sigma _{eff}$ for the scattering of the 
same flavour quark-antiquark pairs (for which no experimental constraint exists) 
is significantly smaller than that  for the quark-gluon and gluon-gluon pairs. 
 
 Several possible sources of enhancements of the DDYP probability 
 were discussed in this contribution:  (1) the reduced 
 transverse plane correlation length for the same flavour, opposite charge quark-antiquark pairs;
(2) the flavour correlation effects in proton excitations satisfying the local charge and flavour conservation;
(3) the spin effects assuring the local spin compensation within the proton; and  
(4) the alternative mechanism of the electro-weak symmetry breaking, enhancing the VV cross-sections.  


\section*{Outlook}

The DDYP contribution to the Higgs background  was assumed by the ATLAS and CMS collaboration  to be negligible. 
This is indeed  the case for the simpleminded model lacking flavour, longitudinal momentum, transverse momentum and spin correlations 
between colliding partons. In our view the above conclusion is premature and needs further investigation of several reasons of the enhancement of the DDYP cross-sections were presented in this talk. The main purpose of the talk was to advocate a need for  a new theoretical calculations beyond the leading-order and leading-twist approximations and, 
perhaps more importantly,  the necessity of a more open investigation of the properties of observed excesses of VV events at the LHC -- beyond  the SM Higgs 
decay context. 


\begin{thebibliography}{9}
\bibitem{DPS}
 M.W. Krasny and W. Placzek, Acta Phys.Polon. B45 (2014) 1, 71-87

\end{thebibliography}



==> DPS/Lewandowska/content_Lewandowska.tex <==
\title{Electroweak boson production in double parton scattering}
\author{Emilia Lewandowska and Krzysztof Golec-Biernat}
\affiliation{Institute of Nuclear Physics Polish Academy of Sciences\\Krakow, Poland}

\maketitle


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Open problems}


We study  the $W^+W^-$ and $Z^0Z^0$ electroweak boson production in double parton scattering (DPS)  using  QCD evolution equations for double parton distribution functions (DPDFs) \cite{Golec-Biernat:2014nsa}.
In particular, we analyse  the impact  of  splitting terms in the evolution equations on the DPS cross sections. 
Unlike the standard terms, the splitting terms are not suppressed for large values of the relative momentum of two partons 
initiating  the DPS, thus they play an important role for  the DPS cross sections.




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Outlook}



In our work, we have analyzed the DPS processes in the collinear approximation, using QCD evolution equations  for the DPDFs.  We have  concentrated on the significance of the splitting terms in these equations
for the DPS processes with a large hard scale $Q\sim 100~{\rm GeV}$. For the illustration, 
we considered the $W^+W^-$ and
$Z^0Z^0$ boson production at the LHC center-of-mass energy ${14}~{\rm TeV}$. To compute the DPS cross sections, 
we have specified the dependence of the DPDFs on the relative momentum ${\bf q}$. 
The DPS cross sections can be written  as
the  sum of two components
\begin{eqnarray}\label{eq:cross11}
\sigma_{AB} \,=\,\sigma_{AB}^{(11)}\,+\,\sigma_{AB}^{(12+21)}\,
\end{eqnarray}
in which
\begin{eqnarray}\nonumber
\label{eq:cross11a}
\sigma_{AB}^{(ij)}\!&=&\!\frac{N}{2}
\sum_{f_i,f_i^\prime}\int dx_1dx_2\,dz_1dz_2\, \int\frac{d^2{\bf q}}{(2\pi)^2}\,
\theta(Q-|{\bf q}|)
\\ 
&\times&\! D_{f_1f_2}^{(i)}(x_1,x_2,Q,{\bf q})\, {\hat{\sigma}}^A_{f_1f_1^\prime}(Q)\,
{\hat{\sigma}}^B_{f_2f_2^\prime}(Q)\, 
D_{f_1^\prime f_2^\prime}^{(j)}(z_1,z_2,Q,-{\bf q}).
\end{eqnarray}
The splitting component, ${\sigma_{AB}^{(12+21)}}$,  is not strongly suppressed  
at large values of $|{\bf q}|$, like the standard component, ${\sigma_{AB}^{(11)}}$, because it originates from the splitting  
of a pointlike parton. 
Based on the  constructed numerical program, which solves the evolution equations for DPDFs, 
we analyzed  the single splitting contribution to the DPS cross sections for the electroweak boson production.
We  quantified  the relevance of the single splitting  contribution in such a case in terms of the effective cross section.
We also discussed the correlations in rapidity for the produced $W^\pm$ bosons pointing out that the single splitting contribution
distorts the standard correlation obtained with the factorized DPS cross section. 
 






%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{thebibliography}{9}
%\cite{Golec-Biernat:2014nsa}
\bibitem{Golec-Biernat:2014nsa} 
  K.~Golec-Biernat and E.~Lewandowska,
  ``Electroweak boson production in double parton scattering,''
  Phys. Rev. D. 90, 094032 (2014).
  %%CITATION = ARXIV:1407.4038;%%
  %1 citations counted in INSPIRE as of 01 Dec 2014.
\end{thebibliography}



==> DPS/Maciula/content_Maciula.tex <==

\title{Double open charm production at the LHC within\\ single- and double-parton scattering}
\author{Rafa{\l} Maciu{\l}a}
\affiliation{Institute of Nuclear Physics Polish Academy of Sciences}

\maketitle

\section*{Outlook}

We discuss production of two pairs of $c \bar{c}$ within a simple formalism of double-parton scattering (DPS). Surprisingly large cross sections, comparable to single-parton scattering (SPS) contribution, are predicted for LHC energies. We compare results of exact calculations of single-parton scattering (SPS) and double-parton scattering (DPS) for production of $c \bar{c} c \bar{c}$ and for $D-D$ meson-meson correlations \cite{Maciula:2013kd}. Each step of DPS is calculated within $k_t$-factorization approach, i.e. effectively including higher order corrections. The SPS calculations are performed in collinear approximation with exact matrix element for $gg \to c \bar{c} c \bar{c}$ subprocess as well as with approximate matrix elements in high-energy approximation. We compare our predictions for double charm production (DD meson-meson pairs) with recent results of the LHCb collaboration for azimuthal angle $\phi_{DD}$, dimeson invariant mass $M_{DD}$ and rapidity distance between mesons $Y_{DD}$. The predicted shapes are similar to the measured ones, however, some strength seems to be lacking. Our calculations clearly confirm the dominance of DPS in the production of events with double charm. At the LHC energy $\sqrt{s}$ = 7 TeV one observes unprecedent
dominance of double parton scattering. At the nominal LHC energy $\sqrt{s}$ = 14 TeV the dominance would be even larger.
This opens a possibility to study the DPS effects in the production of charmed mesons.

\section*{Open problems}
We have calculated several distributions and compared our results
with experimental data of the LHCb collaboration.
Our DPS mechanism gives a reasonable interpretation of the measured
distribution. Some strength is still missing. This rather cannot be explained by
single-ladder-splitting contributions to double-parton scattering production (see e.g. Ref.~\cite{Gaunt}) which are not taken into account in this analysis.
Of course, given large theoretical uncertainties related to $\sigma_{eff}$ or with scales and charm quark mass the problem may not be easy to identify and solve.
In order to make more definite conclusions, one should rather concentrate on violation of simple factorized Ansatz for DPS. Explicit
treatment of the full-form correlation factor $F(b; x_1, x_2, \mu^{2}_{1}, \mu^{2}_{2})$ in double-parton
distributions is expected to result in reduced value of $\sigma_{eff}$ with increasing scales $\mu^{2}_{1}$, $\mu^{2}_{2}$ \cite{Gustaffson2011}.  
Another idea is to include spin correlations \cite{Kasemets}. For conventional DPS mechsanism these effects are expected to be rather small after evolution, especially
when both partons are gluons. However, it might be interesting to do a more detailed study of the spin effects, also
including their effect in the single-ladder-splitting mechanisms. This
is particularly interesting in light of the experimentally
observed azimuthal correlations between two $D^{0}$ mesons produced in proton-proton collisions.  
Still open but very important question is the DPS contribution to
inclusive single particle spectra. We emphasized significant
contribution of DPS mechanism to inclusive charmed meson spectra measured recently by ALICE,
ATLAS and LHCb \cite{Maciula:2013kd}. Clear statement in this subject should be worked out by the MPI community.

\begin{thebibliography}{9}
\vspace{-3mm}
\bibitem{Maciula:2013kd}
R.~Maciu{\l}a, and A.~Szczurek, Phys.~Rev.~{\bf D87}, 074039 (2013).
\vspace{-3mm}
\bibitem{Gaunt}
J.~R. Gaunt, R.~Maciu{\l}a, and A.~Szczurek, Phys.~Rev.~{\bf D90}, 054017 (2014).
\vspace{-3mm}
\bibitem{Gustaffson2011}
C. Flensburg, G. Gustafson, L. L{\"o}nnblad and A. Ster, J. High Energy Phys. {\bf 06}, 066 (2011).
\vspace{-3mm}
\bibitem{Kasemets}
talk given by Tomas Kasemets at MPI@LHC 2014.


\end{thebibliography}



==> DPS/Rinaldi/content_Rinaldi.tex <==
\title{A Light-Front approach to
double parton distribution
functions
within constituent quark models}
\author{Matteo Rinaldi}
\affiliation{Dipartimento di Fisica e Geologia, Universit\`a degli Studi di
Perugia, and INFN, sezione di Perugia}

\maketitle

In a recent paper of ours \cite{new},  double parton correlations
have been properly investigated  in the valence quark region by means of a
relativistic constituent quark model through the ``Light-Front Hamiltonian
dynamics''. As found in non relativistic (NR) previous analyses
\cite{scop}, also in this framework  double parton correlations are present
without any 
additional prescription and their contributions to double parton distribution
functions (dPDFs), in the valence region, turn out to be sizable. 
In particular,
in Ref. \cite{new}, dPDFs have been calculated within a fully Poincar\'e
covariant approach which allow to overcome  some inconsistencies found in the
previous NR treatments, such as ``the bad support problem''. The most important
results of Ref. \cite{new} are the following:  $i)$ 
contributions of longitudinal momentum correlations of the interacting quarks
are found to be sizable, at variance with those related to correlations in
transverse momentum; $ii)$ after LO-QCD evolution, in the low $x$ region
accessed so far at the LHC,
including for the moment being only the non singlet sector,
the effect of dynamical correlations decreases
in the unpolarized case,
while it keeps being sizable in the spin-dependent one.  
In order to obtain a more complete analysis, closer to the present
experimental scenario,
the study of the contribution of the singlet sector to the 
pQCD evolution of the
calculated dPDFs and the calculation of the effective cross section,
entering the ``pocket formula'' approximation to 
the double parton scattering cross section,
are fundamental steps which are presently under scrutiny.

\begin{thebibliography}{9}
\bibitem{new}
%\cite{Rinaldi:2014ddl}
%\bibitem{Rinaldi:2014ddl} 
  M.~Rinaldi, S.~Scopetta, M.~Traini and V.~Vento,
  %``Double parton correlations and constituent quark models: a Light Front
%approach to the valence sector,''
  JHEP {\bf 1412}, 028 (2014)
  [arXiv:1409.1500 [hep-ph]].
  %%CITATION = ARXIV:1409.1500;%%
  %3 citations counted in INSPIRE as of 12 Jan 2015

%\cite{Rinaldi:2013vpa}
\bibitem{scop}
  M.~Rinaldi, S.~Scopetta and V.~Vento,
  %``Double parton correlations in constituent quark models,''
  Phys.\ Rev.\ D {\bf 87} (2013) 114021
  [arXiv:1302.6462 [hep-ph]].
  %%CITATION = ARXIV:1302.6462;%%
  %7 citations counted in INSPIRE as of 05 Feb 2014
\end{thebibliography}



==> DPS/Snigirev/content_Snigirev.tex <==
\title{Towards correlations
in double parton distributions}

\author{Alexander Snigirev$^{a}$, Nina Snigireva$^{b}$, Gennady Zinovjev$^{c}$}
\affiliation{$^{a}$Skobeltsyn Institute of Nuclear Physics,\\Lomonosov Moscow State University, 119991, Moscow, Russia\\
$^{b}$School of Mathematical Sciences,\\ University College Dublin, Belfield, Dublin 4, Ireland \\$^{c}$Bogolyubov Institute for Theoretical Physics, \\ National Academy of Sciences of Ukraine,  03680 Kiev-143, Ukraine}


\maketitle

%\section{Open problems}
The basic properties of double parton distribution functions (dPDFs) are reviewed in the framework of perturbative QCD in the collinear approximation.
The initial state of double parton scattering (DPS) is coded by dPDFs which quantify the joint distribution of two partons in a hadron, depending on their quantum numbers,  longitudinal momentum fractions and the relative transverse distance between them.
The dPDFs and the corresponding evolution equations are well-known only  integrated over the parton pair transverse separation in the collinear approximation.
The particular solutions  of these non-homogeneous equations may be presented in form of a convolution of single distributions  (which coincides with jet calculus rules proposed originally for the fragmentation functions).
They contribute to the inclusive cross section of DPS with a larger weight (different effective cross section) being compared to the solutions of homogeneous equations.  The latter solutions are usually approximated by factorized form if initial nonperturbative correlations are absent.

Using the explicit form of the solutions of evolution equations in the Mellin representation we demonstrate~\cite{Snigirev:2014eua} analytically that the dPDFs "forget" the initial correlation conditions (unknown {\it a priori}) at not parametrically small longitudinal momentum fractions $x_1$ and $x_2$, and the correlations perturbatively calculated survive only in the limit of large enough hard scales. Such a dominance is the mathematical consequence of the relation between the maximum eigenvalues $\Lambda(n)$ in the moments representation, ~$\Lambda(n_1+n_2)~>~\Lambda(n_1)+\Lambda(n_2)$, in QCD at large $n_1$ and $n_2$ (finite $x_1$ and $x_2$). It is independent of the strength of the initial correlation conditions at all. The numerical estimates (done by integrating directly the evolution equations) testify in favour of conclusion also that the perturbative correlation effects are significant in the kinematical region accessible in experimental measurements at energies of Tevatron and LHC.

Unlike naively accepted expectations, the QCD dynamical perturbative correlations result effectively in the dependence of the experimentally extracted effective cross section of DPS on the resolution scale. The measurements covering a larger range of the resolution scale variation might reveal the evolution effects more distinctly in accordance with the asymptotic QCD behaviour.

%\section{Outlook}
%The overall length of contribution must not exceed one page!

\begin{thebibliography}{9}
\bibitem{Snigirev:2014eua}
A.M.~Snigirev, N.A.~Snigireva, G.M.~Zinovjev, Phys. Rev. D {\bf 90}, 014015 (2014); arXiv:1403.6947 [hep-ph].
 \end{thebibliography}



==> DPS/Szczurek/content_Szczurek.tex <==
\title{Effects of double-parton scattering for the rapidity-distant jet 
production at the LHC}
\author{Antoni Szczurek$^\dagger$}
\affiliation{Institute of Nuclear Physics, Krakow, Rzeszow University, Rzeszow,Poland}

\maketitle

%------------------------------------------------------
\section*{Present status and open issues}
%-------------------------------------------------------

We have discussed production of jets widely separated in rapidity.
Several mechanisms have been discussed.
We have concentrateed on four jet $pp \rightarrow j j j j X$ production
with at least two jets with large rapidity separation in proton-proton
collisions at the LHC through the mechanism of double-parton scattering (DPS).
The DPS cross section was calculated in a factorized approximation.
Each hard subprocess was calculated in LO collinear approximation.  
The LO pQCD calculations were shown to give a reasonably good
descritption of CMS and ATLAS data on inclusive jet production
(see \cite{MS2014}).
It has been shown that relative contribution of DPS is growing with 
increasing rapidity distance between the most remote jets, 
center-of-mass energy in the proton-proton collision and with 
decreasing (mini)jet transverse momenta.
We have show also result for angular azimuthal dijet correlations calculated 
in the framework of $k_t$-factorization approximation.
Finally we have compared correlations in transverse momenta of the widely
separated jets for the LHC Run II: for the DPS,
$k_t$-factorization with Kimber-Martin-Ryskin unintegrated gluon
distribution \cite{KMR} and for illustration also for LL BFKL.
We have also shown some recent predictions of the Mueller-Navelet jets
in the LL and NLL BFKL framework.
For the CMS configuration the DPS contribution is smaller than 
the dijet collinear SPS contribution even at the high rapidity distances
and only slightly smaller than that for the NLL BFKL calculation.
The DPS final state topology is clearly different than that for the
collinear dijet SPS which may help to disentangle the two mechanisms.
It is not completely understood at present what is the production 
mechanism of jets widely separated in rapidity as no absolute 
cross section was obtained so far at the LHC.
We have discussed open issues and shown that the problem
of separation of the different mechanisms could be addressed in Run II.

%--------------------
\section*{Outlook}
%--------------------

It is not easy to say how many jets are produced in fact for each case
considered in the presentation.
In the $k_t$-factorization apprach the number of jets can be bigger 
than two, especially when using the KMR UPDFs \cite{CMS2014}. 
In the BFKL approach there can be more jets emitted in 
the middle of the BFKL ladder. This would require a Monte Carlo
BFKL-type program (some steps in this direction have been already 
undertaken \cite{Sabio_Vera}). 
The number of jets in DPS can be both smaller and bigger than 
four (simplified LO case).
We think that a study of different samples with fixed number of jets
would be interesting and useful. However, detailed interpretation will
require better theoretical methods and computer programs to be
developed.

The DPS effects are interesting not only in the context how they 
contribute to distribution in rapidity distance between the jets 
but also per se.
One could make use of correlations in jet transverse momenta,
jet transverse-momentum imbalance (see \cite{MS2014}) and 
azimuthal correlations to enhance the relative contribution of DPS.

\begin{thebibliography}{4}
\vspace{-3mm}
\bibitem{MS2014}
R. Maciula and A. Szczurek, Phys. Rev. {\bf D90} (2014) 014022.
\vspace{-3mm}
\bibitem{CMS2014}
A. Cisek, R. Maciula and A. Szczurek, a paper in preparation.
\vspace{-3mm}
\bibitem{KMR}
M. Kimber, A.D. Martin and M. Ryskin, Eur. Phys. J. {\bf C12} 655.
\vspace{-3mm}
\bibitem{Sabio_Vera}
A. Sabio Vera, a talk at the wokshop on ``QCD and diffractive processes 
at the LHC'', Trento, Italy, April 14-18 2014.


\end{thebibliography}


==> DPS/Waalewijn/content_Waalewijn.tex <==
\title{Dissecting Soft Radiation with Factorization }

\author{Wouter J.~Waalewijn}
\affiliation{Nikhef, Theory Group, Science Park 105, 1098 XG, Amsterdam, The Netherlands \\
ITFA, University of Amsterdam, Science Park 904, 1018 XE, Amsterdam, The Netherlands}

\maketitle

%\newcommand{\eq}[1]{Eq.~(\ref{eq:#1})}
%\newcommand{\fig}[1]{Fig.~\ref{fig:#1}}
%\newcommand{\df}{\mathrm{d}}
%\newcommand{\al}{\alpha}
%\newcommand{\de}{\delta}
%\newcommand{\nn}{\nonumber}

The modeling of soft hadronic activity at the LHC relies heavily on Monte Carlo programs. We scrutinize their theoretical basis, using field theory (specifically factorization) to quantify the effect of perturbative and nonperturbative primary soft radiation. This is motivated by the ambiguity between these effects and multiple parton interactions (MPI) in underlying event measurements. We compare our predictions to Pythia 8 and Herwig++ 2.7.

Instead of looking at the regions away from hard jets, we directly study the effect of various sources of soft hadronic activity on the jet invariant mass $m_J$, which is a benchmark observable at the LHC. We show how these sources can be separated by exploiting their different dependence on the jet radius $R$, jet momentum $p_T^J$, jet rapidity $y_J$, and partonic scattering process~\cite{Stewart:2014nna}.

The \emph{normalized} jet mass spectrum in $pp\to Z+$1-jet and $pp\to H+$1-jet events is given by~\cite{Jouttenus:2013hs}  \\[-2ex]
%%%
\begin{equation}  \label{eq:fact}
  \frac{1}{\sigma} \frac{\df\sigma}{\df m_J^2}
 \simeq \int \df k_S\, J_{\kappa_J}(m_J^2-2p_T^J k_S)\, S_\kappa (k_S , y_J,R)
\,.\end{equation}
%%%
\ \\[-2ex]
Here, $\kappa=\{\kappa_a,\kappa_b,\kappa_J\}$ denotes the partonic channel, and $k_{S}$ is the contribution of soft radiation to the jet mass measurement. The jet function $J_{\kappa_J}$ describes energetic final-state radiation and the soft function $S_\kappa$ initial and final-state soft radiation. \eq{fact} does not include MPI.

The soft function $S_\kappa$ is sensitive to perturbative effects $S_\kappa^{\rm pert}$ and nonperturbative effects $F_\kappa$, which can be factorized $S_\kappa = S_\kappa^{\rm pert} \otimes F_\kappa$~\cite{Korchemsky:1999kt}.
In the tail of the jet mass spectrum, $k_S \gg \Lambda_{\rm QCD}$, $S_\kappa$ can be expanded,
$S_\kappa(k_S, y_J, R) = S_\kappa^\mathrm{pert}\bigl(k_S-\Omega_\kappa(R), y_J, R \bigr)$. The resulting shift of the jet mass $m_J^2 = (m_J^2)^{\rm pert} + 2 p_T^J\, \Omega_\kappa(R)$ agrees with Pythia, as shown in the left panel of \fig{fig}.

\begin{figure}[h]
\centering
\vspace{-3ex}
\includegraphics[width=0.32\columnwidth]{DPS/Waalewijn/pythiashift_Zq} \quad
\includegraphics[width=0.3\columnwidth]{DPS/Waalewijn/Omegahad_R_AU2} \quad
\includegraphics[width=0.29\columnwidth]{DPS/Waalewijn/DelM1_pT_ISRMPI_Zq}%
\vspace{-2ex}
\caption{{\emph{Left:} The change in Pythia's jet mass spectrum from partonic to hadronic+MPI is described by a shift in the tail, and a simple convolution everywhere.
\emph{Center:} The $R$ dependence of hadronization in Pythia agrees with factorization: it fits odd powers of $R$ and for $R \ll 1$ only depends on whether the jet is initiated by a quark or gluon.
\emph{Right:} $p_T^J$ dependence of the $\sim\!\! R^4$ contributions to the jet mass in Pythia and Herwig from MPI and soft ISR for $qg\to Zq$. }}
\label{fig:fig} 
\vspace{-1ex}
\end{figure}

The field-theoretic definition of the nonperturbative parameter $\Omega_\kappa$ allows us to show that it is independent of $y_J$, only involves odd powers of $R$, and that the linear $R$ term differs between quark and gluon jets but does not depend on the full partonic process~\cite{Stewart:2014nna}. Thus MPI cannot be part of $\Omega_\kappa(R)$ because they scale like $R^4$. Hadronization in Pythia agrees very well with our predictions for $\Omega_\kappa$, as shown for the $R$ dependence in the middle panel of \fig{fig}. 

The perturbative soft function contains a interference contribution from initial-state radiation (ISR) that scales like $R^4$~\cite{Stewart:2014nna}. Current tunes do not address its potential degeneracy with MPI. As the right panel in \fig{fig} shows,
these $R^4$ contributions differ much more between tunes than their sum, and can be separated by exploiting their different $p_T^J$  and channel dependence. \ \\[-6ex]

\begin{thebibliography}{6}
\vspace{-1ex}
\bibitem{Stewart:2014nna}
I. W. Stewart, F. J. Tackmann, and W. J. Waalewijn, arXiv:1405.6722  (accepted by PRL). \vspace{-1.5ex}
\bibitem{Jouttenus:2013hs}
T. T. Jouttenus, \emph{et al.}, Phys. Rev. D {\bf 88}, 054031 (2013). \vspace{-1.5ex}
\bibitem{Korchemsky:1999kt}
G. P. Korchemsky and G. Sterman, Nucl. Phys. B {\bf 555}, 335 (1999).
\end{thebibliography}%



==> DPS/Waalewijn/content_Waalewijn_old.tex <==
\title{Separating Soft Radiation, Hadronization Effects and Multiple Parton Interactions with Predictions from Factorization}

\author{Iain W.~Stewart}
\affiliation{Center for Theoretical Physics, Massachusetts Institute of Technology, Cambridge, MA 02139, USA\vspace{0.5ex}}

\author{Frank J.~Tackmann}
\affiliation{Theory Group, Deutsches Elektronen-Synchrotron (DESY), D-22607 Hamburg, Germany\vspace{0.5ex}}

\author{Wouter J.~Waalewijn*\vspace{1.ex}}
\affiliation{Nikhef, Theory Group, Science Park 105, 1098 XG, Amsterdam, The Netherlands
\vspace{0.5ex}}
\affiliation{ITFA, University of Amsterdam, Science Park 904, 1018 XE, Amsterdam, The Netherlands
\vspace{-2ex}}


\maketitle

\begin{figure}[b]
\centering
\vspace{-3ex}
\includegraphics[width=0.8\columnwidth]{DPS/Waalewijn/pythiashift_Zq.eps}
\vspace{-2ex}
\caption{For the jet mass spectrum in \Pythiaeight, the change from partonic to hadronization+MPI is described by a simple shift in the tail, and a simple convolution everywhere.}
\label{fig:pythiashift} 
\vspace{-1ex}
\end{figure}

The modeling of soft hadronic activity at the LHC relies heavily on Monte Carlo programs. We scrutinize their theoretical basis, using field theory to quantify the effect of perturbative and nonperturbative primary soft radiation. This is motivated by the ambiguity between these effects and multiple parton interactions (MPI) in underlying event (UE) measurements. We compare our predictions to \Pythiaeight~\cite{Sjostrand:2006za, Sjostrand:2007gs} and \Herwig 2.7~\cite{Bahr:2008pv,Bellm:2013lba}.

Traditional UE measurements are restricted to the regions away from hard jets~\cite{Aaltonen:2010rm,  Aad:2011qe, Chatrchyan:2012tb}, and are used to tune MPI models in Monte Carlo programs~\cite{ATLAS:2012uec,Seymour:2013qka}. These models are subsequently extrapolated into the jet regions. Here we offer an alternative by directly considering jets. For definiteness, we restrict our discussion to the jet invariant mass $m_J$, which is an important benchmark observable at the LHC~\cite{ATLAS:2012am, CMSjetmass}. We show how various sources of soft hadronic activity can be separated by exploiting their different dependence on the jet radius $R$, jet momentum $p_T^J$, jet rapidity $y_J$, and partonic scattering process~\cite{Stewart:2014nna}.

The most important components of the factorization formula for the \emph{normalized} jet mass spectrum in $pp\to Z+$1-jet and $pp\to H+$1-jet events are~\cite{Stewart:2010tn, Jouttenus:2011wh, Jouttenus:2013hs}
%%%
\begin{align}  \label{eq:fact}
  \frac{1}{\sigma} \frac{\df\sigma}{\df m_J^2}
 &\simeq \int \df k_S\, J_{\kappa_J}(m_J^2-2p_T^J k_S)\, S_\kappa (k_S , y_J,R)
\,.\end{align}
%%%
Here, $\kappa=\{\kappa_a,\kappa_b,\kappa_J\}$ denotes the partonic channel, and $k_{S}$ is the contribution of soft radiation to the jet mass measurement. The jet function $J_{\kappa_J}$ describes energetic final-state radiation and the soft function $S_\kappa$ initial and final-state soft radiation. \eq{fact} does not include MPI.

The soft function $S_\kappa$ depends on the jet through $y_J$ and $R$ but not $p_T^J$. It is sensitive to perturbative effects $S_\kappa^{\rm pert}$~\cite{Jouttenus:2011wh} and nonperturbative effects $F_\kappa$, which can be factorized $S_\kappa = S_\kappa^{\rm pert} \otimes F_\kappa$~\cite{Korchemsky:1999kt, Hoang:2007vb}.
In the perturbative tail of the jet mass spectrum, $S_\kappa$ can be expanded
%%%
\begin{align} \label{eq:SOPE}
S_\kappa(k_S, y_J, R)
&= S_\kappa^\mathrm{pert}\bigl(k_S-\Omega_\kappa(R), y_J, R \bigr)
  \nn\\
 & \quad + \mathcal{O}\big({\lqcd^2}/{k_S^3}, \alpha_s\lqcd/k_S^2 \big)
\,.\end{align}
%%%
The nonperturbative parameter $\Omega_\kappa(R)$ shifts the jet mass
%%%
\begin{equation} \label{eq:shift}
m_J^2 = (m_J^2)^{\rm pert} + 2 p_T^J\, \Omega_\kappa(R)
\,.\end{equation}
%%%
Its field-theoretic definition allows us to show that $\Omega_\kappa$ is independent of $y_J$, only involves odd powers of $R$, and that the coefficient of the linear $R$ term differs between quark and gluon jets but does not depend on the full partonic process~\cite{Stewart:2014nna}. 

\begin{figure}[b]
\centering
\vspace{-3ex}
\includegraphics[width=0.75\columnwidth]{DPS/Waalewijn/Omegahad_R_AU2.eps}%
\vspace{-2ex}
\caption{The $R$ dependence of hadronization in \Pythiaeight agrees with factorization: It is fits odd powers of $R$, and for $R \ll 1$ only depends on whether the jet is initiated by a quark (blue dashed) or gluon (orange solid and green dotted).}
\label{fig:pythiahadr} 
\vspace{-1ex}
\end{figure}

We test the shift in \eq{shift} for \Pythiaeight in \fig{pythiashift}. By a properly chosen shift (green dot-dashed curve) of the partonic result (black dotted curve), we can describe the effect of hadronization and MPI (blue dashed curve) well in the tail. Extending the shift to a convolution (solid red curve) also leads to agreement for small $m_J$, for any reasonable $F_\kappa$ satisfying $\int \df k_S\, k_S F_\kappa(k_S,y_J,R) = \Omega_\kappa(R)$. 

Although hadronization and MPI were considered simultaneously in \fig{pythiashift}, MPI cannot be part of $\Omega_\kappa(R)$ because they scale like $R^4$. Hadronization in \Pythiaeight agrees very well with our predictions for $\Omega_\kappa$. It is independent of $p_T^J$ and $y_J$, and has the  predicted $R$ dependence, as shown in \fig{pythiahadr}. The agreement is not as good for \Herwig, which also exhibits surprisingly little dependence on the partonic scattering process~\cite{Stewart:2014nna}.

The perturbative soft function contains a contribution due to interference between initial-state radiation (ISR) from the two beams that scales like $R^4$~\cite{Stewart:2014nna}. Current tunes do not address its potential degeneracy with MPI. As \fig{DelM1MPI} shows,
these $R^4$ contributions differ much more between tunes than their sum. They can be separated by exploiting their different $p_T^J$ dependence (see \fig{DelM1MPI}) and channel dependence. The MPI contribution has a negligible channel dependence, whereas the soft ISR is largely channel dependent and, in particular, exhibits destructive interference for $q\bar q \to Zg$.

\begin{figure}[t!]
\hfill%
\includegraphics[width=0.7\columnwidth]{DPS/Waalewijn/DelM1_pT_ISRMPI_Zq.eps}%
\hspace*{\fill}
\vspace{-2ex}
\caption{$p_T^J$ dependence of the $\sim R^4$ contributions to the jet mass moment in \Pythiaeight and \Herwig from MPI (solid lines) and soft ISR (dashed lines) for $qg\to Zq$. They can be distinguished by their $p_T^J$ dependence.
}
\label{fig:DelM1MPI}
\vspace{-3ex}
\end{figure}

\bibliography{mpi_lhc_2014_waalewijn.bib}

==> DPS/content_Summary.tex <==
\title{Outlook on theory of soft and hard MPI (DPS)}
\author{Jonathan R.~Gaunt}
\affiliation{}

\maketitle

\noindent Open issues and suggestions on what can be done with Run 2 (in addition to repeating Run 1 at higher energies):

\subsubsection*{Soft MPI, disentangling MPI and ISR/FSR}

 Soft activity accompanying some hard process can arise from several sources – perturbative and non-perturbative initial- or final-state radition, and MPI. Observables that are particularly (or only) sensitive to one of these components would be a useful tool to better understand the different components of the soft activity, and improve their modelling in Monte Carlo generators. Observables that worked well at electron-positron colliders to probe final-state radiation (including hadronisation) effects were the event shape variables, and one may think that similar variables (such as beam thrust and transverse thrust) could be useful to probe ISR/FSR in proton-proton collisions. However a recent study of Glauber gluons and their connection to MPI \cite{Gaunt:proc1} has highlighted that these observables have a strong sensitivity to soft MPI, which can formally be connected to non-cancelling Glauber exchanges between spectator partons. This sensitivity to the soft MPI can be exploited however – since the perturbative ISR/FSR component of such event shape variables is often known to high accuracy, a measurement of the event shape can be used to study the effects of the soft MPI. 

 What observables can then be used to disentangle the different components of soft radiation? An important study was performed in this direction recently, in the context of Z+jet or H+jet production \cite{Stewart:proc}. They considered the mass of the jet, and showed that the different sources of soft radiation could be disentangled via their different dependencies on jet radius, jet $p_t$, and the partonic process. Experimental measurements of these dependencies would be valuable to get a better understanding of the soft underlying event, as would further theoretical work in identifying other potentially useful observables.

\subsubsection*{Hard MPI (DPS), double parton distributions, correlations}

  Progress has been made in using constituent quark models to calculate non-perturbative properties of the double parton distributions \cite{Rinaldi:proc}. These calculations indicate that there are quite significant correlations in longitudinal momentum and quark spin, at least in the large $x$ region in which these models should be valid. Further analyses, possibly using more sophisticated models, would be very valuable in building up a more detailed picture of the non-perturbative correlations in the proton.

  Studies in which these model distributions, or other simple forms, were evolved up to higher scales using simple two-chain branching evolution, indicate that certain spin correlations (e.g. the quark-quark longitudinal spin correlation) can be non-negligible at smaller $x$ values and higher scales \cite{Rinaldi:proc, Diehl:2014vaa}. These spin correlations can manifest themselves as correlations in the final state in DPS processes. An interesting question is how these types of correlations can be investigated experimentally, especially given that an assumption that is often made to make experimental extractions of the DPS signal is that the two scatters in DPS are uncorrelated. Double open charm production offers promise in this regard, since for this process DPS dominates over SPS and any DPS correlations are more prominent. An interesting distribution in which spin correlations may be measurable is the double differential distribution of the charm quark $p_t$s \cite{Echevarria:proc}. 

 More generally, processes involving heavy quark pair production (e.g. Zcc, 4b, J/$\psi$ J/$\psi$ production at large rapidity differences) are very interesting to measure DPS, since for these the DPS/SPS ratio tends to be enhanced. Multiple production of heavy quarks in DPS takes place mainly at low $p_t$. Very valuable information could thus be obtained by identifying and measuring all heavy quarks produced in an inelastic event, with particular attention to those at low $p_t$. 

 Another interesting process is 4 jet production, which for DPS shows very different topologies as compared with SPS and NLL BFKL \cite{Maciula:proc}. Presently missing experimental information on jets widely separated in rapidity would be relevant to identify and disentangle the different production mechanisms.

 Recently much attention has been paid to the role of parton splitting mechanisms in DPS, including numerical estimations of the relative size and shape of the so called (2 $\to$ 2)$^2$ (or 2v2) and  3 $\to$ 4 (or 2v1) mechanisms \cite{Blok:proc,Gaunt:proc2}. These studies indicate that the shapes of the two contributions are rather similar, with the main effect of the  3 $\to$ 4 mechanism being to induce a mild dependence of the measured effective cross section on c.m. energy $s$ and scale $Q$. Experimental indications of this dependence would thus be very valuable. In particular, by covering larger ranges of the resolution scale than presently available, and reducing the experimental errors, it should be possible to reveal the QCD evolution effects.

 Despite recent theoretical progress in DPS, there are still problems in a consistent definition of the double parton distributions.  There are still outstanding issues related to the separation of DPS and SPS, which are linked to issues with the double parton distributions at small impact parameter. More theoretical work in this direction is needed.

Important additional information could be obtained by measuring DPS in pA interactions, where DPS are enhanced and probed in a different way as compared to pp \cite{Calucci:2013pza}. Measuring DPS in pA in addition to pp is a way to disentangle some of the multitude of correlations possible between partons in a nucleon, and gain a more detailed insight into the nucleon structure.


\begin{thebibliography}{99}
\bibitem{Gaunt:proc1}
J.~R. Gaunt, These proceedins.

\bibitem{Stewart:proc}
I.~W. Stewart, F.~J. Tackmann and W.~J. Waalewijn, These proceedings.

\bibitem{Rinaldi:proc}
M. Rinaldi, S. Scopetta, M. Traini and V. Vento, These proceedings.

%\cite{Diehl:2014vaa}
\bibitem{Diehl:2014vaa} 
  M.~Diehl, T.~Kasemets and S.~Keane,
  %``Correlations in double parton distributions: effects of evolution,''
  J. High Energy Phhys. {\bf 05}, 118 (2014) [arXiv:1401.1233 [hep-ph]].
  %%CITATION = ARXIV:1401.1233;%%
  %12 citations counted in INSPIRE as of 10 juin 2015

\bibitem{Echevarria:proc}
M.~G. Echevarria, T. Kasemets, P.~J. Mulders and C. Pisano, These proceedings.

\bibitem{Maciula:proc}
R. Maciula and A. Szczurek, These proceedings.

\bibitem{Blok:proc}
B. Blok, Yu. Dokshitzer, L. Frankfurt and M. Strikman, These proceedings.

\bibitem{Gaunt:proc2}
J.~R. Gaunt, R. Maciula and A. Szczurek, These proceedings.

%\cite{Calucci:2013pza}
\bibitem{Calucci:2013pza} 
  S.~Salvini, D.~Treleani and G.~Calucci,
  %``Double Parton Scatterings in High-Energy Proton-Nucleus Collisions and Partonic Correlations,''
  Phys.\ Rev.\ D {\bf 89}, 016020 (2014) [arXiv:1309.6201 [hep-ph]].
  %%CITATION = ARXIV:1309.6201;%%
  %9 citations counted in INSPIRE as of 10 juin 2015



\end{thebibliography}

==> HIon/Blok/content_Blok.tex <==
\title{Double parton interactions in $\gamma p, \gamma A$ collisions in the direct photon kinematics.}

\author{B.\ Blok$^{1}$,
 M.\ Strikman$^{2}$
\\[2mm] \normalsize $^1$ Department of Physics, Technion -- Israel Institute of Technology,
Haifa, Israel\\
\normalsize $^2$ Physics Department, Penn State University, University Park, PA, USA}

  \maketitle
{\em Multiple hard parton interactions}\/ (MPI) started to play an important role in the description of the inelastic $pp$ collisions at the collider energies.
Extensive theoretical studies were carried out in the last decade, both for pp collisions
 and for $pA$ collisions.
In particular it was realized that MPI in pp collisions are expressed through convolution of new objects-two parton GPD \cite{BDFS1}, and determined by the two different
mechanisms \12 and \22 (see refs. \cite{BDFS1,BDFS2,BDFS3,BDFS4} and \cite{Blok1} for details and notations.)
Presence of two mechanisms and limited knowledge of the nucleon multiparton structure makes a unique interpretation of the data rather difficult.
Hence  we proposed \cite{Blok1} to study the MPI process of
$\gamma p (A)$ interaction  with production of four jets in the kinematics where two jets carry most of the light cone fraction of the photon four momentum - direct photon mechanism. In this process the \22 mechanism is absent and the only process which contributes is
 an analog of the \12 process.Since in the proposed kinematics the contribution of the resolved photon is strongly suppressed the cross section in  the leading log approximation (LLA)  i.e. summing leading collinear singularities is expressed through the integral over  two particle GPDs,
$_2D(x_1,x_2,Q_1^2,Q_2^2,\Delta)$, introduced in \cite{BDFS1}. This is in difference from the case of $pp,pA$ scattering  where \22  contribution  is proportional to  a more complicated  integral with the integrant proportional to the  product of two double
parton GPDs.
\par Our main result is that processes with direct photon in photon proton  collisions considered in \cite{Blok1} provide  a golden opportunity for the
model independent determination of the double parton distributions $_2D$, free of the ambiguities inherent in $pp/pA$ scattering \cite{BDFS3}.
We   consider the
 process of the interaction of the
real/quasireal photon  with proton with production of
  two pairs of hard jets in the  back to back kinematics with each dijet consisting of a heavy (charm) quark and gluon jets  (see Fig. 1).
  We focus on the production of charm to suppress the contribution of the resolved photons.
   \begin{center}
 \begin{figurehere}
   \includegraphics[height=5.6cm]{HIon/Blok/photonfig1new.eps}
   \caption{  \label{kin}MPI two dijet photoproduction -$Ap$}
 \end{figurehere}
 \end{center}

In the discussed process a  $c\bar c$ pair is produced in the photon fragmentation region, while two gluon jets are created predominantly  in the target region,
so that there is a  large rapidity gap between the
gluon and quark jets. The gluon and c-quark jets are approximately balanced pair vice. The cross section of the analogous process in $pp$ collisions is influenced by parton correlations in both nucleons participating in the process,
while in the case of the photon the cross section depends only on
the integral over one wave function.
 The reason is  that the process
involves only one GPD from the nucleon, while the upper part of the diagram 1 is determined by the hard physics of the photon splitting to $Q\bar Q$ pair in an unambiguous way.
It does not  involve the scale $Q_0^2$ that separates perturbative and nonperturbative correlations in a nucleon. Thus the cross section of such a process is directly expressed through the
nucleon
 double GPD.
 Hence the measurement of the discussed cross section would allow
 to
 perform a nearly model independent analysis of
 DPI in  $pp$ scattering.


\par Here we 
 consider the MPI rates for all three types of processes mentioned above, $\gamma p, AA, pA$. We will restrict ourselves to the   kinematics $x_1,x_2>0.2$, thus guaranteeing
the dominance of the direct photon contribution (For  this cutoff the direct photons contribute 60\% of the
dijet
 cross section).
For a lower $x_i$ cutoffs the relative contribution of the direct photon mechanism  rapidly decreases for transverse momenta under consideration.

We see that for the LHeC collider  energies
$\sqrt{s}=1.3$ TeV the rate of the discussed reaction will be very high:  $2\cdot 10^9$ events per $10^7$ s (one year of running)
 for  the luminosity $10^{34}$ cm$^{-2}$s$^{-1}$ and   $p_t>5$ GeV.
The relative rate of MPI
 to dijets  is found to  be  $0.045\%$. Moreover, as it is clear from Fig. 5 below, we shall have a large MPI rate up to $p_t$ of order 17 GeV.

 A large number of events in the discussed kinematics was  produced at HERA: $\sim 1.2\cdot 10^5$
 for the total luminosity $1$ fb$^{-1}$.
  It would  be interesting to reanalyze the HERA data in the direct photon kinematics with the purpose of identifying MPI events.

Another way to observe the discussed process in the near future maybe possible - study of MPI in the  ultraperipheral $pA, AA$ processes at the full LHC energy.
For example, for $p_t>5$ GeV, we have $\sim 6\cdot 10^4$ events for $AA$, and $\sim 6.6\cdot 10^3$ events  for $pA$ scattering where we used luminosities
 $\sim 10^{27}$ ($AA$) , $10^{29}$ cm$^{-2}$s$^{-1}$ ($pA$) and running time of $10^6$ s.
In the discussed kinematics  MPI events constitute  $\sim 0.04\%$ ($\sim 0.02\%$, $\sim 0.0125\%$) of the dijet events for $AA , pA$ collisions respectively
 for the same jet cutoff. These fractions  decrease rather rapidly with $p_t$ increase.
\begin{thebibliography}{99}	
\bibitem{BDFS1}
  B.\ Blok, Yu.\ Dokshitzer, L.\ Frankfurt and M.\ Strikman,
  %``The Four jet production at LHC and Tevatron in QCD,''
  Phys.\ Rev.\  D {\bf 83}, 071501 (2011)
  [arXiv:1009.2714 [hep-ph]].
  %%CITATION = PHRVA,D83,071501;%%
  \bibitem{BDFS2} B.\ Blok, Yu.\ Dokshitser, L.\ Frankfurt and M.\ Strikman,
  %``pQCD physics of multi-parton interactions,''
  Eur.\ Phys.\ J.\ C {\bf72}, 1963  (2012)
  [arXiv:1106.5533 [hep-ph]].
  %%CITATION = ARXIV:1106.5533;%%
\bibitem{BDFS3} B.\ Blok, Yu.\ Dokshitser, L.\ Frankfurt and M.\ Strikman,
  %``Origins of parton correlations in nucleon and multi-parton collisions','
 arXiv:1206.5594v1 [hep-ph] (unpublished).
 \bibitem{BDFS4}
 B.~Blok, Y.~Dokshitzer, L.~Frankfurt and M.~Strikman,
  %``Perturbative QCD correlations in multi-parton collisions,''
  Eur.\ Phys.\ J.\ C {\bf 74} (2014) 2926
  [arXiv:1306.3763 [hep-ph]].
\bibitem{Blok1} B.~Blok and M.~Strikman,
  %``Double parton interactions in $\gamma p, \gamma A$ collisions in the direct photon kinematics,''
  Eur.\ Phys.\ J.\ C {\bf 74} (2014) 12,  3214
  [arXiv:1410.5064 [hep-ph]].
\end{thebibliography}

==> HIon/Helenius/content_helenius.tex <==
\title{Constraints for small-$x$ gluon nPDFs from p+Pb collisions at the LHC }
\author{Ilkka Helenius}
\affiliation{Department of Astronomy and Theoretical Physics, Lund University}

\maketitle

\section*{Open problems}
The current nuclear parton distribution function (nPDF) fits are mainly constrained by the deep inelastic scattering and Drell-Yan data (see e.g. ref.~\cite{Paukkunen:2014nqa} for a recent review). These data provide strong constraints for quark distributions at $x>0.01$ but gluon distributions are constrained only indirectly. Some analyses utilize also data for inclusive pion production in d+Au collisions at RHIC which provides further constraints for gluon distributions but as the kinematic reach is rather limited, the gluons remain unconstrained at $x<0.01$. 

In ref. \cite{Helenius:2014qla} we studied how the gluon nPDFs at small values of $x$ could be constrained using the p+Pb collisions at the LHC. Special emphasis were on quantifying the different regions of $x$ that are probed with inclusive hadrons and direct photons at different rapidities according to NLO pQCD. In the case of hadron production we found that due to the convolution of the partonic spectra with the fragmentation functions the relation between the partonic kinematics and the final state hadrons is significantly smeared. In addition to fragmentation mechanism the direct photons can be produced also directly at the hard scattering. The presence of this so-called prompt component makes the direct photons more sensitive to the small-$x$ physics than inclusive hadrons at the same values of transverse momentum $p_T$ and pseudorapidity $\eta$.

In addition to the nPDF studies these results can be applied also to seek for deviations from the collinear factorization based calculations. Large deviations from the pQCD predictions at certain $p_T$ and $\eta$ would hint for breaking of the factorization and the values of $x$ in which this takes place could be estimated from the presented $x$ distributions. An example of such a factorization breaking effect is the gluon saturation built into the Color-Glass-Condensate -framework, see e.g. ref.~\cite{Albacete:2013ei} for related applications

\section*{Outlook}

In order to reduce the uncertainties in the current nPDFs, measurements with better than 10\% accuracy are required. The required accuracy could be achieved by installing a forward electromagnetic calorimeter (FoCal) to the ALICE detector which have been considered as a possible upgrade of ALICE experiment \cite{T.PeitzmannfortheALICEFoCal:2013fja}. Also LHCb experiment has potential to measure electroweak cross sections in nuclear collisions at large rapidities as demonstrated e.g. in ref.~\cite{Aaij:2014pvu}. The proposed measurements at forward rapidities would serve also as a further test of factorization in nuclear collisions in a so far unexplored kinematic region.

\vspace{1mm}
\noindent Work supported by the MCnetITN FP7 Marie Curie Initial Training Network, contract
PITN-GA-2012-315877.

\begin{thebibliography}{9}

\bibitem{Paukkunen:2014nqa}
  H.~Paukkunen,
  Nucl.\ Phys.\ A {\bf 926} (2014) 24

\bibitem{Helenius:2014qla}
  I.~Helenius, K.~J.~Eskola and H.~Paukkunen,
  JHEP {\bf 1409} (2014) 138

\bibitem{Albacete:2013ei}
  J.~L.~Albacete, N.~Armesto, R.~Baier, G.~G.~Barnafoldi, J.~Barrette, S.~De, W.-T.~Deng and A.~Dumitru {\it et al.},
  Int.\ J.\ Mod.\ Phys.\ E {\bf 22} (2013) 1330007

\bibitem{T.PeitzmannfortheALICEFoCal:2013fja}
  T.~Peitzmann [ALICE Collaboration],
  arXiv:1308.2585 [physics.ins-det].

\bibitem{Aaij:2014pvu}
  R.~Aaij {\it et al.}  [LHCb Collaboration],
  JHEP {\bf 1409} (2014) 030

\end{thebibliography}




==> HIon/Klusek/content_Klusek.tex <==
\title{Double-scattering production of two $\rho^0$ mesons\\ and four pions in heavy ions UPCs}
\author{Mariola K\l{}usek-Gawenda, Antoni Szczurek}
\affiliation{Institute of Nuclear Physics Polish Academy of Sciences}

\maketitle

\section*{Open problems}
%Introduction to the problem(s).
We have calculated cross sections for double-$\rho^0$-meson
as well as four-pion production in exclusive ultraperipheral 
ultrarelativistic heavy ion collisions via a double-scattering
mechanism of single $\rho^0$ photoproduction.
The calculations have been done in the impact parameter space.
We have included the smearing of $\rho^0$ meson masses
and used the latest ALICE data %\cite{ChM_2014}
to parametrize the Breit-Wigner amplitude and the Drell-S\"oding
type continuum term. These data allows to consider
$\rho^0\rho^0$ or corresponding $\pi^+\pi^-\pi^+\pi^-$ double
photoproduction in broader range of center of mass energy of the four pion system.
Our results for single-$\rho^0$ production 
agree well with the STAR and ALICE experimental data.

%\begin{figure}[!h]
%\centering
%\includegraphics[scale=0.25]{dsig_dy_STAR.pdf}
%\includegraphics[scale=0.25]{dsig_dy_ALICE.pdf}
%\caption{Rapidity distribution of $\rho^0$ meson photoproduction
%with fixed mass (solid red lines) and with smeared mass of $\rho^0$ meson (dashed red lines)
%for gold-gold collisions at RHIC energy ($\sqrt{s_{NN}}=200$ GeV) (left panel) and
%for lead-lead collisions at LHC energy ($\sqrt{s_{NN}}=2.76$ TeV) (right panel).
%The theoretical results are compared with the STAR and ALICE data.
%}
%\label{fig:dsig_dy_data}
%\end{figure}
The produced $\rho^0$ mesons decay into charged pions, 
with almost $100\%$ probability, gives large contribution
to exclusive production of the $\pi^+\pi^-\pi^+\pi^-$ final state.
We have made a comparison of four-pion production via
$\rho^0\rho^0$ production ($\gamma\gamma$ fusion \cite{KSSz_rho}
and nuclear photoproduction \cite{KGSz_photoproduction}) with experimental data measured
by the STAR Collaboration for the AuAu$\to$AuAu$\pi^+\pi^-\pi^+\pi^-$
reaction. The theoretical predictions have similar shape
in four-pion invariant mass as the distribution measured by the
STAR Collaboration, 
but exhaust only about $20\%$ of the
measured cross section. The missing contribution
can come from excited state of $\rho^0(770)$ (e.g. $\rho^0(1700)$ resonance)
and its decay into four charged pions. 
A separation of the double-scattering, $\gamma\gamma$, $\rho^0(1450)$
and $\rho^0(1700)$ production and decay
mechanisms seems very important. In general, transverse momentum 
of each of the produced $\rho^0$'s in the double-scattering
mechanism is smaller than in the other mechanisms. 
As a consequence, the pions from the decay of $\rho^0$'s from
the double-scattering mechanism are produced dominantly back to back
in azimuthal angle. This could be used to enhance the purity
of the experimental sample as far as double-scattering
mechanism is considered. %Clearly further studies are needed.
At large rapidity separations between two
$\rho^0$'s and/or large $\pi^+\pi^+\pi^+\pi^-$ rapidity
separations, the double-scattering contribution should dominate
over other contributions. The identification of the dominance region
seems difficult, if not impossible, at RHIC.
We plan a~separate careful analysis devoted to the ALICE
experimental conditions.
It would be interesting if different mechanisms discussed
in this talk could be separated and identified experimentally. 
This requires, however, rather complicated
correlation studies for four charged pions.

\section*{Outlook}


We have concentrated on the process with
final nuclei in the ground state. It is very difficult,
if not impossible, to measure such very forward/backward
nuclei. The multiple Coulomb excitations (Ref. \cite{KGCSS_excitation}) 
associated with $\rho^0\rho^0$
production may cause additional excitation of one or even both nuclei to the
giant resonance region and subsequent emission of neutrons. 
We plan a~detailed study of these processes in the future.

\begin{thebibliography}{9}
%\bibitem{lamport94}
%  Leslie Lamport, \emph{\LaTeX: a document preparation system}. Addison Wesley, Massachusetts, 2nd edition, 1994.

%\bibitem{ChM_2014}
%Christoph Mayer, \emph{Coherent photo-production of $\rho^0$ mesons in ultra-peripheral
%Pb+Pb collisions at the LHC, measured by ALICE}. Talk given during 
%13$^{th}$ International Workshop on Meson Production, 
%Properties and Interaction KRAK\'OW, POLAND, 28.05.2014.  

\bibitem{KSSz_rho}
M. K\l{}usek-Gawenda, W. Sch\"afer and A. Szczurek,
%\emph{Exclusive production of $\rho^0 \rho^0$ pairs in $\gamma \gamma$
%collisions at RHIC},
Phys. Lett. {\bf B674} (2009) 92.
%
\bibitem{KGSz_photoproduction}
M. K\l{}usek-Gawenda and A. Szczurek,
%\emph{Double-scattering mechanism in the exclusive 
%$AA \to AA\rho^0\rho^0$ reaction in ultrarelativistic collisions},
Phys. Rev. {\bf C89} (2014) 024912.
 %     
\bibitem{KGCSS_excitation}
M. K\l{}usek-Gawenda, M. Ciema\l{}a, W. Sch\"afer and A. Szczurek,
%\emph{Electromagnetic excitation of nuclei and neutron evaporation in ultrarelativistic ultraperipheral heavy ion collisions},
Phys. Rev. {\bf C89} (2014) 054907.
\end{thebibliography}



==> HIon/Lykasov/content_Lykasov.tex <==
\title{Transverse momentum dependent gluon density at low $x$}
\author{A.A. Grinyuk$^1$, A. V. Lipatov$^{1,2}$, \underline {G. I. Lykasov$^1$},   
 N. P. Zotov$^2$}
\affiliation{$^1$ Joint Institute for Nuclear Research -
  Dubna 141980, Moscow region, Russia\\
$^2$Skobeltsyn Institute of Nuclear Physics, 
     Lomonosov Moscow State University, 119991, Moscow, Russia \\}

\maketitle

%\section{Unintegrated gluon density}
We present results on the application of the transverse momentum ${\bf k}_T$ dependent
gluon density (TMD) at low $x$, which based on our previous study \cite{GLLZ:2013}.
We match this TMD at low transverse momenta $\mid {\bf k}_T\mid$ and starting scale $Q_0^2 = 1-2$~GeV$^2$
to the exact solution of the BFKL equation outside of the saturation region at large 
$\mid {\bf k}_T\mid$ obtained in \cite{Kovch:2000}. 
%which includes all multiple Pomeron exchanges and allows us to satisfy 
%the unitarization of the DIS cross section and the structure function $F_2$.
Then, to extend this TMD at higher $Q^2$ we use the Catani-Ciafoloni-Fiorani-Marchesini (CCFM) 
evolution equation solution. 
The inclusion of the CCFM evolution results in a large increase of the TMD magnitude. 
The use of new TMD allows us to describe satisfactorily the LHC data on the heavy flavour jet
production and especially the correlation between two $b$-jets produced in $pp$ collisions
at low $x$ and large $\mid {\bf k}_T\mid$. In Fig.1 (left) the rapidity $y$ distribution 
of $b$-jets produced in the $pp$ collision at $\sqrt{s}=$8 TeV is presented. The distribution over the
difference of the azimuthal angles $\Delta\phi$ between similar two $b$-jets is presented in Fig.1(right). 

\begin{figure}[!h]

\begin{minipage}{0.47\textwidth}
\centerline{\includegraphics[width=1.0\textwidth, angle=270]{HIon/Lykasov/y_bjet_CMSe.eps}}
\end{minipage}
\hspace{0.5cm}
\begin{minipage}{0.47\textwidth}
 \centerline{\includegraphics[width=1.0\textwidth, angle=270]{HIon/Lykasov/dphi_bb_ATLASb.eps}}
\end{minipage}
   \caption{
\small The $y$-distribution of $b$-jets produced in the $pp$ collision at $\sqrt{s}=$8 TeV
compared to the CMS data \cite{CMS} (left). The distribution over the difference of the azimuthal angles 
$\Delta\phi$ between similar two $b$-jets compared to the ATLAS data \cite{ATLAS} is presented on the right. 
The solid hystograms correspond to our new TMD, whereas the dashed ones correspond to the TMD 
suggested in \cite{Hannes} (set $A0$).  }
 \label{Fig_ybjet}
\end{figure}


%\section{Summary}
\begin{thebibliography}{9}
\bibitem{GLLZ:2013}
A.A.Grinyuk, A.V.Lipatov, G.I.Lykasov, N.P. Zotov,
Phys.Rev. D{\bf 87} (2013) 074017
\bibitem{Kovch:2000}
Yuri V.Kovchegov, Phys.Rev. D{\bf 61} (2000) 074018.
\bibitem{CMS}
CMS Collaboration, JHEP 1204, 084 (2012); arXiv:1202.4617 [hep-ex]
\bibitem{ATLAS}
ATLAS Collaboration, Eur.Phys.J. C 71, 1846 (2011); arXiv:1109.6833 [hep-ex]
\bibitem{Hannes}
H.~Jung, in Proceedings of 12$^{\rm th}$ International Workshop on Deep-Inelastic 
Scattering and Related Subjects (DIS'2004), Strbske Pleso, Slovakia, April 14-18, 
2004; arXiv:0411287 [hep-ph].
%  Leslie Lamport, \emph{\LaTeX: a document preparation system}. Addison Wesley, Massachusetts, 
%  2nd edition, 1994.
\end{thebibliography}



==> HIon/Otwinowski/content_Otwinowski.tex <==
\title{Transverse momentum spectra of light-flavor hadrons measured with ALICE in pp, p--Pb and Pb--Pb collisions at the LHC}
\author{Jacek Otwinowski}
\affiliation{Institute of Nuclear Physics\\Polish Academy of Sciences}

\maketitle

\section*{Open problems}
Measurements of p--Pb collisions at the LHC has provided a lot of surprising results. In particular, so-called ridge structure was seen in two-particle correlations measured in high-multiplicity p--Pb events \cite{RidgeLHC}, which is similar to that in Pb--Pb collisions originating from collective expansion of dense medium (hydrodynamical flow).  The ridge structure modulation in azimuth is described in terms of Fourier coefficients \cite{FlowRidge}, indicating that the collective flow might develop in such system. Evidence for the flow has been further corroborated from the particle-identification measurements of the ridge \cite{IdentifiedFlow}, showing the characteristic mass ordering in $v_{2}$ vs $p_{T}$ for pions, kaons and protons. However, the measurements of the average $p_{T}$ as a function of the charged particle multiplicity \cite{ColorReconection} indicate that the collective phenomenon seen in p--Pb collisions might be due to the color reconnection. The same conclusion can be drown from the interpretation of the Blast-wave fit to the identified particle $p_{T}$ spectra \cite{BlastWave}. Moreover, the nuclear modification factors measured for charged particles \cite{RpPb} showed no suppression at high-$p_{T}$, indicating that the properties of matter produced in p--Pb and Pb--Pb collisions are different. In addition, the p--Pb system size determined using Bose-Einstein correlations of three pions \cite{Radii} is much smaller  (35-55\%) than size of the Pb--Pb system, measured at the same particle multiplicities.       

\section*{Outlook}
These findings hint at potentially novel mechanisms in collisions of small systems which are far from being understood theoretically. Several authors describe the results in the context of hydrodynamics \cite{FlowModels}, but also saturation models successfully describe some of the measurements \cite{SaturationModels}. Comparison of measurements in pp, p--Pb and Pb--Pb collisions at the same energy $\sqrt{s_{NN}}=5$~TeV, panned in 2015--2018, will help to reveal the properties of matter produced in small systems.

\begin{thebibliography}{9}
\bibitem{RidgeLHC} CMS collaboration, Phys. Lett. B 718 (2013) 795; ALICE Collaboration, Phys. Lett. B 719 (2013) 29; ATLAS Collaboration, Phys. Lett. B 725 (2013) 60. 
\bibitem{FlowRidge} CMS Collaboration, Phys. Lett. B 724 (2013) 213.
\bibitem{IdentifiedFlow} ALICE Collaboration, Phys. Lett. B 726 (2013) 164.
\bibitem{ColorReconection} ALICE Collaboration, Phys. Lett. B727 (2013) 371.
\bibitem{BlastWave} ALICE Collaboration, Phys. Lett. B 728 (2014) 25.
\bibitem{RpPb} ALICE Collaboration, Phys. Rev. Lett. 110 (2013) 082302; Eur. Phys. J. C74 (2014) 3054.
\bibitem{Radii} ALICE Collaboration, Phys. Lett. B 739 (2014) 139.
\bibitem{FlowModels} P. Bozek and W. Broniowski, Phys. Rev. C 85 (2012) 014911, Phys. Lett. B 718 (2013) 1557.
\bibitem{SaturationModels} K. Dusling and R. Venugopalan, Phys. Rev. D 87 (2013) 054014,  Phys. Rev. D 87 (2013) 094034. 
\end{thebibliography}




==> HIon/Snigirev1/content_Snigirev.tex <==
\title{DPS cross sections in
proton-nucleus and nucleus-nucleus collisions \\ at the LHC}

\author{ David~d'Enterria$^{a}$, Alexander~M.~Snigirev$^b$}
\affiliation{$^a$ CERN, PH Department, 1211 Geneva, Switzerland\\
$^b$ Skobeltsyn Institute of Nuclear Physics,\\ Moscow State University, 119991 Moscow, Russia}

\maketitle

The derivation of  simple generic expressions to compute double-parton scattering (DPS) cross sections in high-energy proton-nucleus~\cite{d'Enterria:2012qx} and nucleus-nucleus~\cite{d'Enterria:2013ck} collisions, as a function of the corresponding single-parton hard cross sections and of the event centrality, is presented. The large transverse parton density in nuclei results in a high probability of having two truly hard scatterings in p-A and A-A collisions. The DPS cross sections in p-Pb are found to be enhanced by a factor of $3A \simeq 600$ compared to those in p-p collisions at the same energy. The DPS cross sections in Pb-Pb are found to be enhanced by a factor of $A^{3.3}/5 \simeq 9 \cdot 10^6$ to be compared with the $A^2 (\simeq 4 \cdot 10^4)$ enhancement of single-parton scatterings.

The formalism was applied to estimate the DPS cross sections for quarkonium and electroweak-boson pair production in Pb-Pb and p-Pb collisions at the LHC. Table 1 collects these results~\cite{d'Enterria:2014bga,d'Enterria:2014dva}.
\begin{table}[htbp]
\renewcommand{\arraystretch}{1.3}
\begin{center}
\begin{tabular}{l|lcccccccc}\hline
System & & $J/\psi+J/\psi$ & $J/\psi+\Upsilon$ & $J/\psi$+W & $J/\psi$+Z & $\Upsilon+\Upsilon$ & $\Upsilon+$W & $\Upsilon+$Z & ss\,WW \\\hline
Pb-Pb & $\sigma$            & 210 mb & 28 mb & 500 $\mu$b & 330 $\mu$b & 960 $\mu$b & 34 $\mu$b & 23 $\mu$b & 630 nb \\
5.5 TeV & $N$ & $\sim$250 & $\sim$340 & $\sim$65 & $\sim$14 & $\sim$95 & $\sim$35 & $\sim$8 & $\sim$15 \\\hline
p-Pb & $\sigma$             & 45 $\mu$b &  5.2 $\mu$b & 120 nb & 70 nb & 150 nb & 7 nb & 4 nb & 150 pb \\
8.8 TeV & $N$ & $\sim$65 & $\sim$60 & $\sim$15 & $\sim$3 & $\sim$15 & $\sim$8 & $\sim$1.5 & $\sim$4 \\\hline
\end{tabular}
\caption{DPS production cross sections of double-$J/\psi$, $J/\psi+\Upsilon$, $J/\psi$+W, $J/\psi$+Z,
double-$\Upsilon$, $\Upsilon$+W, $\Upsilon$+Z, and  same-sign WW in Pb-Pb and p-Pb at the LHC. The
corresponding DPS yields, after (di)lepton decays and acceptance+efficiency losses, are given for
  1~nb$^{-1}$ and 1~pb$^{-1}$ respectively.}  
\label{tab:1}
\vspace{-0.5cm}
\end{center}
\end{table}
Processes such as double-$J/\psi$, $J/\psi+\Upsilon$, $J/\psi$+W, $J/\psi$+Z,
double-$\Upsilon$, $\Upsilon$+W, $\Upsilon$+Z, and  same-sign WW production have large cross sections and visible event rates for the nominal LHC luminosities. The study of such processes in p-Pb can help determine the effective nonperturbative parameter (so-called effective cross section $\sigma_{\rm eff}$) characterising the transverse parton distribution in the nucleon. Double--$J/\psi$ and double-$\Upsilon$ production in Pb-Pb provide interesting insights on the event-by-event dynamics of quarkonia in hot and dense strongly-interacting medium.

%The overall length of contribution must not exceed one page!

\begin{thebibliography}{9}
\bibitem{d'Enterria:2012qx} D.~d'Enterria,  A.M.~Snigirev, Phys.Lett. B 718 (2013) 1395; arXiv:1211.0197 [hep-ph].
\bibitem{d'Enterria:2013ck} D.~d'Enterria, A.M.~Snigirev, Phys.Lett. B 727 (2013) 157; arXiv:1301.5845 [hep-ph].
\bibitem{d'Enterria:2014bga} D.~d'Enterria, A.M.~Snigirev, Nucl. Phys. A 932 (2014) 296; arXiv:1403.2335 [hep-ph].
\bibitem{d'Enterria:2014dva} D.~d'Enterria, A.M.~Snigirev, Nucl. Phys. A 931 (2014) 303; arXiv:1408.5172 [hep-ph].
 \end{thebibliography}



==> HIon/Strikman/content_Strikman.tex <==
\title{Evidence for $x$-dependent proton
 color fluctuations \\in pA collisions at the LHC}
\author{M. Alvioli$^1$, B. A. Cole$^2$, L. Frankfurt$^3$, M. Strikman$^4$}
\maketitle
\begin{center}
$^1$ CNR-IRPI, via Madonna Alta 126, I-06128, Perugia, Italy\\
$^2$ Columbia University, New York, NY 10027, USA\\
$^3$ Tel Aviv University, Tel Aviv,  Israel\\
$^4$ 104 Davey Lab, The Pennsylvania State University, University Park, PA 16803, USA\\
\end{center}
In pA collisions at collider energies a projectile stays in a frozen 
configuration over the distances which by far exceed the nuclear diameter. 
As a result the proton coherently interacts with nucleons along its impact 
parameter. In QCD a nucleon is build of quark-gluon configurations of different transverse 
size which are expected to interact with different strength, leading to
fluctuations of the global strength of the projectile interactions. Also, 
configurations of smaller size are expected to have a reduced gluon field 
leading to a correlation of soft and hard interactions. To describe these
effects it is convenient to introduce a probability distribution for the projectile
to interact with strength $\sigma$, $P_N(\sigma)$. $P_N(\sigma)$ is strongly
constrained by the diffractive $pp$ data, the behavior  of $P_N$ for $\sigma\to 0$
expected in pQCD, etc \cite{Heiselberg:1991is}. We developed a Monte Carlo procedure
to describe these effects in soft collisions and collisions with a hard
trigger taking into account the difference of the transverse scales of hard and soft
interactions  \cite{Alvioli:2013vk,Alvioli:2014sba}. The prediction that the distribution
over the number of wounded nucleons should be broader than the Glauber
model expectation was confirmed at the LHC \cite{TheATLAScollaboration:2013cja}.
We argue that the violation of the Glauber approximation
for the dependence  of the rate of forward jet production on centrality observed in $pA$
collisions at the LHC provides the first experimental evidence that parton configurations
in the projectile proton containing a parton with large $x_p$ interact with a nuclear target
with a significantly smaller than average cross section, and have smaller than average size.
Implementing effects of such fluctuations of the interaction strengths and using the ATLAS
analysis \cite{TheATLAScollaboration:2013cja} of the dependence of  the hadron production at backward rapidities on the number
of wounded nucleons, we make quantitative predictions for the centrality dependence of the
jet production rate as a function of the interaction strength $\sigma(x_p)$. For $x_p=0.6$
we find $\sigma(x_p)\sim \sigma_{tot}(pp)/2$ \cite{Alvioli:2014eda} which has implications
on the origin of the EMC effect. Future studies of  dijet production along these lines would
allow to investigate the global 3D structure of the nucleon and to trigger on particular
configurations which interact with a larger-than-average strenght.
 %
\begin{thebibliography}{9}
 %
\bibitem{Heiselberg:1991is} 
  H.~Heiselberg, G.~Baym, B.~Blaettel, L.~L.~Frankfurt and M.~Strikman,
  %``Color transparency, color opacity, and fluctuations in nuclear collisions,''
  Phys.\ Rev.\ Lett.\  {\bf 67}, 2946 (1991); Phys.\ Rev.\ C {\bf 52}, 1604 (1995)
 %
\bibitem{Alvioli:2013vk} 
  M.~Alvioli and M.~Strikman,
  %``Color fluctuation effects in proton-nucleus collisions,''
  Phys.\ Lett.\ B {\bf 722}, 347 (2013)
  %[arXiv:1301.0728 [hep-ph]].
  %
\bibitem{Alvioli:2014sba} 
  M.~Alvioli, L.~Frankfurt, V.~Guzey and M.~Strikman,
  %``Revealing ÒflickeringÓ of the interaction strength in pA collisions at the CERN LHC,''
  Phys.\ Rev.\ C {\bf 90}, no. 3, 034914 (2014)
  %[arXiv:1402.2868 [hep-ph]].
  %
\bibitem{TheATLAScollaboration:2013cja} 
  The ATLAS collaboration,
  %``Measurement of the centrality dependence of the charged particle pseudorapidity distribution in proton-lead collisions at $\sqrt{s_{NN}} = 5.02$ TeV with the ATLAS detector,''
  ATLAS-CONF-2013-096, ATLAS-COM-CONF-2013-117,
  %%CITATION = ATLAS-CONF-2013-096, ATLAS-COM-CONF-2013-117;%%
  %22 citations counted in INSPIRE as of 09 Jan 2015
  https://cds.cern.ch/record/1599773.
  %
\bibitem{Alvioli:2014eda} 
  M.~Alvioli, B.~Cole, L.~Frankfurt and M.~Strikman,
  %``Evidence for x-dependent proton color fluctuations in pA collisions at the LHC,''
  arXiv:1409.7381 [hep-ph]. 
  %
\end{thebibliography}
   


==> HIon/content_Summary.tex <==
\title{Outlook on MPI and the Heavy Ions}
\author{P. Bartalini}
\affiliation{}
\maketitle


This brand new working group deals with the interplays between the MPI and the Heavy Ions research lines. 

The LHC RUN I highlights in this field include the unexpected observation of long-range, near-side angular correlations in small systems (i.e. pp and pPb collisions) \cite{ref1,ref2} as well as the systematic studies of high multiplicity events, the latter pointing to a fundamental role of rather soft MPI in driving the final states with large multiplicities: the ALICE event shape analysis [Eur.Phys.J. C72 (2012) 2124] demonstrates that these events look more spherical than predicted by the general purpose QCD models, disfavoring the presence of well-pronounced jet structures. This is basically confirmed by the CMS analysis focusing on the study of jets and Underlying Event (UE) activity in large multiplicity events \cite{ref3}. ALICE also launched a systematic investigation of event yields versus charged multiplicity, Nch, \cite{ref4} that - at least in pp - corroborates the trivial picture in which Nch and all the event yields are proportional to the number of MPI. In pPb, the observed discrepancies to this rule, point to the need of improving the centrality determination in these asymmetric interactions \cite{ref5}; this requires a strict collaboration between experimentalist and theorist [M. Strikman, this proceedings].

Progress in Run 2 is expected by the adoption of large multiplicity triggers at low luminosity: as far as pPb interactions are concerned all the experiments are expected to improve while only ALICE will take large low luminosity pp samples at 13 TeV, ending up with at least one million of events with average multiplicity of one order of magnitude higher than the minimum bias average. Progress should also arise from the adoption of new experimental techniques that allow separating jetty from not jetty events using the event shapes \cite{ref6}. Possible variations of the hadro-chemistry in large multiplicity events should be investigated in detail; alternative explanations to this flow-like phenomenon may be provided by MPI models with color reconnections [G. Paic, 5th MPI@LHC]. A significant progress in understanding flow-like effects in small systems with large multiplicities in the final states is expected by the adoption of models describing MPI in an homogeneous way in both pp and pPb interactions [C. Bierlich, this proceedings].

A lot of emphasis has been put in the possible observation of the double parton scattering (DPS) in pPb events [D. Treleani, 5th MPI@LHC and most of the theoretical contributions in this section of the proceedings]. Indeed Ð due to anti-shadowing effects - the DPS signal/background ratios in pPb are expected to be enhanced with respect to the corresponding final states in pp. However one needs to be very careful in taking into account the LHC luminosity figures: in the LHC RUN I all the LHC experiments got around 10 nb-1 at centre-of-mass energies per nucleon pair of 5.02TeV; given the current constraints, the RUN II plans are to collect data at the same energy integrating a significantly higher statistics that in any case will not go beyond 100 nb-1. This means that the DPS measurements in pPb should select final states with large cross section; the significant pp progress [arXiv:1410.6664 and DPS section of these proceedings] suggests to focus on final states with multiple heavy flavors production. 

\begin{thebibliography}{99}
\bibitem{ref1} CMS Collaboration, JHEP {\bf 1009} (2010) 091. 
\bibitem{ref2} CMS Collaboration, Phys. Lett. B {\bf 718} (2013) 795.
\bibitem{ref3} ALICE Collaboration, Eur. Phys. J. C{\bf 72} (2012) 2124.
\bibitem{ref4} ALICE Collaboration, Phys. Lett. B {\bf 712} (2012) 165.
\bibitem{ref5} ALICE Collaboration, http://arxiv.org/abs/1412.6828.
\bibitem{ref6} E. Cuautle, A. Ortiz, G. Paic, http://arxiv.org/abs/1412.6828.

\end{thebibliography}

==> HIon/content_Summary2.tex <==
\title{Outlook on MPI and the Heavy Ions}
\author{P. Bartalini}
\affiliation{}
\maketitle


This brand new working group deals with the interplays between the MPI and the Heavy Ions research lines. 

The LHC RUN I highlights in this field include the unexpected observation of long-range, near-side angular correlations in small systems (i.e. pp and pPb collisions) \cite{ref1,ref2} as well as the systematic studies of high multiplicity events, the latter pointing to a fundamental role of rather soft MPI in driving the final states with large multiplicities: the ALICE event shape analysis [Eur.Phys.J. C72 (2012) 2124] demonstrates that these events look more spherical than predicted by the general purpose QCD models, disfavoring the presence of well-pronounced jet structures. This is basically confirmed by the CMS analysis focusing on the study of jets and Underlying Event (UE) activity in large multiplicity events \cite{ref3}. ALICE also launched a systematic investigation of event yields versus charged multiplicity, Nch, \cite{ref4} that - at least in pp - corroborates the trivial picture in which Nch and all the event yields are proportional to the number of MPI. In pPb, the observed discrepancies to this rule, point to the need of improving the centrality determination in these asymmetric interactions \cite{ref5}; this requires a strict collaboration between experimentalist and theorist [M. Strikman, this proceedings]. 

Progress in Run 2 is expected by the adoption of large multiplicity triggers at low luminosity: as far as pPb interactions are concerned all the experiments are expected to improve while only ALICE will take large low luminosity pp samples at 13 TeV, ending up with at least one million of events with average multiplicity of one order of magnitude higher than the minimum bias average. Progress should also arise from the adoption of new experimental techniques that allow separating jetty from not jetty events using the event shapes \cite{ref6}. Possible variations of the hadro-chemistry in large multiplicity events should be investigated in detail; alternative explanations to this flow-like phenomenon may be provided by MPI models with color reconnections [G. Paic, 5th MPI@LHC]. A significant progress in understanding flow-like effects in small systems with large multiplicities in the final states is expected by the adoption of models describing MPI in an homogeneous way in both pp and pPb interactions [C. Bierlich, this proceedings].

A lot of emphasis has been put in the possible observation of the double parton scattering (DPS) in pPb events [D. Treleani, 5th MPI@LHC and most of the theoretical contributions in this section of the proceedings]. Indeed Ð due to anti-shadowing effects - the DPS signal/background ratios in pPb are expected to be enhanced with respect to the corresponding final states in pp. However one needs to be very careful in taking into account the LHC luminosity figures: in the LHC RUN I all the LHC experiments got around 10 nb-1 at centre-of-mass energies per nucleon pair of 5.02TeV; given the current constraints, the RUN II plans are to collect data at the same energy integrating a significantly higher statistics that in any case will not go beyond 100 nb-1. This means that the DPS measurements in pPb should select final states with large cross section; the significant pp progress [arXiv:1410.6664 and DPS section of these proceedings] suggests to focus on final states with multiple heavy flavors production. 

% ----------------------------------------------------------------------------
\begin{thebibliography}{99}
\bibitem{ref1} CMS Collaboration, JHEP {\bf 1009} (2010) 091. 
\bibitem{ref2} CMS Collaboration, Phys. Lett. B {\bf 718} (2013) 795.
\bibitem{ref3} ALICE Collaboration, Eur. Phys. J. C{\bf 72} (2012) 2124.
\bibitem{ref4} ALICE Collaboration, Phys. Lett. B {\bf 712} (2012) 165.
\bibitem{ref5} ALICE Collaboration, http://arxiv.org/abs/1412.6828.
\bibitem{ref6} E. Cuautle, A. Ortiz, G. Paic, http://arxiv.org/abs/1412.6828.

\end{thebibliography}
% ----------------------------------------------------------------------------



==> HIon/snigirev2/content.tex <==
\title{Towards correlations
in double parton distributions}

\author{Alexander Snigirev$^{a}$, Nina Snigireva$^{b}$, Gennady Zinovjev$^{c}$}
\affiliation{$^{a}$Skobeltsyn Institute of Nuclear Physics,\\Lomonosov Moscow State University, 119991, Moscow, Russia\\
$^{b}$School of Mathematical Sciences,\\ University College Dublin, Belfield, Dublin 4, Ireland \\$^{c}$Bogolyubov Institute for Theoretical Physics, \\ National Academy of Sciences of Ukraine,  03680 Kiev-143, Ukraine}


\maketitle

The basic properties of double parton distribution functions (dPDFs) are reviewed in the framework of perturbative QCD in the collinear approximation.
The initial state of double parton scattering (DPS) is coded by dPDFs which quantify the joint distribution of two partons in a hadron, depending on their quantum numbers,  longitudinal momentum fractions and the relative transverse distance between them.
The dPDFs and the corresponding evolution equations are well-known only  integrated over the parton pair transverse separation in the collinear approximation.
The particular solutions  of these non-homogeneous equations may be presented in form of a convolution of single distributions  (which coincides with jet calculus rules proposed originally for the fragmentation functions).
They contribute to the inclusive cross section of DPS with a larger weight (different effective cross section) being compared to the solutions of homogeneous equations.  The latter solutions are usually approximated by factorized form if initial nonperturbative correlations are absent.

Using the explicit form of the solutions of evolution equations in the Mellin representation we demonstrate~\cite{Snigirev:2014eua} analytically that the dPDFs "forget" the initial correlation conditions (unknown {\it a priori}) at not parametrically small longitudinal momentum fractions $x_1$ and $x_2$, and the correlations perturbatively calculated survive only in the limit of large enough hard scales. Such a dominance is the mathematical consequence of the relation between the maximum eigenvalues $\Lambda(n)$ in the moments representation, ~$\Lambda(n_1+n_2)~>~\Lambda(n_1)+\Lambda(n_2)$, in QCD at large $n_1$ and $n_2$ (finite $x_1$ and $x_2$). It is independent of the strength of the initial correlation conditions at all. The numerical estimates (done by integrating directly the evolution equations) testify in favour of conclusion also that the perturbative correlation effects are significant in the kinematical region accessible in experimental measurements at energies of Tevatron and LHC.

Unlike naively accepted expectations, the QCD dynamical perturbative correlations result effectively in the dependence of the experimentally extracted effective cross section of DPS on the resolution scale. The measurements covering a larger range of the resolution scale variation might reveal the evolution effects more distinctly in accordance with the asymptotic QCD behaviour.

%The overall length of contribution must not exceed one page!

\begin{thebibliography}{9}
\bibitem{Snigirev:2014eua}
A.M.~Snigirev, N.A.~Snigireva, G.M.~Zinovjev, Phys. Rev. D {\bf 90}, 014015 (2014); arXiv:1403.6947 [hep-ph].
 \end{thebibliography}



==> Org/org.tex <==
\newpage
 \thispagestyle{empty}
%\pagestyle{plain}
\normalsize
{\Huge{\bf Organizing Committee}} \\
\vskip1.5cm

{\Large \underline{International Advisory Board}}\\
\vskip1mm
\noindent Paolo Bartalini - China Central Normal University\\
Jonathan Butterworth - UC London\\
Markus Diehl - DESY\\
Livio Fanò - University of Perugia, INFN\\
Rickard Field - University of Florida\\
Hannes Jung - DESY, University of Antwerp\\
Judith Katzy - DESY\\
Frank Krauss - IPPP Durham\\
Krzysztof Kutak - IFJ PAN Krakow\\
Stefano Lami - CERN\\
Michelangelo Mangano - CERN\\
Arthur Moraes - Centro Brasileiro de Pesquisas Físicas\\
Andreas Morsch - CERN\\
Zoltan Nagy - DESY\\
Giulia Pancheri - INFN Frascati Nat. Lab.\\
Michael Schmelling - MPIK Heidelberg\\
Torbjorn Sjöstrand - Lund University\\
Peter Skands - CERN, Monash University\\
Mark Strikman - Pennsylvania State University\\
Antoni Szczurek - IFJ PAN Krakow\\
Daniele Treleani - INFN Trieste\\
Pierre van Mechelen - University of Antwerp\\
Nick van Remortel - University of Antwerp

\vskip1.5cm
{\Large \underline{Local Organising Committee}}\\
\vskip1mm

\noindent Krzysztof Kutak (chair)\\
Antoni Szczurek (chair)\\
Rafał Maciu{\l}a\\
Rafał Staszewski\\
Maciej Trzebi{\'n}ski

\vskip+30mm

\begin{flushleft}
\underline{Editors}:\\
K. Kutak, R. Maciu{\l}a, A.~M. Moraes, and A. Szczurek\\
June 2015, Krakow
\end{flushleft}


\newpage
 \thispagestyle{empty}
%\pagestyle{plain}
\normalsize
{\Huge{\bf List of Authors}} \\
\vskip1.5cm

R. Astalos (Comenius University, Bratislava), S. Baranov (Russian Academy of Sciences), P. Bartalini (Central China Normal University CCNU), I. Belyaev (Institute for Theoretical And Experimental Physics, Moscow), Ch. Bierlich (Lund University), B. Blok (Technion, Israel), A. Buckley (University of Glasgow), F.~A. Ceccopieri (Universite de Liege), I. Cherednikov (University of Antwerp), J.~R. Christiansen (Lund University), D. Ciangottini (CERN/INFN), M. Deak (IFIC/CSIC, Universitat de Valencia), B. Ducloue (University of Jyvaskyla), R. Field (University of Florida), J.~R. Gaunt (DESY, Hamburg), K. Golec-Biernat (IFJ PAN, Krakow/Rzeszow University), L. Goerlich (IFJ PAN, Krakow),  A. Grebenyuk (Université Libre De Bruxelles), O. Gueta (Tel Aviv University), P. Gunnellini (DESY, Hamburg/Universiteit Antwerpen), I. Helenius (Lund University), H. Jung (DESY, Hamburg), D. Kar (University of Glasgow), O. Kepka (Acad. of Sciences of the Czech Rep.), M. K{\l}usek-Gawenda (IFJ PAN, Krakow), A. Knutsson (University of Antwerp), P. Kotko (Penn State University), M.~W. Krasny (Univ. Paris VI), K. Kutak (IFJ PAN, Krakow), E. Lewandowska (IFJ PAN, Krakow), G. Lykasov (Joint Institute for Nuclear Research, Dubna), R. Maciu{\l}a (IFJ PAN, Krakow), A.~M. Moraes (Brazilian Center for Physics Research), T. Martin (University of Warwick), G. Mitsuka (Universita e INFN), L. Motyka (Jagiellonian University), M. Myska (CTU, Prague), J. Otwinowski (IFJ PAN, Krakow), T. Pierog (KIT/IKP), V. Pleskot (Charles University in Prague), M. Rinaldi (INFN, Perugia), W. Sch\"afer (IFJ PAN, Krakow), A. Siodmok (CERN/IFJ PAN, Krakow), T. Sj{\"o}strand (Lund Univeristy), A. Snigirev (SINP MSU), A. Sta{\'s}to (Penn State University/IFJ PAN, Krakow), R. Staszewski (IFJ PAN, Krakow), T. Stebel (Jagiellonian University), M. Strikman (Penn State University), A. Szczurek (IFJ PAN, Krakow/Rzeszów University), D. Treleani (University of Trieste), M. Trzebi{\'n}ski (IFJ PAN, Krakow), H. van~Haevermaet (DESY, Hamburg/University of Antwerp), A. van~Hameren (IFJ PAN, Krakow), P. van~Mechelen (University of Antwerp), W. Waalewijn (University of Amsterdam/Nikhef), W.~Y. Wang (National University of Singapore),


%\newpage
% \thispagestyle{empty}
%\pagestyle{plain}
%\normalsize
%{\Huge{\bf List of Participants}} \\
%\vskip1.5cm

%R. Astalos (Comenius University, Bratislava), S. Baranov (Russian Academy of Sciences), P. Bartalini (Central China Normal University CCNU), I. Belyaev (Institute for %Theoretical And Experimental Physics, Moscow), Ch. Bierlich (Lund University), B. Blok (Technion, Israel), A. Buckley (University of Glasgow), A. Bursche (Universitaet %Zuerich), S. Camarda (DESY, Hamburg), F.~A. Ceccopieri (Universite de Liege), I. Cherednikov (University of Antwerp), J.~R. Christiansen (Lund University), J. Chwastowski %(IFJ PAN, Krakow), D. Ciangottini (CERN/INFN), M. Deak (IFIC/CSIC, Universitat de Valencia), B. Ducloue (University of Jyvaskyla), L. Fano (INFN, Perugia), R. Field %(University of Florida), L. Forthomme (Universite catholique de Louvain), J.~R. Gaunt (DESY, Hamburg), K. Golec-Biernat (IFJ PAN, Krakow/Rzeszow University), L. Gorlich %(IFJ PAN, Krakow), J. Grados Luyando (DESY, Hamburg), A. Grebenyuk (Université Libre De Bruxelles), O. Gueta (Tel Aviv University), P. Gunnellini (DESY, %Hamburg/Universiteit Antwerpen), I. Helenius (Lund University), C. Jeske (University of Warwick), H. Jung (DESY, Hamburg), D. Kar (University of Glasgow), T. Kasemets %(University of Amsterdam/Nikhef), O. Kepka (Acad. of Sciences of the Czech Rep.), M. K{\l}usek-Gawenda (IFJ PAN, Krakow), A. Knutsson (University of Antwerp), P. Kotko %(Penn State University), M.~W. Krasny (Univ. Paris VI), K. Kutak (IFJ PAN, Krakow), E. Lewandowska (IFJ PAN, Krakow), M. {\L}uszczak (Rzeszow University), G. Lykasov (Joint %Institute for Nuclear Research, Dubna), R. Maciu{\l}a (IFJ PAN, Krakow), A.~M. Moraes (Brazilian Center for Physics Research), T. Martin (University of Warwick), G. Mitsuka %(Universita e INFN), L. Motyka (Jagiellonian University), M. Myska (CTU, Prague), S. Ostapchenko (Frankfurt Institute for Advanced Studies), J. Otwinowski (IFJ PAN, %Krakow), T. Pierog (KIT/IKP), V. Pleskot (Charles University in Prague), M. Prasza{\l}owicz (Jagiellonian University), P. Puzo (Université Paris Sud), W. P{\l}aczek %(Jagiellonian University), M. Rinaldi (INFN, Perugia), A. Rybicki (IFJ PAN, Krakow), W. Sch\"afer (IFJ PAN, Krakow), M. Serino (IFJ PAN, Krakow), A. Siodmok (CERN/IFJ PAN, %Krakow), T. Sj{\"o}strand (Lund Univeristy), A. Snigirev (SINP MSU), I. Sputowska (IFJ PAN, Krakow), A. Sta{\'s}to (Penn State University/IFJ PAN, Krakow), R. Staszewski %(IFJ PAN, Krakow), T. Stebel (Jagiellonian University), M. Strikman (Penn State University), A. Szczurek (IFJ PAN, Krakow/Rzeszów University), T. Szumlak (AGH - UST, %Krakow), D. Treleani (University of Trieste), M. Trzebi{\'n}ski (IFJ PAN, Krakow), H. van~Haevermaet (DESY, Hamburg/University of Antwerp), A. van~Hameren (IFJ PAN, %Krakow), P. van~Mechelen (University of Antwerp), L. van~Lindern (Max-Planck-Gesellschaft), W. Waalewijn (University of Amsterdam/Nikhef), W.~Y. Wang (National University %of Singapore), K. Zapp (CERN)

==> Preface/Introduction_original.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Short Sectioned Assignment
% LaTeX Template
% Version 1.0 (5/5/12)
%
% This template has been downloaded from:
% http://www.LaTeXTemplates.com
%
% Original author:
% Frits Wenneker (http://www.howtotex.com)
%
% License:
% CC BY-NC-SA 3.0 (http://creativecommons.org/licenses/by-nc-sa/3.0/)
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%----------------------------------------------------------------------------------------
%	PACKAGES AND OTHER DOCUMENT CONFIGURATIONS
%----------------------------------------------------------------------------------------



\title{	
\normalfont \normalsize 
\textsc{$6^{th}$ International Workshop on Multiple Partonic Interactions at the LHC - MPI@LHC2014} \\ [25pt] % Your university, school and/or department name(s)
\horrule{0.5pt} \\[0.4cm] % Thin top horizontal rule
\huge Preface \\ % The assignment title
\horrule{2pt} \\[0.5cm] % Thick bottom horizontal rule
}

\author{Arthur Moraes} % Your name

\date{\normalsize\today} % Today's date or a custom date

%----------------------------------------------------------------------------------------

\begin{document}

\maketitle % Print the title

%\section{Problem title}

The Sixth International Workshop on Multiple Partonic Interactions at the Large Hadron Collider 
(MPI@LHC2014) took place at the Polish Academy of Arts and Sciences (PAU) in Krak\'{o}w, 
from 3 to 7 November 2014.

MPI are often crucial for interpreting results obtained at the Large Hadron Collider (LHC). 
The quest for a sound understanding of the dynamics behind MPI - particularly at this time when the LHC 
is due to start its "Run II" operations - has focused the aim of this workshop. 
MPI@LHC2014 concentrated mainly on the phenomenology of LHC measurements whilst keeping 
in perspective those results obtained at previous hadron colliders.  The workshop has also debated some of the 
\textit{state-of-the-art} theoretical considerations and the modeling of MPI in Monte Carlo event generators.

The topics debated in the workshop included:
\begin{itemize}
\item
Phenomenology of MPI processes and multiparton distributions;
\item
Considerations for the description of MPI in Quantum Chromodynamics (QCD);
\item
Measuring multiple partonic interactions;
\item
Experimental results on inelastic hadronic collisions: underlying event, minimum bias, forward energy flow;
\item
Monte Carlo generator development and tuning;
\item
Connections with low-x phenomena, diffraction, heavy-ion physics and cosmic rays.
\end{itemize}

In a total of 57 plenary talks the workshop covered a wide range of experimental results, 
Monte Carlo development and tuning, phenomenology and dedicated measurements of 
MPI which were produced with data from the LHC's Run I. 
Recent progress of theoretical understanding of MPI in pp, pA and AA collisions as well as 
the role of MPI in diffraction and small-x physics were also covered. 
Two discussion sessions focused on \textit{Double Parton Scattering and the Underlying Event} and on 
\textit{Small-x and Collisions with Nuclei} were also held at the workshop and debated how the lessons 
learned from the LHC Run I analyses could help the community to plan ahead for the incoming Run II.

The workshop forstered close contact between the experimental and theoretical communities. 
It provided a setting to discuss many of the different aspects of MPI, eventually identifying them as a 
unifying concept between apparently different lines of research and evaluating their impact on the LHC 
physics programme. 
 
We want to thank the International Advisory Board for the MPI@LHC Workshop Series and the Working 
Group Conveners who contributed so effectively to the preparation of an interesting and successful scientific 
program for the workshop. We must also express our deepest gratitude to our sponsors: Institute of Nuclear 
Physics - Polish Academy of Sciences; National Science Centre - Poland;  Krakow to business - KRK>2B.
It is also a pleasure to thank the Local Organising Committee, Krzysztof Kutak (chair), Antoni Szczurek (chair), 
Rafal Maciula, Rafal Staszewski, Maciej Trzebinski and Jolanta Mosurek for their tireless work before and 
during the workshop. 

In the following, the reader will find summary reports of plenary talks presented at the workshop. 
These contributions are organized in "chapters" corresponding to the working groups which 
were part of the scientific program.  

All the presentations are available at: \textit{https://indico.cern.ch/event/305160/overview} .
\vspace{2cm}
\begin{flushright} 
\textit{Arthur M. Moraes} 
\end{flushright}

\end{document}



==> Preface/preface.tex <==
\newpage
\pagestyle{plain}
\addcontentsline{toc}{section}{\textbf{Preface}}
\normalsize
{\Huge{\bf Preface}} \\
\vskip0.5cm
The Sixth International Workshop on Multiple Partonic Interactions at the Large Hadron Collider 
(MPI@LHC2014) took place at the Polish Academy of Arts and Sciences (PAU) in Krak\'{o}w, 
from 3 to 7 November 2014.

MPI are often crucial for interpreting results obtained at the Large Hadron Collider (LHC). 
The quest for a sound understanding of the dynamics behind MPI - particularly at this time when the LHC 
is due to start its "Run II" operations - has focused the aim of this workshop. 
MPI@LHC2014 concentrated mainly on the phenomenology of LHC measurements whilst keeping 
in perspective those results obtained at previous hadron colliders.  The workshop has also debated some of the 
\textit{state-of-the-art} theoretical considerations and the modeling of MPI in Monte Carlo event generators.

The topics debated in the workshop included:
\begin{itemize}
\item
Phenomenology of MPI processes and multiparton distributions;
\item
Considerations for the description of MPI in Quantum Chromodynamics (QCD);
\item
Measuring multiple partonic interactions;
\item
Experimental results on inelastic hadronic collisions: underlying event, minimum bias, forward energy flow;
\item
Monte Carlo generator development and tuning;
\item
Connections with low-x phenomena, diffraction, heavy-ion physics and cosmic rays.
\end{itemize}

In a total of 57 plenary talks the workshop covered a wide range of experimental results, 
Monte Carlo development and tuning, phenomenology and dedicated measurements of 
MPI which were produced with data from the LHC's Run I. 
Recent progress of theoretical understanding of MPI in pp, pA and AA collisions as well as 
the role of MPI in diffraction and small-x physics were also covered. 
Two discussion sessions focused on \textit{Double Parton Scattering and the Underlying Event} and on 
\textit{Small-x and Collisions with Nuclei} were also held at the workshop and debated how the lessons 
learned from the LHC Run I analyses could help the community to plan ahead for the incoming Run II.

The workshop forstered close contact between the experimental and theoretical communities. 
It provided a setting to discuss many of the different aspects of MPI, eventually identifying them as a 
unifying concept between apparently different lines of research and evaluating their impact on the LHC 
physics programme. 
 
We want to thank the International Advisory Board for the MPI@LHC Workshop Series and the Working 
Group Conveners who contributed so effectively to the preparation of an interesting and successful scientific 
program for the workshop. We must also express our deepest gratitude to our sponsors: Institute of Nuclear 
Physics - Polish Academy of Sciences; National Science Centre - Poland;  Krakow to business - KRK>2B.
It is also a pleasure to thank the Local Organising Committee, Krzysztof Kutak (chair), Antoni Szczurek (chair), 
Rafal Maciula, Rafal Staszewski, Maciej Trzebinski and Jolanta Mosurek for their tireless work before and 
during the workshop. 

In the following, the reader will find summary reports of plenary talks presented at the workshop. 
These contributions are organized in "chapters" corresponding to the working groups which 
were part of the scientific program.  

All the presentations are available at: \textit{https://indico.cern.ch/event/305160/overview} .
\vspace{1cm}
\begin{flushright} 
\textit{Arthur M. Moraes} 
\end{flushright}


==> Summary/summary.tex <==
\newpage
 \thispagestyle{empty}
\pagestyle{plain}
%\addcontentsline{toc}{chapter}{\textbf{Summary and Conclusions}}
\normalsize
{\Huge{\bf Summary and Conclusions}} \\
\vskip0.5cm

The Sixth International Workshop on Multiple Partonic Interactions at the Large Hadron Collider 
(MPI@LHC2014) is the latest installment of a series of very successful workshops dedicated to the   
understanding of the dynamics behind Multiple Partonic Interactions (MPI). 
As in previous editions of the MPI@LHC series, the quest for an improved description of the dynamics 
behind MPI has focused the aim of this workshop. 

Once again, the workshop provided an unique setting that promoted active interaction between the 
experimental and theoretical communities. 
It encouraged the discussion of many of the different aspects of MPI, identified common concepts 
between apparently different lines of research and evaluated the impact of MPI on the LHC 
physics program. 

The experimental collaborations have reported on measurements that show evidence 
of MPI effects in pp, pA and AA collisions. These effects can be noticed in several scenarios defined experimentally, 
such as minimum bias and underlying event measurements in pp collisions, as well as in many observables inspired by the 
phenomenology of MPI for pp, pA and AA collisions. 
At the heart of the experimental discussion were the recent advances on direct measurements 
of double-parton scattering (DPS) and on strategies to extract $\sigma_{eff}$ with the aid of 
phenomenology models implemented in Monte Carlo (MC) generators. 
It is also noticeable that there has been a growing interest on studies which look for MPI effects in events with topologies 
characterized by forward particle production and/or rapidity gaps. 

The workshop has also debated some of the modern theoretical considerations and the modeling of 
MPI in MC event generators.
Theoretical studies on unintegrated PDFs, double parton distribution functions, double parton cross-section 
predictions, electroweak boson production in DPS, correlations in particle pair productions and final state 
topologies with forward tagged particles, jets and/or rapidity gaps are just some examples of the work that has 
been presented at the workshop.
It is also worth mentioning that since the first meeting of this workshop series, there have been many advances on 
MC generator development and tuning which originated from discussions held at the MPI@LHC workshops - this edition included 
- and are now part of a recognizable legacy of these meetings. 

Looking ahead to 2015 we can only be very excited with the possibilities the restart of LHC will bring to the MPI
community. The Run II of the LHC is expected to deliver data on proton-proton collisions at a centre-of-mass energy of 
13 TeV as well as new collisions at high energies with heavy ions. 
In this context of being confronted with the dawning of a new era while still harvesting many lessons from the LHC Run I 
cycle, the workshop participants have debated and agreed on a few points we should document here for future reference 
when we reconvene in 2015. These include:
\begin{itemize}
\item
Experimental collaborations are strongly encouraged to define a set of "common measurements" with event selection and 
kinematic cuts which can be performed by as many experiments as possible. Minimum bias and underlying event measurements
are key targets for this exercise. The set of common measurements produced with Run I data and documented in the "Minimum 
bias and Underlying Event Working Group of the LPCC"\footnote{The LHC Physics Center at CERN (LPCC) - Minimum Bias \& 
Underlying Event Working Group. Documentation and plots for the common measurements produced with the LHC's Run I data 
is available at this web-address: \textit{http://lpcc.web.cern.ch/LPCC/index.php?page=mb\_ue\_wg\_docs}} 
has been identified as a starting point which will be proposed to the experiments. 
\item
It is also recommended that a common MC tuning should be used as a reference by the experimental collaborations, the MC
authors and users who will be developing new models or tunings. The PYTHIA8 - Monash\footnote{P. Skands, S. Carrazza, 
J. Rojo, Eur. Phys. J. C 74 (8) (2014) 3024.} tune was chosen as the MC tune to be used as 
the reference.  
\item
Isolating the DPS signal at the LHC remais quite challenging and usually implies on the reliance of model dependent 
corrections in order to interpret the measurements. 
There is a need to re-think the observables used to perform a direct measurement of DPS at the LHC. 
It is also recommended that, where possible, experimental collaborations seek to use consistent (if not common) definitions of 
phase-space selection cuts and background templates. 
\item
The range of experimental scenarios traditionally investigated in the search for MPI has been broadened.
MPI is relevant for measurements done with data collected from pp, pA and AA collisions. 
Recent theory studies indicate that stronger experimental signatures of DPS in pp collisions are predicted to 
be observed in topologies which include final states with forward tagged particles, forward jets and/or rapidity gaps. 
It is also recommended that for pp, pA and AA collisions, new analyses on high-multiplicity final states, jet activity rates, 
correlations in particle pair production (double open charm, J/$\Psi$ pair and electroweak boson pair, to mention a few) should be 
further pursued with the LHC's Run II data.
\end{itemize}

Many other advances and open problems were reported at the workshop and the reader 
will certainly have found these described in the various contributions collected in these proceedings.

In 2015, the 7$^{th}$ International Workshop on Multiple Partonic Interactions  at the LHC - MPI@LHC2015 - will be 
hosted by  the Intenational Centre for Theoretical Physics, in Trieste, Italy. 
On behalf of the International Advisory Board for the MPI@LHC Workshop Series I would like to invite all those interested in advances on MPI to come and join us at the next edition of this workshop. 
We look forward to meeting all our MPI friends at Trieste. 
The year 2015 promises to bring us many new results and very interesting physics indeed!
\vspace{1cm}

\begin{flushright} 
\textit{Arthur M. Moraes} 
\\
\textit{Chairman of the International Advisory Board for the MPI@LHC Workshop Series} 
\end{flushright}

\clearpage

==> UE/Astalos/content_Astalos.tex <==
\title{Measurements of event shapes and particle production with the ATLAS detector}
\author{R\'obert Astalo\v{s}\\\vspace{0.1cm}
{\small on behalf of the ATLAS Collaboration}}
\affiliation{Comenius University Bratislava, Radboud University Nijmegen}

\maketitle

Measurements of event shapes and production properties of mesons and baryons at 7 TeV proton-proton collisions data taken by the ATLAS detector\cite{atlas} in 2010 are presented.

The evolution of the event shape variables, such as the transverse thrust, thrust minor and transverse sphericity has been studied for minimum bias events as functions of the $p_\mathrm{T}$ of the leading 
particle in an event\cite{event_shapes}. With increasing $p_\mathrm{T}^{\rm lead}$ a shift to less spherical events is observed. This effect is more profound in case of the transverse sphericity than 
for the other event shape variables. All MC models considered tend to reproduce data better for higher $p_{\rm T}^{\rm lead}$ ranges. Among them the 
Pythia 6 tune Z1 which was tuned to Underlying Event at LHC agrees best with data. The dependence of the mean values of the event shape variables on a charged-particle 
transverse momentum scalar sum of the event shows an increse followed by a decrease. For all MC models considered, this decrease occurs before that of the data (see left plot of 
Fig.~\ref{fig:1} for case of the transverse sphericity mean value). Furthermore, all MC models predict less high-sphericity events than seen in the data.

The differential production cross section of the $\phi$(1020)-meson has been studied using the $\phi\rightarrow K^+K^-$ decay mode\cite{phi_meson}. The integrated $\phi$-meson production cross 
section in this fiducial range ($500 < p_{\mathrm{T},\phi} < 1200$ MeV, $|y_\phi|<0.8$) is measured to be 
$\sigma_\phi\times BR(\phi\rightarrow K^+K^-)=570\pm8$~(stat) $\pm$ 68 (syst) $\pm$ 20 (lumi) $\mu$b. The cross section has also 
been studied as a function of the transverse momentum $p_{\mathrm{T},\phi}$ (right plot of Fig.~\ref{fig:1}) and rapidity $|y_\phi|$ and was found to be in best agreement with 
the predictions of the MC generator tunes EPOS-LHC and Pythia 6 DW.

The transverse polarization of $\Lambda$ and ${\bar \Lambda}$ hyperons produced in minimum bias events has been measured to be 
$P_\Lambda$ = - 0.010 $\pm$ 0.005~(stat) $\pm$ 0.004~(syst) and $P_{\bar \Lambda}$ = 0.002 $\pm$ 0.006~(stat) $\pm$ 0.004~(syst). In bins of $p_\mathrm{T}$ 
and Feynman-$x$ variable, polarization is found to be less than 2\% and is consistent with zero within estimated uncertainties as predicted by the Standard Model.


\begin{figure}[h]
\includegraphics[width=0.39\linewidth]{UE/Astalos/fig1.eps}
\hspace{0.5cm}
\includegraphics[width=0.35\linewidth]{UE/Astalos/fig2.eps}

\caption{Mean value of the transverse sphericity as a function of charged-particle transverse momentum scalar sum of the event (left) and the $\phi(1020)\rightarrow K^+K^-$ 
cross section as a function of the transverse momentum $p_{\mathrm{T},\phi}$ (right). The error bars represent the statistical uncertainty 
and the green boxes represent the combined statistical and systematic uncertainty.
\label{fig:1}}
\end{figure}
\vspace{-0.85cm}

\begin{thebibliography}{9}
\bibitem{atlas} ATLAS Collaboration, JINST 3 (2008) S08003
\bibitem{event_shapes}  ATLAS Collaboration, Phys. Rev. D 88, 032004 (2013) [arXiv:1207.6915]
\bibitem{phi_meson} ATLAS Collaboration, Eur. Phys. J. C (2014) 74:2895 [arXiv:1402.6162]
\end{thebibliography}


==> UE/Buckley/content_Buckley.tex <==
\title{ATLAS Pythia\,8 tunes to 7\,\TeV~data}
\author{Andy Buckley, on behalf of the ATLAS collaboration}
\affiliation{School of Physics \& Astronomy, University of Glasgow, UK}

\maketitle

\section*{Summary}

The main Monte Carlo (MC) event generators in use at the LHC apply models of
parton showers, hadronisation and multiple partonic interactions, augmenting
fixed-order matrix element events into simulations very similar to real collider
data. But the approximations inherent in these models introduce parameters into
the modelling, which are fixed by ``tuning'' to data
~\cite{Buckley:2011ms}.

I presented the two most recent ATLAS collaboration~\cite{Aad:2008zzm} tunes for the Pythia$\,$8
generator~\cite{Sjostrand:2007gs}: the AZ/AZNLO tunes for optimal description of
the low-end of the $Z$-boson $\pt$ spectrum~\cite{ATL-PHYS-PUB-2013-017} with
standalone \& \textsc{Powheg}~\cite{Alioli:2010xd} matrix elements; and the A14
general-purpose high-$\pt$ tunes for standalone
Pythia$\,$8~\cite{ATL-PHYS-PUB-2014-021}. Both these tune sets were created using
the Rivet~\cite{Buckley:2010ar} MC analysis system and the
Professor~\cite{Buckley:2009bj} MC tuning tools.

The AZ(NLO) tunes were constructed specifically to describe the experimental $Z$
$\pt$ data better than achievable with fixed-order or analytically-resummed
calculations -- this is an important systematic in $W$ mass measurement. Only
the Pythia primordial $\kt$ smearing parameter and initial state parton shower
cutoff were tuned, the effects of these parameters being important for very
low-$\pt$ recoil modelling but virtually irrelevant for other observables. In the
case of AZNLO, the crucial developments were in the basic configuration: use of
the \textsc{Powheg} per-event \kbd{SCALUP} variable as the starting scale of the
initial-state parton shower, and raising the \textsc{Powheg} emission cutoff to
give Pythia control over the lowest-$\pt$ shower emissions. The standalone tune
describes the $Z$ $\pt$ spectrum between 1--100$\;\GeV$ within 2\% of the data,
while the \textsc{Powheg} tune is within 5\% of the data for the same $\pt(Z)$
range.

Cross-checks indicate that the AZ tunes are largely viable for use as general
purpose tunes, albeit with a rough MPI description. But for general-purpose MC
generation a true global tune is preferred. ATLAS' standalone Pythia$\,$8 "A14"
tunes have been created for that purpose, using a large tuning space of ten
parameters from the parton shower and MPI models, plus the LO hard-process
$\aS$. The tunes were independently constructed for the four most recent LO PDFs
from the NNPDF, CTEQ, MSTW, and HERA fitting
groups~\cite{Ball:2012cx,Pumplin:2002vw,Martin:2009iq,Sarkar:2014zua}, serving
as a test of PDF impact and a consistency check on tune stability. All relevant
\& available observables from ATLAS' Run~1 data-taking were used, including
measurements in QCD jet production, $Z$ production, and $\ttbar$ production
processes. Cuts were placed on the tuned ranges of these observables to avoid
regions where multi-jet emission dominates. Pythia$\,$8's damped shower setup was
used for $\ttbar$ showering; this setting was found crucial to describe $\ttbar$
event jet veto observables and reduce tensions between datasets.

The resulting A14 tunes show remarkable consistence between the optimal $\aS$
values in initial- and final-state parton showers. Variation between PDFs are
small, except in the MPI parameters, as expected. The strength of colour
reconnection is also consistent between the four tunes. A set of five
variation-tune pairs have also been created, using the ``eigentune'' method, to
provide a covering set of tunes for various modelling and tuning
systematics. The A14 tunes are principally intended for use in LO modelling of
fairly high-$\pt$ processes, but may also be useful for showering of NLO and
multi-leg events.
% given that non-specialist shower tunes have previously been used for this
% purpose.


\section*{Open problems}

The main open problem in MC tunes for high-$\pt$ process modelling is that there
is no clear path to a generator configuration suitable for use in LO, LO
multi-leg, and NLO hard process showering. A well-defined ME/PS matching scheme
is a crucial prerequisite for this, and this does not yet exist for the
\textsc{Powheg} matching.
% and NLO matching schemes more similar to the CKKW/MLM approaches for LO
% matching may be more compatible with LO tunes.
Whether it is possible to create NLO tunes which can be used for example in both
\textsc{Powheg}~\cite{Alioli:2010xd} and \textsc{aMC@NLO}~\cite{Alwall:2014hca},
and across many process types is still an open question.

On the softer side of tuning, the A14 tune provides very good global description
of high-$\pt$ phenomena but at the cost of finding a final-state shower $\aS$ rather
different than that found in tunes to LEP event shapes and differential jet
rates only. The A14 performance on LEP observables needs to be investigated.
The softest and most forward physics also continues to pose the toughest challenges:
modelling of fiducial minimum bias observables and their connection to total
cross-sections remains rather poor, and it seems reasonable to first aim for progress
in that modelling area before aiming for consistent do-everything tunes.

Finally, the big question in soft-QCD tuning before LHC Run~2 is obviously the
level of underlying event and pile-up backgrounds at 13$\;\TeV$. The A14 tunes do
not address that issue but have been constructed with decoupled energy
extrapolation so that adjustment can be made without any effect at 7$\;\TeV$.  The
spread of model predictions at 13$\;\TeV$ is rather small, but surprises can
always happen!

% Given the availability of comprehensive Pythia\,8 tunes like A14, AMBT2,
% Monash~\cite{Skands:2014pea}, and CMS' offerings, a fairly robust prediction
% is expected\dots


\section*{Outlook}

More ATLAS tune studies are in progress for description of minimum-bias \&
forward physics (for pile-up modelling), and for use with NLO/multi-leg matrix
element events. Tuning of Sherpa and Herwig++ is also planned. A rapid MPI
MC/data study and possible retuning is expected in response to data from the
early LHC Run~2 run with a low rates of pile-up.


\begin{thebibliography}{99}

\bibitem{Aad:2008zzm}
  %G.~Aad {\it et al.}
  ATLAS Collaboration,
  %``The ATLAS Experiment at the CERN Large Hadron Collider,''
  JINST {\bf 3} (2008) S08003.
  %%CITATION = JINST,3,S08003;%%
  %3130 citations counted in INSPIRE as of 05 Dec 2014

\bibitem{Buckley:2011ms}
  A.~Buckley, J.~Butterworth, S.~Gieseke, D.~Grellscheid, S.~Hoche, H.~Hoeth, F.~Krauss and L.~Lonnblad {\it et al.},
  %``General-purpose event generators for LHC physics,''
  Phys.\ Rept.\  {\bf 504} (2011) 145
  [arXiv:1101.2599 [hep-ph]].
  %%CITATION = ARXIV:1101.2599;%%
  %190 citations counted in INSPIRE as of 03 Dec 2014

\bibitem{Sjostrand:2007gs}
  T.~Sjostrand, S.~Mrenna and P.~Z.~Skands,
  %``A Brief Introduction to PYTHIA 8.1,''
  Comput.\ Phys.\ Commun.\  {\bf 178} (2008) 852
  [arXiv:0710.3820 [hep-ph]].
  %%CITATION = ARXIV:0710.3820;%%
  %1390 citations counted in INSPIRE as of 03 Dec 2014

\bibitem{ATL-PHYS-PUB-2013-017}
  ATLAS Collab.,
  ATL-PHYS-PUB-2013-017,
  %``Example ATLAS tunes of Pythia8, Pythia6 and Powheg to an observable sensitive to $Z$ boson transverse momentum,''
  % Nov 2013,
  \url{http://cds.cern.ch/record/1629317/}

\bibitem{Alioli:2010xd}
  S.~Alioli, P.~Nason, C.~Oleari and E.~Re,
  %``A general framework for implementing NLO calculations in shower Monte Carlo programs: the POWHEG BOX,''
  JHEP {\bf 1006} (2010) 043
  [arXiv:1002.2581 [hep-ph]].
  %%CITATION = ARXIV:1002.2581;%%
  %576 citations counted in INSPIRE as of 03 Dec 2014

\bibitem{ATL-PHYS-PUB-2014-021}
  ATLAS Collab., ATL-PHYS-PUB-2014-021,
  %``ATLAS Run 1 Pythia8 tunes},''
  % Nov 2014,
  \url{https://cds.cern.ch/record/1966419/}

\bibitem{Buckley:2010ar}
  A.~Buckley, J.~Butterworth, L.~Lonnblad, D.~Grellscheid, H.~Hoeth, J.~Monk, H.~Schulz and F.~Siegert,
  %``Rivet user manual,''
  Comput.\ Phys.\ Commun.\  {\bf 184} (2013) 2803
  [arXiv:1003.0694 [hep-ph]].
  %%CITATION = ARXIV:1003.0694;%%
  %155 citations counted in INSPIRE as of 03 Dec 2014

\bibitem{Buckley:2009bj}
  A.~Buckley, H.~Hoeth, H.~Lacker, H.~Schulz and J.~E.~von Seggern,
  %``Systematic event generator tuning for the LHC,''
  Eur.\ Phys.\ J.\ C {\bf 65} (2010) 331
  [arXiv:0907.2973 [hep-ph]].
  %%CITATION = ARXIV:0907.2973;%%
  %163 citations counted in INSPIRE as of 03 Dec 2014

\bibitem{Ball:2012cx}
  R.~D.~Ball, V.~Bertone, S.~Carrazza, C.~S.~Deans, L.~Del Debbio, S.~Forte, A.~Guffanti and N.~P.~Hartland {\it et al.},
  %``Parton distributions with LHC data,''
  Nucl.\ Phys.\ B {\bf 867} (2013) 244
  [arXiv:1207.1303 [hep-ph]].
  %%CITATION = ARXIV:1207.1303;%%
  %233 citations counted in INSPIRE as of 03 Dec 2014

\bibitem{Pumplin:2002vw}
  J.~Pumplin, D.~R.~Stump, J.~Huston, H.~L.~Lai, P.~M.~Nadolsky and W.~K.~Tung,
  %``New generation of parton distributions with uncertainties from global QCD analysis,''
  JHEP {\bf 0207} (2002) 012
  [hep-ph/0201195].
  %%CITATION = HEP-PH/0201195;%%
  %4189 citations counted in INSPIRE as of 03 Dec 2014

\bibitem{Martin:2009iq}
  A.~D.~Martin, W.~J.~Stirling, R.~S.~Thorne and G.~Watt,
  %``Parton distributions for the LHC,''
  Eur.\ Phys.\ J.\ C {\bf 63} (2009) 189.
  %%CITATION = ARXIV:0901.0002;%%
  %2431 citations counted in INSPIRE as of 03 Dec 2014

\bibitem{Sarkar:2014zua}
  A.~M.~Cooper-Sarkar,
  %``HERAPDF1.5LO PDF Set with Experimental Uncertainties,''
  PoS DIS {\bf 2014} (2014) 032.
  %%CITATION = POSCI,DIS2014,032;%%

% \bibitem{Skands:2014pea}
%   P.~Skands, S.~Carrazza and J.~Rojo,
%   %``Tuning PYTHIA 8.1: the Monash 2013 Tune,''
%   Eur.\ Phys.\ J.\ C {\bf 74} (2014) 8,  3024
%   [arXiv:1404.5630 [hep-ph]].
%   %%CITATION = ARXIV:1404.5630;%%
%   %10 citations counted in INSPIRE as of 03 Dec 2014

\bibitem{Alwall:2014hca}
  J.~Alwall, R.~Frederix, S.~Frixione, V.~Hirschi, F.~Maltoni, O.~Mattelaer, H.-S.~Shao and T.~Stelzer {\it et al.},
  %``The automated computation of tree-level and next-to-leading order differential cross sections, and their matching to parton shower simulations,''
  JHEP {\bf 1407} (2014) 079
  [arXiv:1405.0301 [hep-ph]].
  %%CITATION = ARXIV:1405.0301;%%
  %137 citations counted in INSPIRE as of 03 Dec 2014

\end{thebibliography}


==> UE/Christiansen/content_Christiansen.tex <==
\title{A new Colour Reconnection model in PYTHIA}
\author{Jesper Roy Christiansen\footnote{Work supported by the MCnetITN FP7 Marie Curie Initial Training Network, contract PITN-GA-2012-315877.}$^,$\footnote{In collaboration with Peter Skands.}}


\affiliation{Department of Astronomy and Theoretical Physics \\ Lund University}

\maketitle

The recent renewal of interest in colour reconnection (CR) at LHC is due to 
two observations: the model prediction for baryon production does not match 
the data (Fig.~\ref{fig:lambda}), and the CR uncertainty on the top mass has 
become one of the larger 
uncertainties. The last point was discussed in more detail 
in Torbj\"orn Sj\"ostrand's talk.
\\ \\
\noindent The new CR model (implemented in PYTHIA) builds on two main physics ideas:
 \begin{itemize}
 \item  It uses the colour rules from SU(3) to determine which reconnections 
 are allowed. Especially, the epsilon structure of the SU(3) group is also 
 included, allowing the creation of junction structures (and thereby 
 additional baryons).
 \item  The $\lambda$-measure is used to determine which of the allowed colour configurations is chosen. Only reconnection which lowers the total string length (the $\lambda$-measure) is considered and thereby a local minimization is achieved.
 \end{itemize} 
A new beam remnant model following similar principles was also introduced in PYTHIA.
\begin{figure}[ht]
\begin{minipage}{0.48\textwidth}
By tuning the amount of junction structures, the baryon production 
can be described simultaneously at both LEP and LHC (Fig.~\ref{fig:lambda}). Other 
models (also presented at this conference) describe the baryon production 
as well, however. All the models rely on the higher colour/energy density of LHC to
provide the additional baryons needed, but the method to obtain them varies. 
A natural continuation is therefore to consider additional 
observables especially sensitive to the higher densities. One suggestion 
is to study the baryon production as a function of the multiplicity. 
With the correlation between multiplicity and energy/colour density, 
this observable can both probe the regime dominated by the new models as 
well as their onsets.
\end{minipage} \hspace{0.02\textwidth}
\begin{minipage}{0.48\textwidth}
  \centering
  \includegraphics[width=0.95\textwidth]{UE/Christiansen/test.eps}
  \centering
  \vspace{-10pt}
  \caption{\label{fig:lambda}The $\Lambda / K_s^0$ $p_\perp$-distribution as recorded by the CMS collaboration~\cite{lambda}}
\end{minipage}
\end{figure}

Other suggested observables include the $\langle p_\perp \rangle$  vs mass, where the standard PYTHIA can not describe the slope even at lower centre-of-mass energies~\cite{star}. A corresponding measurement at LHC energies could shed light on its relation to energy/colour densities.

\begin{thebibliography}{9}
\bibitem{lambda}
  CMS collaboration, \emph{Strange Particle Production in $pp$ Collisions at $\sqrt{s}=0.9$ and 7 TeV}, JHEP 1105 (2011) 064 [arXiv:1102.4282 [hep-ph]]
\bibitem{star}
 STAR collaboration, \emph{Strange Particle production in p+p collisions at $\sqrt{s} = 200$ GeV},
Phys. Rev. C75 (2007) 064901 [nucl-ex/0607033]
\end{thebibliography}



==> UE/Field/content_Field.tex <==
\title{CMS UE and MB Tunes}
\author{Rick Field}
\affiliation{University of Florida\\ \textit{For the CMS Collaboration}}

\maketitle

\section*{Summary}
Just before the shutdown of the Tevatron, CDF collected about 12 million ``Min-Bias" (MB) collisions at 
$300\gev$ and about $54$ million MB collisions at $900\gev$ (the ``Tevatron Energy Scan").  
CDF ``underlying event" (UE) measurements at $300\gev$, $900\gev$, and $1.96\tev$ when combined with LHC 
measurements allow for a detailed study of the energy dependence of the UE.  The CMS Physics Comparisons \& Generator Tunes 
group have used the CDF data together with CMS UE measurements $7\tev$ to produce the following PYTHIA tunes \cite{cms1}: 

\begin{itemize}
\item
PYTHIA $6$ Tune CUETP6S1-CTEQ6L: Start with Tune Z$2^\star$-lep and tune to the CDF UE data at $300\gev$, $900\gev$, and $1.96\tev$ 
and the CMS UE data at $7\tev$. Improved version of Tune Z$2^\star$-lep using the CTEQ6L structure functions.
\item
PYTHIA $8$ Tune CUETP8S1-CTEQ6L: Start with Tune 4C \cite{tune4c} and tune to the CDF UE data at $900\gev$ and $1.96\tev$ 
and the CMS UE data at $7\tev$. Improved version of Tune 4C using the CTEQ6L structure function.
\item
PYTHIA 8 Tune CUETP8S1-HERALOPDF: Start with Tune 4C and tune to the CDF UE data at $900\gev$ and $1.96\tev$ 
and the CMS UE data at $7\tev$. Improved version of  Tune 4C using the HERAPDF1.5LO structure function.
\item
PYTHIA 8 Tune CUETP8M1-NNPDF2.3LO: Start with the Peter Skands Monash Tune \cite{monash} and tune to the CDF UE data 
at $900\gev$ and $1.96\tev$ and the CMS UE data at $7\tev$. Improved version of the Monash Tune using 
the NNPDF2.3LO structure function.
\end{itemize}

The CDF $300\gev$ UE data are excluded from the PYTHIA $8$ tunes becase we are unable to get a good fit to all 
four energies with PYTHIA $8$.  However, these PYTHIA $8$ tunes fit the UE data at $900\gev$, $1.96\gev$, and $7\tev$ 
very well.  The PYTHIA $6$ tune fits all four energies fairly well.  We have extrapolated these tunes to $13\tev$.  
The three PYTHIA $8$ tunes give almost identical predictions at $13\tev$.  The  PYTHIA $6$ tune gives almost the 
same predictions at $13\tev$. Are focus has been on the energy dependence of the UE and making precise predictions 
at $13\tev$.  We expect the early LHC UE data at $13\tev$ to agree closely with the predictions of these tunes.

We have studied the preductions of these tunes for the energy and particle flow in the forward region 
($|\eta| >4$).  Both the original Monash tune and the CMS Tune CUETP8M1-NNPDF2.3LO agree better with the 
CMS-TOTEM data in the forward region than tunes with other structure functions.  The low $x$ behavior of 
the NNPDF2.3LO gluon distribution results in more energy in the forward forward region than the other structure functions.  
One can increase the low $x$ gluon distribution of the the HERAPDF1.5LO structure function and improve the fits to the 
forward region.  These modifications are in the region $x <\approx 10^{-5}$ and are below the HERA data.  There is a 
bit of freedom to tune the low $x$ gluon distribution to improve the fits to collider data, but in doing so one has to 
carefully examine all the Monte-Carlo model parameters that might also affect the forward region.

\section*{Open problems}
\begin{itemize}
\item
We do not understand why our PYTHIA $6$ tune fits the CDF $300\gev$ UE data better than our PYTHIA $8$ tunes.
\item
We do not yet know if it makes sense to tune the low $x$ gluon distribution to improve the fit to collider data in the forward region.  
One must first carefully study all the QCD Monte-Carlo model parameters that might affect the forward region.  Tuning the PDF 
should be the last resort. 
\end{itemize}

\section*{Outlook}
I expect many interesting QCD Monte-Carlo model comparisons with the early Run $2$ LHC data.  It should be a very exciting year.

\begin{thebibliography}{9}
\bibitem{cms1}
 \textit{Underlying Event Tunes and Double Parton Scattering}, CMS Collaboration, CMS PAS GEN-14-001.
\bibitem{tune4c}
\textit{Interleaved Parton Showers and Tuning Prospects}, R. Corke, T. Sj\"ostrand, J. High Energy Phys. 1103:032 (2011), arXiv:1011.1759 [hep-ph].
\bibitem{monash}
\textit{Tuning PYTHIA 8.1: the Monash 2013 Tune}, P. Skands, S. Carrazza, J. Rojo, Eur. Phys. J. C74 (2014) 8, 3024, arXiv:1404.5630 [hep-ph].


\end{thebibliography}



==> UE/Mitsuka/content.tex <==
\title{Measurements of forward neutron and neutral pion productions with the LHCf detector}
\author{Gaku Mitsuka}
\affiliation{University of Florence and INFN Firenze}

\maketitle

\section{Energy and transverse-momentum spectra in forward region}

The Large Hadron Collider forward (LHCf) experiment has been designed to measure
the hadronic production cross sections of neutral particles emitted in very
forward angles, including zero degrees, in proton-proton ($p$--$p$) and
proton-lead ($p$--Pb) collisions at the LHC.

Figures~\ref{fig:pi0} show the energy and transverse momentum ($\pt$)
distribution for inclusive neutral pions in very forward rapidity region has
been measured with the LHCf detector in $p$--$p$ collisions at $\sqs = \tev{7}$
at the LHC.
The both spectra contain the recent analysis extension to the \textit{Type-II}
$\pizero$ events, which consist of two photons entering either of two
calorimeters (see the presentation at the workshop).

\begin{figure}[htbp]
  \centering
  \includegraphics[width=4.2cm, keepaspectratio]{./pT_E.pdf}
  \includegraphics[width=4.2cm, keepaspectratio]{./pi0pt.pdf}
  \caption{(Left) Energy spectrum of $\pizero$'s at $y>8.6$ and $\pt<\gev{0.2}$.
  (Right) $\pt$ spectrum of $\pizero$'s at $8.6<y<8.8$.}
  \label{fig:pi0}
\end{figure}

Figures~\ref{fig:neutron} shows the energy spectra measured with the LHCf
detector. The experimental results indicate that the highest neutron production
rate occurs at the most forward rapidity range ($\eta > 10.76$) compared with
the hadronic interaction models. {\sc qgsjet} II-03 predicts a neutron
production rate compatible with the experimental result at the most forward
rapidity.

\begin{figure*}[htbp]
  \centering
  \includegraphics[width=13cm,keepaspectratio]{./neutron.pdf}
  \caption{Energy spectra of neutrons obtained with the LHCf detector.}
  \label{fig:neutron}
  \centering
\end{figure*}

\section{Discussions}

There exist several proposals (by A. Szczurek, M. Strikman, and S.
Ostapchenko) to extend the LHCf capabilities to the diffractive event ragging
and investigation of impact-parameter-dependent energy spectra which can be
realized with a help of the ATLAS detector and a correlation between two LHCf
detectors.


==> UE/Mitsuka/content_Mitsuka.tex <==
\title{Measurements of forward neutron and neutral pion productions with the LHCf detector}
\author{Gaku Mitsuka}
\affiliation{University of Florence and INFN Firenze}

\maketitle

\section*{Energy and transverse-momentum spectra in forward region}

The Large Hadron Collider forward (LHCf) experiment has been designed to measure
the hadronic production cross sections of neutral particles emitted in very
forward angles, including zero degrees, in proton-proton ($p$--$p$) and
proton-lead ($p$--Pb) collisions at the LHC.

Figures~\ref{fig:pi0} show the energy and transverse momentum ($\pt$)
distribution for inclusive neutral pions in very forward rapidity region has
been measured with the LHCf detector in $p$--$p$ collisions at $\sqs = \tev{7}$
at the LHC.
The both spectra contain the recent analysis extension to the \textit{Type-II}
$\pizero$ events, which consist of two photons entering either of two
calorimeters (see the presentation at the workshop).

\begin{figure}[htbp]
  \centering
  \includegraphics[width=4.2cm, keepaspectratio]{UE/Mitsuka/mit2.eps}
  \includegraphics[width=4.2cm, keepaspectratio]{UE/Mitsuka/mit1.eps}
  \caption{(Left) Energy spectrum of $\pizero$'s at $y>8.6$ and $\pt<\gev{0.2}$.
  (Right) $\pt$ spectrum of $\pizero$'s at $8.6<y<8.8$.}
  \label{fig:pi0}
\end{figure}

Figures~\ref{fig:neutron} shows the energy spectra measured with the LHCf
detector. The experimental results indicate that the highest neutron production
rate occurs at the most forward rapidity range ($\eta > 10.76$) compared with
the hadronic interaction models. {\sc qgsjet} II-03 predicts a neutron
production rate compatible with the experimental result at the most forward
rapidity.

\begin{figure*}[htbp]
  \centering
  \includegraphics[width=13cm,keepaspectratio]{UE/Mitsuka/neutron.eps}
  \caption{Energy spectra of neutrons obtained with the LHCf detector.}
  \label{fig:neutron}
  \centering
\end{figure*}

\section*{Discussions}

There exist several proposals (by A. Szczurek, M. Strikman, and S.
Ostapchenko) to extend the LHCf capabilities to the diffractive event ragging
and investigation of impact-parameter-dependent energy spectra which can be
realized with a help of the ATLAS detector and a correlation between two LHCf
detectors.


==> UE/Myska/content_Myska.tex <==
\title{Improving the forward rapidity gap description in Herwig++}
\author{Miroslav Myska$^{*1}$, Jonathan Da Silva$^{2}$, Michael H. Seymour$^{2}$, Andrzej Si\'odmok$^{3}$}
\affiliation{
\begin{tabular}{l}
$^{*}$ Speaker\\
$^{1}$ FNSPE, Czech Technical University in Prague\\
$^{2}$ School of Physics and Astronomy, University of Manchester\\
$^{3}$ Physics Department, CERN\\
\end{tabular}
}

\maketitle


Herwig++ \cite{Bahr:2008pv} is a general-purpose Monte Carlo event generator for lepton and hadron collisions
and it is successful in many directions, including standard underlying event measurements at the Tevatron and the LHC. 
However, Herwig++ did not turn out to correctly describe the forward rapidity gap ($\Delta\eta^{F}$) measurement \cite{Aad:2012pw}.
$\Delta\eta^{F}$ is defined as the largest pseudorapidity difference between the most forward particle detected 
and the edge of the acceptance of the detector. Our investigation deals
only with the non-diffractive component of the $\Delta\eta^{F}$ distribution, which should reach 
its maximum at $\Delta\eta^{F}$ $\rightarrow$ 0 and should fall exponentially down. 
However, Herwig++ produces large amount of events with very large gaps.

%and it aims for a good description of a widest range of processes as possible. For a specific precision, Herwig++
%allows to incorporate a different evaluation of matrix elements and provides an additional event construction steps, commonly 
%called as underlying event. Among others, this includes the modeling of multiple parton interactions (MPI), evolution of initial and 
%final state partons and cluster hadronization. Herwig++ is 

Since the minimal threshold on the transverse momentum of the measured particles was set to 200 MeV, 
a very simple color-less minimum bias matrix element has to be used. 
It scatters mostly valence quarks in the direction very close to the remaining proton remnants.
The rest of the particle population in the event is produced through the soft 
remnant-remnant scattering, which is included in the eikonal model of MPI \cite{Borozan:2002fk}. 
In this model, the soft MPI proceeds effectively as a gluon scattering, whose multiplicity is determined 
according to the Poisson distribution. It reflects the measured total cross section and the calculated hard
cross section for the given settings. In fact, the generation mechanism models
the outgoing gluons in the 2$\rightarrow$4-like process, where two initial remnants change their momenta and emit two gluons,
each collinear with its remnant. Herwig++ assigns the longitudinal fractional momentum as well as the transverse momentum to these gluons
according to the predefined distributions. Both distributions are desired to be similar to the ones known from the perturbative 
scattering and thus the model fulfills the consistency requirements between hard and soft production. 
%The model also requires to be as 
%simple as possible relying only on the necessary number of tunable parameters but also flexible in accommodating new phenomena.

It has been found that the oversimplified assignment of color charges to the outgoing gluons and proton remnants
causes the rapidity gap mismodeling. Originally, the model introduced two color connections 
between the gluons scattered in the opposite direction assuming that such arrangement will sufficiently populate the phase space.
The situation was slightly generalized by introducing the color disrupt probability parameter disconnecting 
these gluons completely and connecting each of them to its remnant. The new model presented at the workshop is motivated by
the mentioned consistency requirement and it implements the color connections among soft gluons and remnants  
as in the case of QCD interaction. There are two possible arrangements of color connections.
There can be a color line between the two outgoing remnants or a color line between a remnant and a gluon outgoing in the opposite direction.

Results for the $\Delta\eta^{F}$ distribution are now fully in agreement with the expected shape for 
the non-diffractive events. However, these results are obtained with the color reconnection mechanism turned off.
Since this mechanism has been proven to be very useful, it will have to be improved
to adopt the minimum bias measurements. One of the possibility is to introduce the space-time dependence of color
reconnection algorithm which would conserve the effective amount of color connections all over the $\eta$ space.


\begin{thebibliography}{9}
\bibitem{Bahr:2008pv}
  M. Bahr \textit{et al.}, %\emph{Herwig++ Physics and Manual}, 
  Eur. Phys. J. C \textbf{58} (2008) 639.
  
\bibitem{Aad:2012pw}
  ATLAS Collaboration, %\emph{Rapidity gap cross sections measured with the ATLAS detector in $pp$ collisions at $\sqrt{s}=7$ TeV}, 
  Eur. Phys. J. C \textbf{72} (2012) 1926.
%\bibitem{CMS-PAS-FSQ-12-005}
  %CMS Collaboration, %\emph{Measurement of diffraction dissociation cross sections at sqrt(s)=7 TeV at the LHC}, 
  %CMS-PAS-FSQ-12-005.
\bibitem{Borozan:2002fk}
  I. Borozan and M. H. Seymour, %\emph{An eikonal model for multiparticle production in hadron-hadron interactions}, 
  JHEP \textbf{0209} (2002) 015.

\end{thebibliography}



==> UE/Pierog/content_Pierog.tex <==
\title{Underlying events in EPOS 3.1xx}
\author{Tanguy Pierog}
\affiliation{Karlsruhe Institute of Technology (KIT), Campus North, Karlsruhe, Germany}

\maketitle

\section*{Open problems}
The measurement of underlying event activity has been initiated by the CDF collaboration more than ten years ago~\cite{Affolder:2001xt} to understand multiple parton interaction and test the capability of the event generators to reproduce real events. This analysis has been generalized to more recent collider data including the main LHC experiment ATLAS~\cite{Aad:2010fh} and CMS~\cite{Chatrchyan:2011id}. With the minimum bias hadronic interaction model EPOS~LHC~\cite{Pierog:2013ria} (dashed line), data are well reproduce below $5~GeV/c$ (Fig.~\ref{simu} right) with an active core producing collective flow but the description was not so good above $10~GeV/c$. Without core (Fig.~\ref{simu} left), simulations from EPOS~LHC do not reproduce data at all because not enough hard scattering are present and flow is not there to increase the average transverse momentum. Using a preliminary version of EPOS~3 (full line) which include a new variable saturation scale~\cite{Werner:2013vba} which provide more hard scattering, simulations without flow from collective hadronization  (Fig.~\ref{simu} left) reproduce very well the data. While with flow (Fig.~\ref{simu} right) the description becomes very bad at high $p_t$ due to a too large energy loss in the high density medium which is probably overestimated here (based on PbPb collisions). 

\begin{figure}[hptb]
\begin{centering}
\includegraphics[height=0.85\columnwidth,angle=-90]{UE/Pierog/underlying.eps}%
\caption{\label{simu} ATLAS measurement  of  charged particles with $p_t \geq 100$MeV  produced in the transverse region~\protect\cite{Aad:2010fh} compared to  EPOS~LHC (dashed line) and EPOS~3.1 (solid line) simulations without (left) or with (right) core formation.}
\end{centering}
\end{figure}
 \vspace{-2mm}
\section*{Outlook}

Collective flow (or color reconnection) are very important for the description of underlying events for leading track $p_t$ below $5~Gev/c$. Collective flow treatment in EPOS~3 will be improve to describe both low and high $p_t$ particles.

\begin{thebibliography}{9}
\bibitem{Affolder:2001xt}
  T.~Affolder {\it et al.}  [CDF Collaboration],
  %``Charged jet evolution and the underlying event in $p\bar{p}$ collisions at 1.8 TeV,''
  {\em Phys.\ Rev.\ D} {\bf 65} (2002) 092002.
  %%CITATION = PHRVA,D65,092002;%%
  %272 citations counted in INSPIRE as of 16 Jan 2015
 \vspace{-2mm}
\bibitem{Aad:2010fh}
  G.~Aad {\it et~al.} [Atlas Collaboration], , 
%{\it {Measurement of
%  underlying event characteristics using charged particles in pp collisions at
%  $\sqrt{s} = 900 GeV$ and 7 TeV with the ATLAS detector}},  
  {\em Phys.Rev.}
  {\bf D83} (2011) 112001
%, [\href{http://xxx.lanl.gov/abs/1012.0791}{{\tt
   [arXiv:1012.0791].
 \vspace{-2mm}
\bibitem{Chatrchyan:2011id}
  S.~Chatrchyan {\it et al.}  [CMS Collaboration],
  %``Measurement of the Underlying Event Activity at the LHC with $\sqrt{s}= 7$ TeV and Comparison with $\sqrt{s} = 0.9$ TeV,''
  {\em JHEP} {\bf 1109} (2011) 109
  [arXiv:1107.0330 [hep-ex]].
  %%CITATION = ARXIV:1107.0330;%%
  %148 citations counted in INSPIRE as of 16 Jan 2015
 \vspace{-7mm}
\bibitem{Pierog:2013ria}
  T.~Pierog, I.~Karpenko, J.~M.~Katzy, E.~Yatsenko and K.~Werner,
  %``EPOS LHC : test of collective hadronization with LHC data,''
  arXiv:1306.0121 [hep-ph].
  %%CITATION = ARXIV:1306.0121;%%
  %55 citations counted in INSPIRE as of 16 Jan 2015
 \vspace{-2mm}
\bibitem{Werner:2013vba}
  K.~Werner, B.~Guiot, I.~Karpenko and T.~Pierog,
  %``New developments in EPOS: Parton saturation,''
  {\em J.\ Phys.\ Conf.\ Ser.\ }  {\bf 458} (2013) 012020.
  %%CITATION = 00462,458,012020;%%
  %1 citations counted in INSPIRE as of 16 Jan 2015

\end{thebibliography}




==> UE/Siodmok/content_Siodmok.tex <==
\title{MPI in Herwig++}
\author{Andrzej Siodmok}
\affiliation{CERN, PH-TH, CH-1211 Geneva 23, Switzerland}

\maketitle

Models with hard~\cite{Bahr:2008dy} (similar to JIMMY [2] package) and soft component [3] of multiple
partonic interactions as well as improved colour reconnection models [4] are available in Herwig++. 
The main parameters of the model are $p_{t,min}$ which sets a transition scale between hard and soft 
(non-perturbative) component, $\mu$ parameter which can be interpreted as the inverse radius of the proton and 
$p_{reco}$ the probablity of colour reconnection. The parameters are obtained from fits to previous MPI, 
UE and sigma effective data. The most recent UE-EE-5 tune~\cite{Seymour:2013qka} is able to describe
the double-parton scattering cross section~\cite{Bahr:2013gkj,Seymour:2013sya} 
and charged tracks underlying event data collected over the collision energy range 
from $\sqrt{s} = 300$~GeV to $\sqrt{s} = 7$~TeV, see Fig.~\ref{fig:TVT} and Fig.~\ref{fig:LHC}.
\begin{figure*}[htb]
  \includegraphics[width=0.5\textwidth]{UE/Siodmok/CDF_2012_NOTE10874_d01.eps}
  \includegraphics[width=0.5\textwidth]{UE/Siodmok/CDF_2012_NOTE10874_d02.eps}
  \vspace*{-5ex}
    \caption{CDF data and model fits at at ${300}$~GeV\ (lowest sets),
      ${900}$~GeV\ (middle sets) and ${1960}$~GeV\ (top sets), showing
      the mean multiplicity density (left panel) and mean scalar
      $p_{\perp}$ sum (right panel) of the stable charged particles in
      the ``transverse'' area as a function of~$\ptlead$.}
  \label{fig:TVT}
\end{figure*}
\begin{figure*}[htb]
  \includegraphics[width=0.5\textwidth]{UE/Siodmok/ATLAS_2010_S8894728_d01.eps}
  \includegraphics[width=0.5\textwidth]{UE/Siodmok/ATLAS_2010_S8894728_d02.eps}
  \vspace*{-5ex}
    \caption{ATLAS data and model fits at ${900}$~GeV\ (lowest sets)
      and ${7}$~TeV\ (middle sets), showing the mean multiplicity
      density (left panel) and mean scalar $p_{\perp}$ sum (right panel)
      of the stable charged particles in the ``transverse'' area as a
      function of~$\ptlead$. The predictions for 14~TeV (top sets) are
      shown for comparison.}
  \label{fig:LHC}
\end{figure*}
The predictions for 14~TeV are shown in Fig.~\ref{fig:LHC} (top sets).\\
There was also progress in improving the forward rapidity gap description in Herwig++
presented in a separate contribution by M. Myska. 
\newpage
\providecommand{\href}[2]{#2}\begingroup\begin{thebibliography}{10}
                                         
                                        
  \bibitem{Bahr:2008dy}
  M.~Bahr, S.~Gieseke and M.~H.~Seymour,
  %``Simulation of multiple partonic interactions in Herwig++,''
  JHEP {\bf 0807} (2008) 076
  [arXiv:0803.3633 [hep-ph]].
  
%\cite{Butterworth:1996zw}
\bibitem{Butterworth:1996zw}
  J.~M.~Butterworth, J.~R.~Forshaw and M.~H.~Seymour,
  %``Multiparton interactions in photoproduction at HERA,''
  Z.\ Phys.\ C {\bf 72} (1996) 637
  [hep-ph/9601371].
  %%CITATION = HEP-PH/9601371;%%
  %1003 citations counted in INSPIRE as of 01 juin 2015


  %%CITATION = ARXIV:0803.3633;%%
  %109 citations counted in INSPIRE as of 13 May 2015
  %\cite{Seymour:2013qka}
  %\cite{Gieseke:2012ft}
\bibitem{Gieseke:2012ft}
  S.~Gieseke, C.~Rohr and A.~Siodmok,
  %``Colour reconnections in Herwig++,''
  Eur.\ Phys.\ J.\ C {\bf 72} (2012) 2225
  [arXiv:1206.0041 [hep-ph]].
  %%CITATION = ARXIV:1206.0041;%%
  %54 citations counted in INSPIRE as of 13 May 2015
\bibitem{Seymour:2013qka}
  M.~H.~Seymour and A.~Siodmok,
  %``Constraining MPI models using $\sigma_{eff}$ and recent Tevatron and LHC Underlying Event data,''
  JHEP {\bf 1310} (2013) 113
  [arXiv:1307.5015 [hep-ph]].
  %%CITATION = ARXIV:1307.5015;%%
  %21 citations counted in INSPIRE as of 13 May 2015
  %\cite{Bahr:2013gkj}
\bibitem{Bahr:2013gkj}
  M.~Bahr, M.~Myska, M.~H.~Seymour and A.~Siodmok,
  %``Extracting $\sigma_{\rm effective}$ from the {CDF} $\gamma$+3jets measurement,''
  JHEP {\bf 1303} (2013) 129
  [arXiv:1302.4325 [hep-ph]].
  %%CITATION = ARXIV:1302.4325;%%
  %21 citations counted in INSPIRE as of 13 May 2015
  %\cite{Seymour:2013sya}
\bibitem{Seymour:2013sya}
  M.~H.~Seymour and A.~Siodmok,
  %``Extracting $\sigma_{\rm effective}$ from the LHCb double-charm measurement,''
  arXiv:1308.6749 [hep-ph].
  %%CITATION = ARXIV:1308.6749;%%
  %6 citations counted in INSPIRE as of 13 May 2015
  
  \end{thebibliography}


==> UE/Sjostrand/content_Sjostrand.tex <==
\title{MPI in PYTHIA}
\author{Torbj\"orn Sj\"ostrand}
\affiliation{Department of Astronomy and Theoretical Physics\\Lund University}

\maketitle

The development of the MPI framework for hadronic collisions in PYTHIA
was begun almost exactly 30 years ago. Most of the basic ideas of the 
early framework \cite{zijl87} have survived, and several have come to be 
generally accepted:\\
$-$ multiple (semi)perturbative (mini)jet production as the origin for a 
unified description of hard jets, underlying events and minimum-bias 
events;\\
$-$ screening as a mechanism to tame the divergence of the cross section
in the $p_{\perp} \to 0$ limit, with a characteristic turnoff scale
around 2 GeV;\\ 
$-$ a $p_{\perp}$-ordered generation ensures that the PDFs of the hardest 
interaction can be the conventional ones, while the ones used for softer 
interactions need to be successively modified;\\
$-$ an impact-parameter dependence gives a natural mechanism to obtain a
pedestal effect; and\\
$-$ colour reconnection is needed to explain the rise of 
$\langle p_{\perp} \rangle(n_{\mathrm{ch}})$.

Over the years this basic picture has been refined in numerous ways,
including interleaved evolution of MPI, ISR and FSR, energy-dependent 
screening, more sophisticated multiparton PDFs, junction topologies, 
partonic rescattering, an $x$-dependent proton size, MPI in diffractive 
events, and more. These models have continuously been made publicly 
available, most recently in PYTHIA~8.2 \cite{pythia14}. Some have led 
to improvements in the description of data, while others have yet to 
make a visible impact. Much but not all data can be explained, leaving 
room for further improvements, and for the inclusion of additional effects, 
such as hadronic rescattering.

Potentially the biggest ``known unknown'' in the MPI framework is the 
role of colour reconnection (CR). The description of MPI, ISR and FSR 
leads to multiple colour confinement fields -- strings -- being spanned 
criss-cross in the event, often overlapping with each other. While this 
picture typically is formulated in the limit of an infinite number of 
colours, there is no indication that a more correct, but static, colour 
description would resolve the issue. Rather some kind of dynamical effects 
seem required, where the overlapping strings may reconnect, usually
so as to reduce the total string length. This still leaves a big room
for potential models.

The understanding of colour reconnection can have an impact on issues
such as top mass reconstruction, where the experimental precision now 
is below 1~GeV. Since the PYTHIA~8.1 code only contained one CR model
(unlike PYTHIA 6.4, which contained more), recently several new models
were introduced \cite{arg14}. These fall into two main classes. In one 
the top decay products only get the chance to reconnect after the rest of 
the event has been handled as usual, while in the other the top decay 
products are handled in the same way as other partons. The former class
stealthily gives more freedom from experimental constraints, and therefore
is convenient to explore worst-case scenarios. Experience with these models 
suggest that the CR top mass uncertainty could be as high as half a GeV, 
but with a rather asymmetric distribution.

Other models for CR have been presented by several other speakers at this
meeting, whereof the one described by Jesper Roy Christiansen is also 
available in PYTHIA 8.2. 

\begin{thebibliography}{9}
\bibitem{zijl87}
T. Sj\"ostrand and M. van Zijl, \emph{A Multiple Interaction Model for 
the Event Structure in Hadron Collisions}, Phys.Rev. D36 (1987) 2019
\bibitem{pythia14}
T. Sj\"ostrand et al., \emph{An Introduction to PYTHIA 8.2},
arXiv:1410.3012 [hep-ph]
\bibitem{arg14}
S. Argyropoulos and T. Sj\"ostrand, \emph{Effects of color reconnection 
on $t\overline{t}$ final states at the LHC},
JHEP 1411 (2014) 043 [arXiv:1407.6653 [hep-ph]]  
\end{thebibliography}



==> UE/Strikman/content_StrikmanUE.tex <==
\title{Jets in multiparticle production in and beyond\\ geometry of proton-proton collisions at the LHC}
\author{M. Yu. Azarkin$^1$, M. Strikman$^2$}
\maketitle
\begin{center}
$^1$ Lebedev Physical Institute of RAS,
National Research Nuclear University "MEPhI",\\$^2$ 104 Davey Lab, The Pennsylvania State University,  University Park, PA 16803, USA\\
\end{center}
The impact parameter (b) distribution  of the minimum bias inelastic $pp$ collisions can be calculated based on the information about elastic $pp$ scattering while 
the distribution over $b$   of inclusive dijet production is given by the convolution of the generalized parton distributions (GPDs) of the colliding protons.
The GPDs for small $x$ gluons can be extracted from the HERA data on hard exclusive processes like $\gamma p\to J/\psi p$.
It was demonstrated in  \cite{Frankfurt:2003td} that minimum bias and hard collisions  occur, on average, at very different impact parameters -- medians of $b$-distribution differ by a factor of $\approx 2$.
At the same time, the b-distribution for production of dijets weakly depends on $p_{\rm T}$ of the jets or their rapidity. 

We use this information to analyze 
experimental findings by CMS on properties of jets and underlying events at different multiplicities in proton-proton interactions at 7 TeV.  
Observed  data-MC disagreements at hight multiplicities are interpreted as  an indication of increasing role of central collisions. 
The value of the average impact parameter of the pp collisions  as a function of the soft hadron multiplicity is estimated. 
 We find an indication that  the rates of  different hard processes  observed by CMS and ALICE  universally depend on the underlying event charged-particle multiplicity until it becomes four times higher than average. 
It is shown that the increase of the overlap area of colliding protons is not sufficient to explain  the rate of jet production in events with charged-particle multiplicity
 that is more than three times higher than average.  New mechanisms are necessary, like interaction of protons in rare configurations of higher than average gluon density.
Such mechanisms are not included in the present Monte Carlo event generators. In any case it is interesting that the  ridge in $pp$ scattering  observed for multiplicities where geometry breaks and hard processes are strongly enhanced. 


More detailed studies are also highly desirable. In particular, it would be preferable to study dependence on the multiplicity of the underlying event rather than on the total multiplicity.
It would be also interesting to study events where 
$R=N_{\rm ch}/\left<N_{\rm ch}\right> < 1$.  In this case  the ratio  of double parton scattering rate  to single parton scattering one should be significantly suppressed as compared to inclusive case, 
while for  $R\sim 3$  it is expected to be enhanced as compared to the inclusive case by a factor $\sim 2$ with a further  possible increase due to gluon fluctuations.
It would  be also interesting to investigate how  the  production of leading baryons (for example, production of leading neutrons with $x_{\rm F} \ge 0.3$) is correlated with $R$. 
Indeed, it was argued \cite{Drescher:2008zz}   that the  neutron yield in the proton fragmentation region drops with an increase of the centrality of the pp collisions 
and also decreases  faster  with increase of $x_{\rm F}$. If so, one  expects that, with increase of  $R$, the neutron multiplicity for large $x_{\rm F} \ge 0.3$  will diminish and it will be 
very strongly suppressed for  $R \ge  4 $. 

Acknowledgments:
M. Azarkin is  grateful for support by the RFBR grants 12-02-91504-CERN-a, 14-02-00099, and the RAS-CERN program.  M. Strikman's research  was supported  by DOE grant No. DE-FG02-93ER40771.
\vspace{-0.3cm}
        \begin{thebibliography}{9}
        %
\bibitem{Frankfurt:2003td} 
  L.~Frankfurt, M.~Strikman and C.~Weiss,
  %``Dijet production as a centrality trigger for $p p$ collisions at CERN LHC,''
  Phys.\ Rev.\ D {\bf 69}, 114010 (2004)
  [hep-ph/0311231];
          Phys.\ Rev.\ D {\bf 83}, 054012 (2011)
  [arXiv:1009.2559 [hep-ph]].
  
   \bibitem{Azarkin:2014cja} 
  M.~Y.~Azarkin, I.~M.~Dremin and M.~Strikman,
  %``Jets in multiparticle production in and beyond geometry of protonÐproton collisions at the LHC,''
  Phys.\ Lett.\ B {\bf 735}, 244 (2014)
  [arXiv:1401.1973 [hep-ph]].
  
  \bibitem{Drescher:2008zz}H.~J.~Drescher and M.~Strikman,
  %``How to probe high gluon densities in p p collisions at the Large Hadron Collider,''
  Phys.\ Rev.\ Lett.\  {\bf 100}, 152002 (2008).
   \end{thebibliography}
   



==> UE/Strikman/content_massi.tex <==
\title{Evidence for $x$-dependent proton
 color fluctuations \\in pA collisions at the LHC}
\author{M. Alvioli$^1$, B. A. Cole$^2$, L. Frankfurt$^3$, M. Strikman$^4$}
\maketitle
\begin{center}
$^1$ CNR-IRPI, via Madonna Alta 126, I-06128, Perugia, Italy\\
$^2$ Columbia University, New York, NY 10027, USA\\
$^3$ Tel Aviv University, Tel Aviv,  Israel\\
$^4$ 104 Davey Lab, The Pennsylvania State University, University Park, PA 16803, USA\\
\end{center}
In pA collisions at collider energies a projectile stays in a frozen 
configuration over the distances which by far exceed the nuclear diameter. 
As a result the proton coherently interacts with nucleons along its impact 
parameter. In QCD a nucleon is build of quark-gluon configurations of different transverse 
size which are expected to interact with different strength, leading to
fluctuations of the global strength of the projectile interactions. Also, 
configurations of smaller size are expected to have a reduced gluon field 
leading to a correlation of soft and hard interactions. To describe these
effects it is convenient to introduce a probability distribution for the projectile
to interact with strength $\sigma$, $P_N(\sigma)$. $P_N(\sigma)$ is strongly
constrained by the diffractive $pp$ data, the behavior  of $P_N$ for $\sigma\to 0$
expected in pQCD, etc \cite{Heiselberg:1991is}. We developed a Monte Carlo procedure
to describe these effects in soft collisions and collisions with a hard
trigger taking into account the difference of the transverse scales of hard and soft
interactions  \cite{Alvioli:2013vk,Alvioli:2014sba}. The prediction that the distribution
over the number of wounded nucleons should be broader than the Glauber
model expectation was confirmed at the LHC \cite{TheATLAScollaboration:2013cja}.
We argue that the violation of the Glauber approximation
for the dependence  of the rate of forward jet production on centrality observed in $pA$
collisions at the LHC provides the first experimental evidence that parton configurations
in the projectile proton containing a parton with large $x_p$ interact with a nuclear target
with a significantly smaller than average cross section, and have smaller than average size.
Implementing effects of such fluctuations of the interaction strengths and using the ATLAS
analysis \cite{TheATLAScollaboration:2013cja} of the dependence of  the hadron production at backward rapidities on the number
of wounded nucleons, we make quantitative predictions for the centrality dependence of the
jet production rate as a function of the interaction strength $\sigma(x_p)$. For $x_p=0.6$
we find $\sigma(x_p)\sim \sigma_{tot}(pp)/2$ \cite{Alvioli:2014eda} which has implications
on the origin of the EMC effect. Future studies of  dijet production along these lines would
allow to investigate the global 3D structure of the nucleon and to trigger on particular
configurations which interact with a larger-than-average strenght.
 %
\begin{thebibliography}{9}
 %
\bibitem{Heiselberg:1991is} 
  H.~Heiselberg, G.~Baym, B.~Blaettel, L.~L.~Frankfurt and M.~Strikman,
  %``Color transparency, color opacity, and fluctuations in nuclear collisions,''
  Phys.\ Rev.\ Lett.\  {\bf 67}, 2946 (1991); Phys.\ Rev.\ C {\bf 52}, 1604 (1995)
 %
\bibitem{Alvioli:2013vk} 
  M.~Alvioli and M.~Strikman,
  %``Color fluctuation effects in proton-nucleus collisions,''
  Phys.\ Lett.\ B {\bf 722}, 347 (2013)
  %[arXiv:1301.0728 [hep-ph]].
  %
\bibitem{Alvioli:2014sba} 
  M.~Alvioli, L.~Frankfurt, V.~Guzey and M.~Strikman,
  %``Revealing ÒflickeringÓ of the interaction strength in pA collisions at the CERN LHC,''
  Phys.\ Rev.\ C {\bf 90}, no. 3, 034914 (2014)
  %[arXiv:1402.2868 [hep-ph]].
  %
\bibitem{TheATLAScollaboration:2013cja} 
  The ATLAS collaboration,
  %``Measurement of the centrality dependence of the charged particle pseudorapidity distribution in proton-lead collisions at $\sqrt{s_{NN}} = 5.02$ TeV with the ATLAS detector,''
  ATLAS-CONF-2013-096, ATLAS-COM-CONF-2013-117,
  %%CITATION = ATLAS-CONF-2013-096, ATLAS-COM-CONF-2013-117;%%
  %22 citations counted in INSPIRE as of 09 Jan 2015
  https://cds.cern.ch/record/1599773.
  %
\bibitem{Alvioli:2014eda} 
  M.~Alvioli, B.~Cole, L.~Frankfurt and M.~Strikman,
  %``Evidence for x-dependent proton color fluctuations in pA collisions at the LHC,''
  arXiv:1409.7381 [hep-ph]. 
  %
\end{thebibliography}
   


==> UE/Strikman/contentmaxim.tex <==
\title{Jets in multiparticle production in and beyond\\ geometry of proton-proton collisions at the LHC}
\author{M. Yu. Azarkin$^1$, M. Strikman $^2$}
\maketitle
\begin{center}
$^1$ Lebedev Physical Institute of RAS,
National Research Nuclear University "MEPhI",\\$^2$ 104 Davey Lab, The Pennsylvania State University,  University Park, PA 16803, USA\\
\end{center}
The impact parameter (b) distribution  of the minimum bias inelastic $pp$ collisions can be calculated based on the information about elastic $pp$ scattering while 
the distribution over $b$   of inclusive dijet production is given by the convolution of the generalized parton distributions (GPDs) of the colliding protons.
The GPDs for small $x$ gluons can be extracted from the HERA data on hard exclusive processes like $\gamma p\to J/\psi p$.
It was demonstrated in  \cite{Frankfurt:2003td} that minimum bias and hard collisions  occur, on average, at very different impact parameters -- medians of $b$-distribution differ by a factor of $\approx 2$.
At the same time, the b-distribution for production of dijets weakly depends on $p_{\rm T}$ of the jets or their rapidity. 

We use this information to analyze 
experimental findings by CMS on properties of jets and underlying events at different multiplicities in proton-proton interactions at 7 TeV.  
Observed  data-MC disagreements at hight multiplicities are interpreted as  an indication of increasing role of central collisions. 
The value of the average impact parameter of the pp collisions  as a function of the soft hadron multiplicity is estimated. 
 We find an indication that  the rates of  different hard processes  observed by CMS and ALICE  universally depend on the underlying event charged-particle multiplicity until it becomes four times higher than average. 
It is shown that the increase of the overlap area of colliding protons is not sufficient to explain  the rate of jet production in events with charged-particle multiplicity
 that is more than three times higher than average.  New mechanisms are necessary, like interaction of protons in rare configurations of higher than average gluon density.
Such mechanisms are not included in the present Monte Carlo event generators. In any case it is interesting that the  ridge in $pp$ scattering  observed for multiplicities where geometry breaks and hard processes are strongly enhanced. 


More detailed studies are also highly desirable. In particular, it would be preferable to study dependence on the multiplicity of the underlying event rather than on the total multiplicity.
It would be also interesting to study events where 
$R=N_{\rm ch}/\left<N_{\rm ch}\right> < 1$.  In this case  the ratio  of double parton scattering rate  to single parton scattering one should be significantly suppressed as compared to inclusive case, 
while for  $R\sim 3$  it is expected to be enhanced as compared to the inclusive case by a factor $\sim 2$ with a further  possible increase due to gluon fluctuations.
It would  be also interesting to investigate how  the  production of leading baryons (for example, production of leading neutrons with $x_{\rm F} \ge 0.3$) is correlated with $R$. 
Indeed, it was argued \cite{Drescher:2008zz}   that the  neutron yield in the proton fragmentation region drops with an increase of the centrality of the pp collisions 
and also decreases  faster  with increase of $x_{\rm F}$. If so, one  expects that, with increase of  $R$, the neutron multiplicity for large $x_{\rm F} \ge 0.3$  will diminish and it will be 
very strongly suppressed for  $R \ge  4 $. 

Acknowledgments:
M. Azarkin is  grateful for support by the RFBR grants 12-02-91504-CERN-a, 14-02-00099, and the RAS-CERN program.  M. Strikman's research  was supported  by DOE grant No. DE-FG02-93ER40771.
\vspace{-0.3cm}
        \begin{thebibliography}{9}
        %
\bibitem{Frankfurt:2003td} 
  L.~Frankfurt, M.~Strikman and C.~Weiss,
  %``Dijet production as a centrality trigger for $p p$ collisions at CERN LHC,''
  Phys.\ Rev.\ D {\bf 69}, 114010 (2004)
  [hep-ph/0311231];
          Phys.\ Rev.\ D {\bf 83}, 054012 (2011)
  [arXiv:1009.2559 [hep-ph]].
  
   \bibitem{Azarkin:2014cja} 
  M.~Y.~Azarkin, I.~M.~Dremin and M.~Strikman,
  %``Jets in multiparticle production in and beyond geometry of protonÐproton collisions at the LHC,''
  Phys.\ Lett.\ B {\bf 735}, 244 (2014)
  [arXiv:1401.1973 [hep-ph]].
  
  \bibitem{Drescher:2008zz}H.~J.~Drescher and M.~Strikman,
  %``How to probe high gluon densities in p p collisions at the Large Hadron Collider,''
  Phys.\ Rev.\ Lett.\  {\bf 100}, 152002 (2008).
   \end{thebibliography}
   



==> UE/WeiYang/content_WeiYang.tex <==
\title{Measurement of the underlying event activity using charged particle jets in proton-proton collisions at 2.76 TeV}
\author{Wei Yang Wang}
\affiliation{On behalf of the CMS Collaboration\\National University of Singapore\\University of Antwerp}

\maketitle

%\section{Open problems}
A measurement of the underlying event in proton-proton collisions is performed using events with a leading charged 
particle jet produced at central pseudorapidity ($|\eta^{\textrm{jet}}|<2$) and of transverse momentum 
($p^{\textrm{jet}}_{\textrm{T}}$) in the range of $1$ to $100$ \textrm{GeV}. 
The analysis uses a data sample collected at the LHC by the CMS experiment at a centre-of-mass energy of 2.76 \textrm{TeV},
corresponding to an integrated luminosity of 0.3 \textrm{nb$^{-1}$}. 
The particle and $\Sigma p_{\textrm{T}}$ densities are studied in the
transverse region, defined by the difference in azimuthal angle between the leading track jet
and charged particle directions, $60^{\circ}<|\Delta\phi|<120^{\circ}$.
By dividing the transverse region into the minimum and maximum activity sides with respect to the highest $p_{\textrm{T}}$ jet,
and studying their difference, further information on the dynamics of the UE is obtained \cite{UEleadjet0}.

A steep rise of the underlying event activity in the transverse region is seen with increasing leading jet $p_{\textrm{T}}$.
This fast rise is followed by a saturation region above $\sim 8$ \textrm{GeV}, with nearly constant multiplicity and
small $\Sigma p_{\textrm{T}}$ density increase. Such a distinct change of the amount of activity depending on the transverse
momentum of the leading charged-particle jet is clearly seen for all the observables. The difference between the
minimum and maximum activity transverse regions show an increase of activity with $p^{\textrm{jet}}_{\textrm{T}}$ corroborating
the hypothesis of an increasing contribution from initial- and final-state radiation.

The results are compared to recent Monte Carlo event generator tunes\cite{PYTHIA6, PYTHIA8, HERWIG++, Z2*, CUETP68S1, UE-EE-5C}.
By comparing data taken at $\sqrt{s}=0.9$, $2.76$ and $7$ \textrm{TeV}
\cite{UEleadjet0, UEleadjet, UEleadjet2}, a strong growth with increasing centre-of-mass
energy of the hadronic activity in the transverse region is also observed for the same value of
the leading charged-particle jet $p_{\textrm{T}}$.
All MC tunes predict the centre-of-mass energy dependence of the hadronic activity in a way that is very similar to data.
These measurements are expected to play a significant role in the future development and tuning of MC
models of the underlying event.

\begin{figure}[htbp]
\centering
\begin{subfigure}[b]{0.4\textwidth}
	\includegraphics[width=\textwidth]{UE/WeiYang/compMCResultUnfoldNchEnergies.eps}
\end{subfigure}
\qquad
\begin{subfigure}[b]{0.4\textwidth}
        \includegraphics[width=\textwidth]{UE/WeiYang/compMCResultUnfoldPtsumEnergies.eps}
\end{subfigure}
        \caption{\label{fig:genProfiletransregVSe} Comparison of UE activity at $\sqrt{s}=$ 0.9, 2.76 and 7 \textrm{TeV} for
         for particle density (a) and $\Sigma p_{\textrm{T}}$
density (b) as a function of the leading charged-particle jet $p_{\textrm{T}}$~\cite{UEleadjet0, UEleadjet, UEleadjet2}.}
\end{figure}

%\section{Outlook}
Measurements of the underlying event activity has contributed to our understanding of soft dynamics and Monte Carlo generator tuning.
A measurement of the underlying event activity at 13 \textrm{TeV} would be crucial for the verification of these tunes and provide 
additional discriminatory power of multi parton interactions and beam-beam remnants against initial- and final-state radiation effects 
on the UE activity.

\begin{thebibliography}{9}
\bibitem{UEleadjet0}
  CMS Collaboration, ``Measurement of the underlying event activity using charged particle jets in proton-proton collisions at 2.76 TeV'',
  CMS-PAS-FSQ-12-025
\bibitem{PYTHIA6}
  T. Sj{\"o}strand and S. Mrenna and P. Skands, ``PYTHIA $6.4$ physics and manual'', \emph{JHEP} \textbf{05} (2006) 026
\bibitem{PYTHIA8}
  T. Sj{\"o}strand and S. Mrenna and P. Skands, ``A Brief Introduction to PYTHIA 8.1'', \emph{Comput. Phys. Commun.} 
  \textbf{178} (2008) 852
\bibitem{HERWIG++}
  M. B{\"a}hr et al., ``Herwig++ physics and manual'', \emph{Eur. Phys. J. C} \textbf{58} (2008) 639
\bibitem{Z2*}
  The CMS Collaboration, ``Measurement of energy flow at large pseudorapidities in $pp$ collisions at $\sqrt {s} = 0.9$ and $7$ TeV'', 
  \emph{JHEP} \textbf{11} (2011) 148
\bibitem{CUETP68S1}
  The CMS Collaboration, ``Underlying Event Tunes and Double Parton Scattering'', CMS Physics Analysis Summary, 
  CMS-PAS-GEN-14-001 ,2014
\bibitem{UE-EE-5C}
  M. H Seymour and A. Siodmok, ``Constraining MPI models using $\sigma_{eff}$ and recent Tevatron and LHC Underlying Event data'', 
  \emph{JHEP} \textbf{1310} (2013) 113
\bibitem{UEleadjet}
  The CMS Collaboration, ``Measurement of the underlying event activity at the LHC with $\sqrt {s} = 7$ TeV and
  comparison with $\sqrt {s} = 0.9$ TeV'', \emph{JHEP} \textbf{09} (2011) 109
\bibitem{UEleadjet2}
  The CMS Collaboration, ``First measurement of the underlying event activity at the LHC with $\sqrt{s} = 0.9$ TeV'',
  \emph{Eur. Phys. J. C} \textbf{70} (2010) 555
\end{thebibliography}



==> UE/content_Summary_Jung.tex <==
\title{Outlook on Minimum Bias and Underlying Events}
\author{H. Jung}
\affiliation{}                                    % Activate to display a given date or no date

\maketitle

When LHC started in 2009/2010 none of the predictions for the charged multiplicity $dn/d\eta$ nor for the underlying event as a function of the transverse momentum of a leading track or jet was agreeing with the measurements. Since then, huge progress has been made in the modeling and understanding of minimum bias and the underlying event structure. Now, just before LHC restarts at $\sqrt{s}=13$~TeV, all relevant models are able to describe the main features of the events at $\sqrt{s} = 7(8)$~TeV, after a big effort of tuning the free parameters. 

However, different tunes exist for different observables: tunes for minimum bias events, for underlying events with jets and different parameters might be needed when running with higher order calculations. 
A big step forward was observed with the measurement of $dn/d\eta$ from CMS-Totem, which had a clean definition of the phase space in terms of particles in the forward detectors from Totem. A reasonable description of this measurement was achieved with the CMS underlying event tunes (without the need to further re-tune). 

The latest up-to-date tunes from both ATLAS and CMS are able to describe reasonably well the existing measurements and the predictions to higher energies (for LHC run2 at 13 TeV) do not differ very much. However, ons should keep in mind, that a difference of 0.5 particles/$\eta$ in minimum bias events will lead to a differences of $\sim 20$ particles/$\eta$ at the high pileup conditions of run2. Therefore, the very first measurements of $dn/d\eta$ at 13 TeV will be very important.

Apart from a good description of the minimum bias and underlying events, a few conceptional issues have to be kept in mind:
\begin{itemize}
\item The detailed mechanism of the taming/saturation of the (mini-) jet cross section from large to very small $p_T$  and the connection to saturation physics is still not well understood.
\item With the present tunes, it seems to be non-trivial to describe at the same time minimum bias, underlying events and hard double parton scattering. If the basic principles of multiparton interaction are appropriate at these different scales, a unified description over the full kinematic range is needed.
\item  With the present knowledge it is not clear, whether the same parameter tunes can  be applied in NLO (or multi-leg) matched parton shower and hadronization calculations like POWHEG, MC@NLO or ALPGEN, MADGRAPH. For a unified description, this would be necessary.
\item Experimental observables must be defined in a way, which is free from prejudice, i.e. without assuming the existence of multiparton interactions. The concept of multiparton interaction is directly interwoven with the concept of factorisation. If cross sections can be described with a different way of factorisation, then the role of multi-parton interactions might be very different.
\end{itemize}
%\section{}
%\subsection{}


==> UE/content_Summary_merged.tex <==
\title{Outlook on MPI and MC models}
\author{A. Grebenyuk, D. Kar and A. Siodmok}
\affiliation{}
\maketitle

\subsubsection*{Introduction}

Multiple Parton Interaction (MPI) is among the least well understood phenomenon, but
a proper modeling of it is necessary for measurements and searches. Monte Carlo (MC) 
event generators include different phenomenological models for MPI, 
and a significant progress in development of MPI models happened in response to LHC Run~I data.

\subsubsection*{LHC Run 1 Summary}

ATLAS, ALICE and CMS performed a host of measurements sensitive to different aspects of soft QCD, particularly
MPI. They include
the \textit{minimum bias} (MB) charged particle distributions~\cite{Aamodt:2010pp, Aad:2010ac, Khachatryan:2010us}, transverse energy flow~\cite{Aad:2012mfa}, 
and traditional underlying event (UE) measurements in different topologies~\cite{Aad:2010fh, Aad:2011qe,:2012fs, LJ, DY, Chatrchyan:2011id, 
Chatrchyan:2012tb}, 
There have been other new measurements
as well, but not all of them are corrected back to particle level, thereby reducing their usefulness.

The first charged multiplicity and leading-track underlying events measurements at 7 TeV, 
and surprisingly at 900 GeV showed incompatibility with all the pre-LHC
Monte Carlo models, with the MPI part mostly \textit{tuned} to 1.96 TeV Tevatron data. 
This led to a rapid retuning effort, described in the next section.

The tuning obviously is one part, where the soft-QCD resulted are utilised. On the other hand, many of the results have been
interesting on their own accord. CMS used jet areas to estimate the contribution of underlying event~\cite{Chatrchyan:2012tt}, and ATLAS measured 
the standard deviation of the usual charged particle multiplicity or charged particle sum \pT profiles (as a function of leading track \pT).
A steady non-zero plateau-like shape demonstrated that UE effect cannot just be subtracted as an average value for all events.
The ATLAS measurement with charged particle jets, varying the radius of charged particle jets showed the activity initially increases
with increasing charged particle jet radius - pointing possibly to selection bias. Finally both CMS and ATLAS comparison of UE in 
dijet and $Z$-boson events showed very similar activity, confirming the similar behavior seen at CDF~\cite{Aaltonen:2010rm}. 
It was also realised that at 
very busy LHC environments, the traditional \textit{transverse and trans-min regions} 
(with respect to the hard scattering direction in $\eta$ -$\phi$
space) is not just sensitive to UE, but receive contribution from additional radiation~\cite{DY}. To mitigate the contamination, ATLAS looked
at exclusive dijet topology, vetoing addition hard jets, which can be a promising way to gain sensitivity to MPI effects~\cite{LJ}.

\subsubsection*{Model development and Tuning}

The model development can be briefly summarised as:

\begin{itemize}

 \item Pythia 6/8: had already well developed MPI model before Run 1 data. However, the disagreement with
 LHC data prompted the experiments to start a quick retuning effort 
 and a tension between all three center-of-mass energies were observed. 
 ATLAS and CMS, as well as Peter Skands came up with new Pythia 6 tunes which would describe the 
 7 TeV data better~\cite{Skands:2010ak}, termed the Perugia tune. 
 While the Perugia series of tunes and tunes from CMS were aimed to describe both minimum-bias (MB) 
 and underlying event (UE) data simultaneously, it became apparent that separate tunes for minimum bias and 
 underlying event can result in individually better descriptions for either categories. While this option was certainly 
 not the aesthetically pleasing one, ATLAS adapted this philosophy, and started producing separate 
 MB and UE tunes. 
 As the usage of Pythia 8 gained more popularity, ATLAS focused more attention 
 to Pythia 8 tunes~\cite{:atlasmc11,:atlasmc11new,:atlasmc12}, and separately there were tunes by authors, 
 Peter Skands (the Monash series~\cite{Skands:2014pea}), and finally by CMS~\cite{}.
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%
 %%%TODO: ADD CMS TUNING REF
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 There has also been significant progress in the model development:
  $x$-dependent overlap function~\cite{Corke:2011yy}, MPI re-scattering~\cite{Corke:2009tk}, a lot of 
  tunes~\cite{Skands:2010ak,Skands:2014pea, Corke:2010yf} 
  and most recently a new string formation beyond leading colour~\cite{Christiansen:2015yqa}.

 \item Herwig++: the program includes model with hard~\cite{Bahr:2008dy} and soft~\cite{Bahr:2009ek} MPI scatters.
 The LHC MB data triggered development of colour reconnection (CR)
 models~\cite{Gieseke:2012ft} and the authors provided new tunes~\cite{Gieseke:2012ft,Seymour:2013qka}. 
 The most recent UE-EE-5 tune~\cite{Seymour:2013qka} is able to describe
 the double-parton scattering cross section~\cite{Bahr:2013gkj,Seymour:2013sya} 
 and charged tracks underlying event data collected over the collision energy range 
 from $\sqrt{s} = 300$~GeV to $\sqrt{s} = 7$~TeV.

 \item Sherpa: constructed and implemented a new MPI model SHRiMPS~\cite{Khoze:2010by} based on
  KMR model, which is multi-channel eikonal model with partonic interpretation of pomeron.
  It has been released recently and should be tuned soon (to construct a new model it takes years!).
  Currently the model can be only used to described MB physics and the extention of the model
  to UE is ongoing.
  
\end{itemize}


Other programs which main aim is to describe cosmic rays or/and heavy ion collisions 
also made remarkable progress:
\begin{itemize}
 \item EPOS which is used for both heavy ion interactions and cosmic ray air shower simulations  
  released
  its LHC version~\cite{Pierog:2013ria} which provides successful description of LHC MB data.
  \item DIPSY~\cite{Flensburg:2012zy} a MC generator primarily developed for simulation of MB in pp 
  collisions and heavy ion physics, recently implemented so called rope model~\cite{Bierlich:2014xba}. 
  This model includes the effect of overlapping strings in the Lund Hadronisation Model.
\end{itemize}

With the advent of LHC, tuning of MC generators also saw  an ``industrial revolution''.
In addition to tuning by eye, started by Rick Field, use of automated tuning tool 
Professor~\cite{Buckley:2009bj} using the analysis toolkit Rivet~\cite{Buckley:2010ar} 
became popular. In parallel, platforms like mcplots~\cite{Karneyeu:2013aha} have made
tune comparisons easy by using volunteer computer resources.

 Historically tuning efforts have been by tuning the hadronisation model by LEP results, 
 and MPI model by Tevatron and LHC results. Monash for example-tuned the hadronisation 
 parameters by using LHC data as well, while the latest ATLAS effort~\cite{:mc14} tuned the 
 shower and MPI parameters simultaneously, 
 coming up with a tune suitable for used in high \pT processes, and matched setups.

\subsubsection*{Open Issues and Run 2 Ideas}

Despite of all the progress and successes of the models there is definitively still scope for 
significant improvements in the future. 
There are aspects in data that our models cannot describe. For example, none of the models/tunes do a good job at describing
the transverse energy flow in high rapidity range, as seen from both ATLAS and CMS results. There seems to be a conflict in
describing the transverse energy flow in central rapidity regions in MB events with charged particle \pT spectra.
The particle content in events,
more specifically the fraction of strange mesons and baryons is not modeled accurately by any generators. 

Another example is that the observation that $\langle p_T\rangle$ 
increases with $n_{ch}$ suggests that there is some mechanism of correlating partons 
from different MPI systems. Models which have had some success in describing the $<p_T>$($n_{ch}$) 
distributions have some method of stronger correlating MPI systems using
colour reconnection (CR) (Herwig++ and Pythia) or hydrodynamic collective flow (EPOS). 
This part of modelling is definitively the biggest known unknown.
It would be important task for future experimental and phenomenological studies to find
ways to check which model (or maybe a superposition of both) is realized by the nature. 
It is worth to stress that the CR uncertainties are important to many precision measurements, 
they are especially important in the top mass measurements, 
see for details~\cite{Argyropoulos:2014zoa}. Unfortunately, CR uncertainties are often 
underestimated by the experimental collaborations (see T. Sjöstrand's talk). 
One way to address this problem is by dedicated experimental studies of CR in top events. 
Other examples where MPI uncertainty might be underestimated is DPS background to Higgs searches 
(as presented by W. Krasny) this problem should be also addressed by our community. 
The estimation of DPI/MPI cross section is tied to constructing  
generator specific MPI-on and MPI-off templates~\cite{Aad:2013bjm}, where
we have no evidence that the MPI modeling in any generator is accurate. 
CMS added the effective DPI cross-section as a
tuning parameter, which results in a slightly improved description.

The first major challenge in Run 2 will obviously be to test the energy extrapolation of the models using
the early (low pileup) 13 TeV data. In~Fig.~\ref{fig:EE}, it can be seen that some commonly used tunes have very different
MPI \pT cutoff at 13 TeV. The minimum bias measurements, and height of the underlying event plateau 
will be useful indicators of the models.

\begin{figure}[htb]
  \centering
  \includegraphics[width=0.49\textwidth]{UE/EE_Py8_13.eps} \qquad
   \includegraphics[width=0.44\textwidth]{UE/extrapolation_new.eps} \\
  \caption{Energy Extrapolation of some Pythia8 (left) and Herwig++ (right) tunes}
  \label{fig:EE}
\end{figure}

With more data, the focus will shift to modeling the MPI in high \pT events. It will be essential to find observables
or topologies which are less affected by extra jets, thereby enabling us to estimate MPI contribution to processes
of interest in searches and measurements. 

This also means that rather than leading order parton shower generators,
generators with NLO or multileg matrix element interfaced with a parton shower
generator can lead to a better description of data even for 
observables sensitive to soft effects. 

There is also a lack of a uniform way to treat the model uncertainties. Experimentally this is
often one of the dominant source of systematic uncertainty. Comparison between different
generators or tunes has been the conventional way, but more recently ATLAS has advocated the
eigentunes approach using the Professor system.  There is still some way to go before 
we have a consistent recipe. 

Run 2 data will help us to answer some of the questions, however 
some points  discussed in Perugia 2008 meeting are equally relevant today
\begin{itemize}

\item How should the relative importance of various data be judged? 
\item When are discrepancies due to poor physics or to poorly documented/measured data? 
\item How can we avoid over-tuning, i.e. avoid forcing the model to fit the data even if the data contain 
physics not included in the model (which is often the demand of experimental collaborations)?

\end{itemize}

We end by remembering the warning from Perugia proceedings:

"In summary, the pride of recent successes should not blind us to the challenges ahead." 

\clearpage

\providecommand{\href}[2]{#2}\begingroup\begin{thebibliography}{10}

\bibitem{Aamodt:2010pp} 
{ALICE} Collaboration,
 {\em Charged-particle multiplicity measurement in proton-proton collisions at $\sqrt{s}=7$ TeV with ALICE at LHC}
  Eur.\ Phys.\ J.\ C {\bf 68}, 345 (2010)
  [arXiv:1004.3514 [hep-ex]].
  %%CITATION = ARXIV:1004.3514;%%
  %228 citations counted in INSPIRE as of 01 Jun 2015

\bibitem{Aad:2010ac} 
{ATLAS} Collaboration,
  {\em Charged-particle multiplicities in pp interactions measured with the ATLAS detector at the LHC}
  New J.\ Phys.\  {\bf 13}, 053033 (2011)
  [arXiv:1012.5104 [hep-ex]].
  %%CITATION = ARXIV:1012.5104;%%
  
  \bibitem{Khachatryan:2010us} 
{CMS} Collaboration,
{\em Transverse-momentum and pseudorapidity distributions of charged hadrons in $pp$ collisions at $\sqrt{s}=7$ TeV}
  Phys.\ Rev.\ Lett.\  {\bf 105}, 022002 (2010)
  [arXiv:1005.3299 [hep-ex]].
  %%CITATION = ARXIV:1005.3299;%%
  %306 citations counted in INSPIRE as of 01 juin 2015

%\cite{Aad:2012mfa}
\bibitem{Aad:2012mfa} 
 {ATLAS} Collaboration,
  {\em Measurements of the pseudorapidity dependence of the total transverse energy in proton-proton collisions at $\sqrt{s}=7$ TeV with ATLAS}
  JHEP {\bf 1211}, 033 (2012)
  [arXiv:1208.6256 [hep-ex]].

  \bibitem{Aad:2010fh}
{The ATLAS} Collaboration, {\em {Measurement of underlying event
  characteristics using charged particles in pp collisions at $\sqrt{s} = 900$
  GeV and $7$ TeV with the ATLAS detector}\/},
  \href{http://dx.doi.org/10.1103/PhysRevD.83.112001}{Phys. Rev. D {\bf 83}
  (2011)  112001},
\href{http://arxiv.org/abs/1012.0791}{{\tt arXiv:1012.0791 [hep-ex]}}.
%%CITATION = 1012.0791;%%.

\bibitem{Aad:2011qe}
{ATLAS} Collaboration, {\em {Measurements of underlying-event
  properties using neutral and charged particles in pp collisions at 900 GeV
  and 7 TeV with the ATLAS detector at the LHC}\/},\\
  \href{http://dx.doi.org/10.1140/epjc/s10052-011-1636-z}{Eur. Phys. J. {\bf
  C71} (2011)  1636},
\href{http://arxiv.org/abs/1103.1816}{{\tt arXiv:1103.1816 [hep-ex]}}. 
%%CITATION = 1103.1816;%%.

 \bibitem{:2012fs}
 {The ATLAS} Collaboration, {\em {Underlying event characteristics and their dependence on jet size of charged-particle jet events in $pp$ collisions at $\sqrt{s}=7$ TeV with the ATLAS detector}\/},
  \href{http://dx.doi.org/10.1103/PhysRevD.86.072004}{Phys. Rev. D {\bf 86}
  (2012)  072004},
\href{http://arxiv.org/abs/1208.0563}{{\tt arXiv:1208.0563 [hep-ex]}}.
  %%CITATION = ARXIV:1208.0563;%%
  
\bibitem{LJ}
{The ATLAS} Collaboration, {\em {Studies of the underlying event accompanying jets measured with ATLAS}\/},
  \href{http://dx.doi.org/10.1140/epjc/s10052-014-2965-5}{Eur. Phys. J. {\bf C74} (2014) 2965},
 \href{http://arxiv.org/abs/1406.0392}{{\tt arXiv:1406.0392 [hep-ex]}}.\\

\bibitem{DY}
{The ATLAS} Collaboration, {\em {Measurement of distributions sensitive 
to the underlying event in inclusive Z-boson production in pp collisions at $\sqrt{s}=7$ TeV with the ATLAS detector}\/},
  \href{http://dx.doi.org/10.1140/epjc/s10052-014-3195-6}{Eur. Phys. J. {\bf C74} (2014) 3195},
   \href{http://arxiv.org/abs/1409.3433}{{\tt arXiv:1409.3433 [hep-ex]}}.

%\cite{Chatrchyan:2011id}
\bibitem{Chatrchyan:2011id} 
{CMS} Collaboration,
  {\em Measurement of the Underlying Event Activity at the LHC with $\sqrt{s}= 7$ TeV and Comparison with $\sqrt{s} = 0.9$ TeV}
  JHEP {\bf 1109}, 109 (2011)
  [arXiv:1107.0330 [hep-ex]].
  %%CITATION = ARXIV:1107.0330;%%
  %166 citations counted in INSPIRE as of 01 juin 2015
  
  %\cite{Chatrchyan:2012tb}
  \bibitem{Chatrchyan:2012tb} 
{CMS} Collaboration,
  {\em Measurement of the underlying event in the Drell-Yan process in proton-proton collisions at $\sqrt{s}=7$ TeV}
  Eur.\ Phys.\ J.\ C {\bf 72}, 2080 (2012)
  [arXiv:1204.1411 [hep-ex]].
  %%CITATION = ARXIV:1204.1411;%%
  %32 citations counted in INSPIRE as of 01 juin 2015

\bibitem{Chatrchyan:2012tt} 
{CMS} Collaboration,
{\em Measurement of the underlying event activity in $pp$ collisions at $\sqrt{s} = 0.9$ and 7 TeV with the novel jet-area/median approach}
  JHEP {\bf 1208}, 130 (2012)
  [arXiv:1207.2392 [hep-ex]].
  %%CITATION = ARXIV:1207.2392;%%
  %19 citations counted in INSPIRE as of 01 juin 2015

%\cite{Aaltonen:2010rm}
\bibitem{Aaltonen:2010rm} 
  T.~Aaltonen {\it et al.}  [CDF Collaboration],
  {\em Studying the Underlying Event in Drell-Yan and High Transverse Momentum Jet Production at the Tevatron}
  Phys.\ Rev.\ D {\bf 82}, 034001 (2010)
  [arXiv:1003.3146 [hep-ex]].
  %%CITATION = ARXIV:1003.3146;%%
  %73 citations counted in INSPIRE as of 01 juin 2015

\bibitem{Skands:2010ak} 
  P.~Z.~Skands,
  %``Tuning Monte Carlo Generators: The Perugia Tunes,''
  Phys.\ Rev.\ D {\bf 82}, 074018 (2010)
  [arXiv:1005.3457 [hep-ph]].
  %%CITATION = ARXIV:1005.3457;%%
  %554 citations counted in INSPIRE as of 31 May 2015
  
\bibitem{:atlasmc11}
{The ATLAS} Collaboration,  {\em {ATLAS tunes of PYTHIA 6 and
  PYTHIA 8 for MC11}\/},  2011.
\newblock ATL-PHYS-PUB-2011-009. \url{http://cdsweb.cern.ch/record/1363300}. 
  
  \bibitem{:atlasmc11new}
{The ATLAS} Collaboration,  {\em {Further ATLAS tunes of PYTHIA 6 and
  PYTHIA 8 for MC11}\/},  2011.
\newblock ATL-PHYS-PUB-2011-014. \url{https://cdsweb.cern.ch/record/1400677}. 
  
\bibitem{:atlasmc12}
{The ATLAS} Collaboration,  {\em {Summary of ATLAS Pythia 8 tunes}\/},  2012.
\newblock ATL-PHYS-PUB-2012-003. \url{https://cdsweb.cern.ch/record/1474107}. 
  
  \bibitem{Skands:2014pea} 
  P.~Skands, S.~Carrazza and J.~Rojo,
  %``Tuning PYTHIA 8.1: the Monash 2013 Tune,''
  Eur.\ Phys.\ J.\ C {\bf 74}, no. 8, 3024 (2014)
  [arXiv:1404.5630 [hep-ph]].
  
\bibitem{:mc14}
{The ATLAS} Collaboration,
 {\em {ATLAS Run 1 Pythia8 tunes}\/},  2014.
\newblock ATLAS-CONF-2014-021.\\ \url{https://cds.cern.ch/record/1966419}.
  
 %\cite{Corke:2011yy}
\bibitem{Corke:2011yy}
  R.~Corke and T.~Sjostrand,
  %``Multiparton Interactions with an x-dependent Proton Size,''
  JHEP {\bf 1105} (2011) 009
  [arXiv:1101.5953 [hep-ph]].
  %%CITATION = ARXIV:1101.5953;%%
  %34 citations counted in INSPIRE as of 13 May 2015 
  %\cite{Argyropoulos:2014zoa}
  
  \bibitem{Corke:2009tk}
  R.~Corke and T.~Sjostrand,
  %``Multiparton Interactions and Rescattering,''
  JHEP {\bf 1001} (2010) 035
  [arXiv:0911.1909 [hep-ph]].
  %%CITATION = ARXIV:0911.1909;%%
  %40 citations counted in INSPIRE as of 13 May 2015
  
  %\cite{Corke:2010yf}
\bibitem{Corke:2010yf}
  R.~Corke and T.~Sjostrand,
  %``Interleaved Parton Showers and Tuning Prospects,''
  JHEP {\bf 1103} (2011) 032
  [arXiv:1011.1759 [hep-ph]].
  %%CITATION = ARXIV:1011.1759;%%
  %140 citations counted in INSPIRE as of 13 May 2015
  %\cite{Skands:2014pea}
  %\cite{Skands:2010ak}
  
  %\cite{Christiansen:2015yqa}
\bibitem{Christiansen:2015yqa}
  J.~R.~Christiansen and P.~Z.~Skands,
  %``String Formation Beyond Leading Colour,''
  arXiv:1505.01681 [hep-ph].
  %%CITATION = ARXIV:1505.01681;%%
  
\bibitem{Bahr:2008dy}
  M.~Bahr, S.~Gieseke and M.~H.~Seymour,
  %``Simulation of multiple partonic interactions in Herwig++,''
  JHEP {\bf 0807} (2008) 076
  [arXiv:0803.3633 [hep-ph]].
  %%CITATION = ARXIV:0803.3633;%%
  %109 citations counted in INSPIRE as of 13 May 2015
  %\cite{Seymour:2013qka}
  %\cite{Gieseke:2012ft}
  
  \bibitem{Bahr:2009ek}
  M.~Bahr, J.~M.~Butterworth, S.~Gieseke and M.~H.~Seymour,
  %``Soft interactions in Herwig++,''
  arXiv:0905.4671 [hep-ph].
  %%CITATION = ARXIV:0905.4671;%%
  %23 citations counted in INSPIRE as of 01 juin 2015
  
\bibitem{Gieseke:2012ft}
  S.~Gieseke, C.~Rohr and A.~Siodmok,
  %``Colour reconnections in Herwig++,''
  Eur.\ Phys.\ J.\ C {\bf 72} (2012) 2225
  [arXiv:1206.0041 [hep-ph]].
  %%CITATION = ARXIV:1206.0041;%%
  %54 citations counted in INSPIRE as of 13 May 2015
  
\bibitem{Seymour:2013qka}
  M.~H.~Seymour and A.~Siodmok,
  %``Constraining MPI models using $\sigma_{eff}$ and recent Tevatron and LHC Underlying Event data,''
  JHEP {\bf 1310} (2013) 113
  [arXiv:1307.5015 [hep-ph]].
  %%CITATION = ARXIV:1307.5015;%%
  %21 citations counted in INSPIRE as of 13 May 2015
  %\cite{Bahr:2013gkj}
  
\bibitem{Bahr:2013gkj}
  M.~Bahr, M.~Myska, M.~H.~Seymour and A.~Siodmok,
  %``Extracting $\sigma_{\rm effective}$ from the {CDF} $\gamma$+3jets measurement,''
  JHEP {\bf 1303} (2013) 129
  [arXiv:1302.4325 [hep-ph]].
  %%CITATION = ARXIV:1302.4325;%%
  %21 citations counted in INSPIRE as of 13 May 2015
  %\cite{Seymour:2013sya}
  
\bibitem{Seymour:2013sya}
  M.~H.~Seymour and A.~Siodmok,
  %``Extracting $\sigma_{\rm effective}$ from the LHCb double-charm measurement,''
  arXiv:1308.6749 [hep-ph].
  %%CITATION = ARXIV:1308.6749;%%
  %6 citations counted in INSPIRE as of 13 May 2015
  
  %\cite{Corke:2009tk}

%\cite{Khoze:2010by}
\bibitem{Khoze:2010by}
  V.~A.~Khoze, F.~Krauss, A.~D.~Martin, M.~G.~Ryskin and K.~C.~Zapp,
  %``Diffraction and correlations at the LHC: Definitions and observables,''
  Eur.\ Phys.\ J.\ C {\bf 69} (2010) 85
  [arXiv:1005.4839 [hep-ph]].
  %%CITATION = ARXIV:1005.4839;%%
  %27 citations counted in INSPIRE as of 13 May 2015  
  
  %\cite{Pierog:2013ria}
\bibitem{Pierog:2013ria}
  T.~Pierog, I.~Karpenko, J.~M.~Katzy, E.~Yatsenko and K.~Werner,
  %``EPOS LHC : test of collective hadronization with LHC data,''
  arXiv:1306.0121 [hep-ph].
  %%CITATION = ARXIV:1306.0121;%%
  %68 citations counted in INSPIRE as of 18 May 2015
 %\cite{Flensburg:2012zy}
\bibitem{Flensburg:2012zy}
  C.~Flensburg, G.~Gustafson and L.~Lönnblad,
  %``Exclusive final states in diffractive excitation,''
  JHEP {\bf 1212} (2012) 115
  [arXiv:1210.2407 [hep-ph]].
  %%CITATION = ARXIV:1210.2407;%%
  %6 citations counted in INSPIRE as of 19 May 2015
 %\cite{Bierlich:2014xba}
\bibitem{Bierlich:2014xba}
  C.~Bierlich, G.~Gustafson, L.~Lönnblad and A.~Tarasov,
  %``Effects of Overlapping Strings in pp Collisions,''
  JHEP {\bf 1503} (2015) 148
  [arXiv:1412.6259 [hep-ph]].
  %%CITATION = ARXIV:1412.6259;%%
  %2 citations counted in INSPIRE as of 19 May 2015
\bibitem{Argyropoulos:2014zoa}
  S.~Argyropoulos and T.~Sjöstrand,
  %``Effects of color reconnection on $t\bar{t}$ final states at the LHC,''
  JHEP {\bf 1411} (2014) 043
  [arXiv:1407.6653 [hep-ph]].
  %%CITATION = ARXIV:1407.6653;%%
  %6 citations counted in INSPIRE as of 13 May 2015
  %\cite{Buckley:2009bj}
\bibitem{Buckley:2009bj}
  A.~Buckley, H.~Hoeth, H.~Lacker, H.~Schulz and J.~E.~von Seggern,
  %``Systematic event generator tuning for the LHC,''
  Eur.\ Phys.\ J.\ C {\bf 65} (2010) 331
  [arXiv:0907.2973 [hep-ph]].
  %%CITATION = ARXIV:0907.2973;%%
  %175 citations counted in INSPIRE as of 20 May 2015
  %\cite{Buckley:2010ar}
\bibitem{Buckley:2010ar}
  A.~Buckley, J.~Butterworth, L.~Lonnblad, D.~Grellscheid, H.~Hoeth, J.~Monk, H.~Schulz and F.~Siegert,
  %``Rivet user manual,''
  Comput.\ Phys.\ Commun.\  {\bf 184} (2013) 2803
  [arXiv:1003.0694 [hep-ph]].
  %%CITATION = ARXIV:1003.0694;%%
  %174 citations counted in INSPIRE as of 20 May 2015
  %\cite{Karneyeu:2013aha}
  
\bibitem{Karneyeu:2013aha}
  A.~Karneyeu, L.~Mijovic, S.~Prestel and P.~Z.~Skands,
  %``MCPLOTS: a particle physics resource based on volunteer computing,''
  Eur.\ Phys.\ J.\ C {\bf 74} (2014) 2714
  [arXiv:1306.3436 [hep-ph]].
  %%CITATION = ARXIV:1306.3436;%%
  %11 citations counted in INSPIRE as of 13 May 2015
  
\bibitem{Aad:2013bjm} 
{The ATLAS} Collaboration,
  {\em Measurement of hard double-parton interactions in $W(\to l\nu)$+ 2 jet events at $\sqrt{s}$=7 TeV with the ATLAS detector}
  New J.\ Phys.\  {\bf 15}, 033038 (2013)
  [arXiv:1301.6872 [hep-ex]].
  %%CITATION = ARXIV:1301.6872;%%
  %93 citations counted in INSPIRE as of 01 juin 2015  
  
\end{thebibliography}

==> lowX/Astalos/content.tex <==
\title{Measurements of event shapes and particle production with the ATLAS detector}
\author{R\'obert Astalo\v{s}\\\vspace{0.1cm}
{\small on behalf of the ATLAS Collaboration}}
\affiliation{Comenius University Bratislava, Radboud University Nijmegen}

\maketitle

Measurements of event shapes and production properties of mesons and baryons at 7 TeV proton-proton collisions data taken by the ATLAS detector\cite{atlas} in 2010 are presented.

The evolution of the event shape variables, such as the transverse thrust, thrust minor and transverse sphericity has been studied for minimum bias events as functions of the $p_\mathrm{T}$ of the leading 
particle in an event\cite{event_shapes}. With increasing $p_\mathrm{T}^{\rm lead}$ a shift to less spherical events is observed. This effect is more profound in case of the transverse sphericity than 
for the other event shape variables. All MC models considered tend to reproduce data better for higher $p_{\rm T}^{\rm lead}$ ranges. Among them the 
Pythia 6 tune Z1 which was tuned to Underlying Event at LHC agrees best with data. The dependence of the mean values of the event shape variables on a charged-particle 
transverse momentum scalar sum of the event shows an increse followed by a decrease. For all MC models considered, this decrease occurs before that of the data (see left plot of 
Fig.~\ref{fig:1} for case of the transverse sphericity mean value). Furthermore, all MC models predict less high-sphericity events than seen in the data.

The differential production cross section of the $\phi$(1020)-meson has been studied using the $\phi\rightarrow K^+K^-$ decay mode\cite{phi_meson}. The integrated $\phi$-meson production cross 
section in this fiducial range ($500 < p_{\mathrm{T},\phi} < 1200$ MeV, $|y_\phi|<0.8$) is measured to be 
$\sigma_\phi\times BR(\phi\rightarrow K^+K^-)=570\pm8$~(stat) $\pm$ 68 (syst) $\pm$ 20 (lumi) $\mu$b. The cross section has also 
been studied as a function of the transverse momentum $p_{\mathrm{T},\phi}$ (right plot of Fig.~\ref{fig:1}) and rapidity $|y_\phi|$ and was found to be in best agreement with 
the predictions of the MC generator tunes EPOS-LHC and Pythia 6 DW.

The transverse polarization of $\Lambda$ and ${\bar \Lambda}$ hyperons produced in minimum bias events has been measured to be 
$P_\Lambda$ = - 0.010 $\pm$ 0.005~(stat) $\pm$ 0.004~(syst) and $P_{\bar \Lambda}$ = 0.002 $\pm$ 0.006~(stat) $\pm$ 0.004~(syst). In bins of $p_\mathrm{T}$ 
and Feynman-$x$ variable, polarization is found to be less than 2\% and is consistent with zero within estimated uncertainties as predicted by the Standard Model.


\begin{figure}[h]
\begin{center}
\begin{tabular}{cc}
\includegraphics[width=0.39\linewidth]{fig1.pdf}
\includegraphics[width=0.535\linewidth]{fig2.pdf}
\end{tabular}
\caption{Mean value of the transverse sphericity as a function of charged-particle transverse momentum scalar sum of the event (left) and the $\phi(1020)\rightarrow K^+K^-$ 
cross section as a function of the transverse momentum $p_{\mathrm{T},\phi}$ (right). The error bars represent the statistical uncertainty 
and the green boxes represent the combined statistical and systematic uncertainty.
\label{fig:1}}
\end{center}
\end{figure}
\vspace{-0.85cm}

\begin{thebibliography}{9}
\bibitem{atlas} ATLAS Collaboration, JINST 3 (2008) S08003
\bibitem{event_shapes}  ATLAS Collaboration, Phys. Rev. D 88, 032004 (2013) [arXiv:1207.6915]
\bibitem{phi_meson} ATLAS Collaboration, Eur. Phys. J. C (2014) 74:2895 [arXiv:1402.6162]
\end{thebibliography}


==> lowX/Baranov/content_Baranov.tex <==
\title{Kinematic corrections to Quarkonium production in NRQCD approach}

\author{Sergey Baranov}
\affiliation{P.N.Lebedev Institute of Physics\\Russian Academy of Sciences}

\maketitle

\def\cc {$c\bar{c}$~}
\def\cj {$\chi_{cJ}$~}
\def\bb {$b\bar{b}$~}
\def\qq {$Q\bar{Q}$~}
%\def\m  {$m_{Octet}$~}
\def\m  {$m_{[8]}$~}
\def\J {$J/\psi$ }   
\def\Js {$J/\psi$'s~}
\def\j { J/\psi  }
\def\pjt {$p_{\psi,T}$~}
\def\ktf {$k_t$-factorization }
\def\ktfa {$k_t$-factorization approach }
\def\dum#1#2#3  {{~}                         {\bf#1}, #2 (#3)}
\def\plb#1#2#3  {{Phys.\ Lett.\ B }          {\bf#1}, #2 (#3)}
\def\prd#1#2#3  {{Phys.\ Rev.\ D }           {\bf#1}, #2 (#3)}
\def\prl#1#2#3  {{Phys.\ Rev.\ Lett.\ }      {\bf#1}, #2 (#3)}
\section*{Introduction and motivation}

Quarkonium production in high energy hadrinic collisions is usually expressed 
in terms of non-relativistic QCD (NRQCD) factorization approach \cite{NRQCD}.
In its mathematical aspects, this approach is similar to the classical theory 
of multipole radiation;
in practice, numerical calculations are always accompanied by an exordium that
a \qq pair produced in hard subprocess as color-octet emits 
(a number of) soft gluons changing the quantum numbers of the \qq system without 
changing its energy-momentum. This is in obvious contradiction with confinement 
which prohibits the emission of soft colored quanta. 
Our note represents an attempt to estimate the numerical effect of final state 
radiation on the experimental observables if to replace an 'infinitely soft' 
gluon with a 'real' quantum of nonzero (of order $\Lambda_{QCD}$)
energy-momentum.

\section*{Results and conclusions}

The simulation is organized as follows. First, we generate the production 
of a color-octet \cc state in a usual perturbative way, but with a mass \m 
slightly higher than the nominal \J mass in order to preserve some phase space 
for the subsequent decay. As an example we tried \m = 3.4 and 3.7 GeV. After 
that we generate a two-body decay $c\bar{c}[8]\to J/\psi + X$. We do not specify 
the nature of the state $X$, since the only property of importance is its mass 
$m_X$. For illustration we tried $m_X$=0, 150, 300, and 500 MeV.

The $p_t$ of the resulting \J is smaller than that of the originall \cc pair, 
as part of the initial momentum is carried away by the quantum $X$. The visible 
kinematic effect (i.e., the ratio of the cross sections before and after emission
$d\sigma(c\bar{c}[8])/dp_t$ and $d\sigma(J/\psi)/dp_t$)
%and $d\sigma(c\bar{c}[8])/dp_t$)
turned out to be very similar for all intermediate octet states
($^1S_0^{[8]}$, $^3S_1^{[8]}$, $^3P_0^{[8]}$, $^3P_1^{[8]}$, $^3P_2^{[8]}$),
despite the individual spectra on their own may be rather different.
The effect is nearly insensitive to the mass of the emitted quantum $m_X$
and is only sensitive to the mass difference between \m and $m_\psi$. 
The kinematic correction is large and, therefore, cannot be neglected.
On the other hand, it flattens at high $p_t$, and so, can be effectively
included into redefined nonperturbative matrix elements.







%\begin{figure}
\hspace*{-1cm}
\includegraphics[width=8.cm, height=4.5cm]{lowX/Baranov/m34.eps}
\includegraphics[width=8.cm, height=4.5cm]{lowX/Baranov/m37.eps}\\
Kinematic correction factors for $p_t$ spectra due to final state radiation.
The mass of the emitted system $m_X$ is set to 0 (solid curves),
150 MeV (dashed), 300 MeV (dotted), and 500 MeV (dash-dotted).
The octet state mass is set to 3.4 GeV (left panel) and 3.7 GeV (right panel).
%\end{figure}

\begin{thebibliography}{9}
\bibitem{NRQCD} G. T. Bodwin, E. Braaten, and G. P. Lepage,
                       \prd{51}{1125}{1995} ; \dum{55}{5853(E)}{1997} .
\end{thebibliography}


==> lowX/Cherednikov/content_Cherednikov.tex <==
\title{Unintegrated PDFs from low to high $x$: theoretical issues}
\author{I.O. Cherednikov}
\affiliation{Universiteit Antwerpen, Belgium}

\maketitle


Partonic content of nucleons beyond the collinear approximation is probed in {\it semi-inclusive reactions} with polarized and unpolarized hadrons, where the intrinsic transverse momenta and spin-orbit correlations of the partons are directly accessible \cite{Boer:2011fh}. To this end, collinear PDFs are replaced by the {\it transverse-momentum dependent} parton densities (TMDs) \cite{Collins:2011zzd}. 




%\begin{enumerate}

%\item 
{Fully inclusive processes} are studied within the collinear QCD factorization framework making use of ($\mathbf k_\perp$-integrated) PDFs. DGLAP resummation is based on the strong {ordering of emitted patrons in their transverse momenta}, which suggests that the hard matrix elements are {on-shell} (e.g., the virtualities are much smaller than the hard scale) \cite{Dokshitzer:1978hw}. The DGLAP evolution sums up ${\ln \mu^2/\Lambda^2}$ logarithms. 

%\item 
Theoretical understanding of the {semi-inclusive processes} calls for updated factorization methods, which include various {\it unintegrated} PDFs. 
%{
%\begin{itemize}

%\item 
{\it BFKL} method is directly applicable in the {high energy} or small-$x$ regime. In contrast to DGLAP, it suggests the strong {ordering in the rapidities} of emitted partons. The 
hard matrix elements are, therefore, allowed to be {off-shell} \cite{Andersson:2002cf}. This method enables resummation of the ${\ln 1/x}$ logarithms and allows for {nonlinear} extensions. 

%\item 
{\it CCFM} approach makes use of the {angular ordering} of the emitted patrons, the hard matrix elements are also {off-shell} and 
the dependence on {extra scale} (maximal angle) is introduced. As such, this approach is not restricted to the {small-$x$ regime} but is valid as also for the {large}-$x$. 
It ${ \ln 1/x}$ as well as ${\ln 1/(1-x)}$ logarithms \cite{Andersson:2002cf}. 
 
%\item 
{\it TMD} framework is constructed as a direct {generalisation} of the collinear picture. The operator definitions of TMD PDFs are formally valid in the {whole range} of $x$. 
However, beyond the tree-approximation a number of specific singularities emerges (the light-cone or rapidity divergences, mixed UV/rapidity terms, etc.), which calls for 
extra {rapidity scale} and yields more complicated, as compared to the collinear case, {evolution} equations \cite{Collins:2011zzd,Cherednikov:2007tw,GarciaEchevarria:2011rb}. 

%\item 
Soft-Collinear Effective Theory {\it (SCET)} utilises the idea of the energy scale separation that results in the construction of an {effective Lagrangian}, the latter being used to obtain the TMD correlators. This approach is shown to be {equivalent to the TMD} scheme \cite{GarciaEchevarria:2011rb}. 
 
%\end{itemize}
%}

%\end{enumerate}

Given that the {unintegrated PDF} framework is aimed to provide a unique theoretical scheme for small- and large-$x$ experiments (EIC, JLab, RHIC, AFTER@LHC), the detailed comparison of the TMD evolution with DGLAP, BFKL, nonlinear small-$x$ and CCFM  appears to be one of the most urgent tasks \cite{REF2014}. 



\begin{thebibliography}{9}

\bibitem{Boer:2011fh}
  D.~Boer, 
  %M.~Diehl, R.~Milner, R.~Venugopalan, W.~Vogelsang, D.~Kaplan, H.~Montgomery and S.~Vigdor 
  {\it et al.},
  %``Gluons and the quark sea at high energies: Distributions, polarization, tomography,''
  arXiv:1108.1713 [nucl-th]
  %%CITATION = ARXIV:1108.1713;%%


  
\bibitem{Collins:2011zzd}
%  \bibitem{D'Alesio:2007jt}
  U.~D'Alesio and F.~Murgia,
  %``Azimuthal and Single Spin Asymmetries in Hard Scattering Processes,''
  Prog.\ Part.\ Nucl.\ Phys.\  {\bf 61} (2008) 394;
 % [arXiv:0712.4328 [hep-ph]].
  %%CITATION = ARXIV:0712.4328;%%
  J.~Collins,
  ``Foundations of perturbative QCD'' (2011)  
  \bibitem{Dokshitzer:1978hw}
  Y.~L.~Dokshitzer, D.~Diakonov and S.~I.~Troian,
  %``Hard Processes in Quantum Chromodynamics,''
  Phys.\ Rept.\  {\bf 58} (1980) 269
  %%CITATION = PRPLC,58,269;%%
 
 \bibitem{Andersson:2002cf}
  B.~Andersson {\it et al.},  
  %[Small x Collaboration],
  %``Small x phenomenology: Summary and status,''
  Eur.\ Phys.\ J.\ C {\bf 25} (2002) 77
%  [hep-ph/0204115].
  %%CITATION = HEP-PH/0204115;%% 

  
 \bibitem{Cherednikov:2007tw}
  I.~O.~Cherednikov and N.~G.~Stefanis,
 % \bibitem{Cherednikov:2008ua}
%  I.~O.~Cherednikov and N.~G.~Stefanis,
  %``Wilson lines and transverse-momentum dependent parton distribution functions: A Renormalization-group analysis,''
  Nucl.\ Phys.\ B {\bf 802} (2008) 146;
 % [arXiv:0802.2821 [hep-ph]].
  %%CITATION = ARXIV:0802.2821;%%
%  \bibitem{Cherednikov:2009wk}
  %I.~O.~Cherednikov and N.~G.~Stefanis,
  %``Renormalization-group properties of transverse-momentum dependent parton distribution functions in the light-cone gauge with the Mandelstam-Leibbrandt prescription,''
  Phys.\ Rev.\ D {\bf 80} (2009) 054008
 % [arXiv:0904.2727 [hep-ph]].
  %%CITATION = ARXIV:0904.2727;%%
  

  \bibitem{GarciaEchevarria:2011rb}
  M.~G.~Echevarria, A.~Idilbi and I.~Scimemi,
  %``Factorization Theorem For Drell-Yan At Low q_T And Transverse Momentum Distributions On-The-Light-Cone,''
  JHEP {\bf 1207} (2012) 002;
 % [arXiv:1111.4996 [hep-ph]].
  %%CITATION = ARXIV:1111.4996;%%
%   \bibitem{Collins:2012uy}
  J.~C.~Collins and T.~C.~Rogers,
  %``Equality of Two Definitions for Transverse Momentum Dependent Parton Distribution Functions,''
  Phys.\ Rev.\ D {\bf 87} (2013) 034018
%  [arXiv:1210.2100 [hep-ph]].
  %%CITATION = ARXIV:1210.2100;%%
  
 
  
  \bibitem{REF2014}
  {\tt https://indico.cern.ch/event/330428}
  
  
\end{thebibliography}



==> lowX/DeakCCFM/content_Deak.tex <==
\title{Kinematical constraint and the CCFM equation}
\author{$^a$Michal De\'ak, $^b$Krzysztof Kutak}
\affiliation{$^a$Instituto de F\'isica Corpuscular, CSIC and Universitat de Valencia, E-46071 Valencia, Spain\\
$^b$Instytut Fizyki J\u adrowej im. H. Niewodnicza\'nskiego 
Radzikowskiego 152, 31-342 Krakow, Poland
}

\maketitle

\section*{Introduction}
In the high energy regime of hadronic scattering (the centre 
of mass energy is larger than any other present scale), perturbative approach 
to processes with high momentum transfer allows factorisation 
of the cross section into a hard matrix element and a gluon 
density~\cite{Gribov:1984tu}. In 
analogy with the BFKL approach the gluon density is a function of the 
longitudinal momentum fraction $x$ and transverse momentum ${\bf k}$ of a gluon.
In addition dependence on a scale $p$ related to a hard process is introduced. 
For small densities the gluon density obtained in the above approach the gluon 
density obeys the CCFM 
equation~\cite{Ciafaloni:1987ur}. The CCFM equation 
incorporates 
gluon radiation coherence by summing gluon ladder diagrams with rungs ordered in 
angle.

The angular ordering -- an essential ingredient of the CCFM equation --
introduces a constraint on kinematic variables in the integral on the 
right-hand-side of the equation. It turns out it is necessary to include also
the kinematical constraint~\cite{Kwiecinski:1996td} into the CCFM and the BFKL equations 
as well since it was 
assumed in the derivation of both of them ensuring the gluon $4$-momentum
invariant  to be dominated by $-{\bf k}^2$. The kinematic constraint causes suppression of the amplitude growth especially for low $|{\bf k}|$. An effect of suppression of the growth of the amplitude is achieved also by introducing saturation effects into the equation. The latter is achieved by including a negative quadratic term on the right hand side of the equation~\cite{Deak:2012mx}.

\section*{Outlook}
For the purpose of seeing the size of the corrections induced by the kinematical constraint and the non-linear term in the CCFM and the BFKL equation we solve it on a grid by iteration with the initial condition ${\mathcal E}_0({\bf k})=1/(2|{\bf k}|)$. 

The correction induced by the kinematical constraint is relatively big especially for small ${\bf k}$ for the BFKL and the CCFM equation as well and cannot be neglected.

The non-linear term causes the amplitude to be suppressed for ${\bf  k}$ smaller than certain scale $Q_s$ which could be identified with the saturation scale. The size of the suppression depends on the constant parameter $R$ -- coefficient in front of the quadratic term. 

\begin{thebibliography}{9}
%\cite{Gribov:1984tu}
\bibitem{Gribov:1984tu} 
  L.~V.~Gribov, E.~M.~Levin and M.~G.~Ryskin,
  %``Semihard Processes in QCD,''
  Phys.\ Rept.\  {\bf 100}, 1 (1983);
  %%CITATION = PRPLC,100,1;%%
  %2225 citations counted in INSPIRE as of 02 Dec 2014
%\cite{Catani:1990eg}
  S.~Catani, M.~Ciafaloni and F.~Hautmann,
  %``High-energy factorization and small x heavy flavor production,''
  Nucl.\ Phys.\ B {\bf 366} (1991) 135.
  %%CITATION = NUPHA,B366,135;%%
  %805 citations counted in INSPIRE as of 02 Dec 2014

%\cite{Ciafaloni:1987ur}
\bibitem{Ciafaloni:1987ur}
  M.~Ciafaloni,
  %``Coherence Effects in Initial Jets at Small q**2 / s,''
  Nucl.\ Phys.\ B {\bf 296} (1988) 49;
  %%CITATION = NUPHA,B296,49;%%
  %613 citations counted in INSPIRE as of 02 Dec 2014
%\cite{Catani:1989sg}
  S.~Catani, F.~Fiorani and G.~Marchesini,
  %``Small x Behavior of Initial State Radiation in Perturbative QCD,''
  Nucl.\ Phys.\ B {\bf 336} (1990) 18;
  %%CITATION = NUPHA,B336,18;%%
  %560 citations counted in INSPIRE as of 02 Dec 2014
%\cite{Catani:1989yc}
  S.~Catani, F.~Fiorani and G.~Marchesini,
  %``QCD Coherence in Initial State Radiation,''
  Phys.\ Lett.\ B {\bf 234} (1990) 339.
  %%CITATION = PHLTA,B234,339;%%
  %490 citations counted in INSPIRE as of 02 Dec 2014

%%\cite{Deak:2009xt}
%\bibitem{Deak:2009xt}
%  M.~Deak, F.~Hautmann, H.~Jung and K.~Kutak,
%  %``Forward Jet Production at the Large Hadron Collider,''
%  JHEP {\bf 0909} (2009) 121
%  [arXiv:0908.0538 [hep-ph]].
%  %%CITATION = ARXIV:0908.0538;%%
%  %77 citations counted in INSPIRE as of 02 Dec 2014
%
%%\cite{Deak:2009ae}
%\bibitem{Deak:2009ae}
%  M.~Deak, F.~Hautmann, H.~Jung and K.~Kutak,
%  %``Jets in the forward region at the LHC,''
%  arXiv:0908.1870 [hep-ph].
%  %%CITATION = ARXIV:0908.1870;%%
%  %32 citations counted in INSPIRE as of 02 Dec 2014
%  
%%\cite{Deak:2010gk}
%\bibitem{Deak:2010gk}
%  M.~Deak, F.~Hautmann, H.~Jung and K.~Kutak,
%  %``Forward-Central Jet Correlations at the Large Hadron Collider,''
%  arXiv:1012.6037 [hep-ph].
%  %%CITATION = ARXIV:1012.6037;%%
%  %62 citations counted in INSPIRE as of 02 Dec 2014
%
%%\cite{Kutak:2012rf}
%\bibitem{Kutak:2012rf}
%  K.~Kutak and S.~Sapeta,
%  %``Gluon saturation in dijet production in p-Pb collisions at Large Hadron Collider,''
%  Phys.\ Rev.\ D {\bf 86} (2012) 094043
%  [arXiv:1205.5035 [hep-ph]].
%  %%CITATION = ARXIV:1205.5035;%%
%  %31 citations counted in INSPIRE as of 02 Dec 2014
%
%%\cite{Chatrchyan:2012gwa}
%\bibitem{Chatrchyan:2012gwa}
%  S.~Chatrchyan {\it et al.}  [CMS Collaboration],
%  %``Measurement of the inclusive production cross sections for forward jets and for dijet events with one forward and one central jet in $pp$ collisions at $\sqrt{s}=7$ TeV,''
%  JHEP {\bf 1206} (2012) 036
%  [arXiv:1202.0704 [hep-ex]].
%  %%CITATION = ARXIV:1202.0704;%%
%  %40 citations counted in INSPIRE as of 02 Dec 2014
%
%%\cite{Kutak:2008ed}
%\bibitem{Kutak:2008ed}
%  K.~Kutak and H.~Jung,
%  %``Saturation effects in final states due to CCFM with absorptive boundary,''
%  Acta Phys.\ Polon.\ B {\bf 40} (2009) 2063
%  [arXiv:0812.4082 [hep-ph]].
%  %%CITATION = ARXIV:0812.4082;%%
%  %16 citations counted in INSPIRE as of 02 Dec 2014
%
%%\cite{Avsar:2009pv}
%\bibitem{Avsar:2009pv}
%  E.~Avsar and E.~Iancu,
%  %``BFKL and CCFM evolutions with saturation boundary,''
%  Phys.\ Lett.\ B {\bf 673} (2009) 24
%  [arXiv:0901.2873 [hep-ph]].
%  %%CITATION = ARXIV:0901.2873;%%
%  %10 citations counted in INSPIRE as of 02 Dec 2014
%  
%%\cite{Avsar:2009pf}
%\bibitem{Avsar:2009pf}
%  E.~Avsar and E.~Iancu,
%  %``CCFM Evolution with Unitarity Corrections,''
%  Nucl.\ Phys.\ A {\bf 829} (2009) 31
%  [arXiv:0906.2683 [hep-ph]].
%  %%CITATION = ARXIV:0906.2683;%%
%  %26 citations counted in INSPIRE as of 02 Dec 2014
%  
%%\cite{Mueller:2002zm}
%\bibitem{Mueller:2002zm}
%  A.~H.~Mueller and D.~N.~Triantafyllopoulos,
%  %``The Energy dependence of the saturation momentum,''
%  Nucl.\ Phys.\ B {\bf 640} (2002) 331
%  [hep-ph/0205167].
%  %%CITATION = HEP-PH/0205167;%%
%  %284 citations counted in INSPIRE as of 02 dic 2014
%
%%\cite{Kutak:2011fu}
%\bibitem{Kutak:2011fu}
%  K.~Kutak, K.~Golec-Biernat, S.~Jadach and M.~Skrzypek,
%  %``Nonlinear equation for coherent gluon emission,''
%  JHEP {\bf 1202} (2012) 117
%  [arXiv:1111.6928 [hep-ph]].
%  %%CITATION = ARXIV:1111.6928;%%
%  %27 citations counted in INSPIRE as of 02 Dec 2014
%
%%\cite{Kutak:2012yr}
%\bibitem{Kutak:2012yr}
%  K.~Kutak,
%  %``Nonlinear extension of the CCFM equation,''
%  arXiv:1206.1223 [hep-ph].
%  %%CITATION = ARXIV:1206.1223;%%
%  %13 citations counted in INSPIRE as of 02 Dec 2014
%
%%\cite{Kutak:2012qk}
%\bibitem{Kutak:2012qk}
%  K.~Kutak,
%  %``Resummation in nonlinear equation for high energy factorisable gluon density and its extension to include coherence,''
%  JHEP {\bf 1212} (2012) 033
%  [arXiv:1206.5757 [hep-ph]].
%  %%CITATION = ARXIV:1206.5757;%%
%  %18 citations counted in INSPIRE as of 02 Dec 2014
%
%%\cite{Kutak:2013yga}
%\bibitem{Kutak:2013yga}
%  K.~Kutak and D.~Toton,
%  %``Gluon saturation scale from the KGBJS equation,''
%  JHEP {\bf 1311} (2013) 082
%  [arXiv:1306.3369 [hep-ph]].
%  %%CITATION = ARXIV:1306.3369;%%
%  %4 citations counted in INSPIRE as of 02 dic 2014
%
%%\cite{Balitsky:1995ub}
%\bibitem{Balitsky:1995ub}
%  I.~Balitsky,
%  %``Operator expansion for high-energy scattering,''
%  Nucl.\ Phys.\ B {\bf 463} (1996) 99
%  [hep-ph/9509348].
%  %%CITATION = HEP-PH/9509348;%%
%  %1063 citations counted in INSPIRE as of 02 Dec 2014
%
%%\cite{Kovchegov:1999yj}
%\bibitem{Kovchegov:1999yj}
%  Y.~V.~Kovchegov,
%  %``Small x F(2) structure function of a nucleus including multiple pomeron exchanges,''
%  Phys.\ Rev.\ D {\bf 60} (1999) 034008
%  [hep-ph/9901281].
%  %%CITATION = HEP-PH/9901281;%%
%  %941 citations counted in INSPIRE as of 02 Dec 2014
%
%%\cite{Kwiecinski:1995pu}
%\bibitem{Kwiecinski:1995pu}
%  J.~Kwiecinski, A.~D.~Martin and P.~J.~Sutton,
%  %``The gluon distribution at small x obtained from a unified evolution equation,''
%  Phys.\ Rev.\ D {\bf 52} (1995) 1445
%  [hep-ph/9503266].
%  %%CITATION = HEP-PH/9503266;%%
%  %65 citations counted in INSPIRE as of 02 Dec 2014
%
%%\cite{Kovchegov:2006wf}
%\bibitem{Kovchegov:2006wf}
%  Y.~V.~Kovchegov and H.~Weigert,
%  %``Quark loop contribution to BFKL evolution: Running coupling and leading-N(f) NLO intercept,''
%  Nucl.\ Phys.\ A {\bf 789} (2007) 260
%  [hep-ph/0612071].
%  %%CITATION = HEP-PH/0612071;%%
%  %77 citations counted in INSPIRE as of 02 Dec 2014
%
%%\cite{Deak:2012mx}
%\bibitem{Deak:2012mx}
%  M.~Deak,
%  %``Estimation of saturation and coherence effects in the KGBJS equation - a non-linear CCFM equation,''
%  JHEP {\bf 1307} (2013) 087
%  [arXiv:1209.6092 [hep-ph]].
%  %%CITATION = ARXIV:1209.6092;%%
%  %10 citations counted in INSPIRE as of 02 Dec 2014
%  
%%\cite{Kutak:2013kfa}
%\bibitem{Kutak:2013kfa}
%  K.~Kutak, W.~P\u0142aczek and D.~Toton,
%  %``Numerical solution of the integral form of the resummed Balitsky-Kovchegov equation,''
%  Acta Phys.\ Polon.\ B {\bf 44} (2013) 7,  1527
%  [arXiv:1303.0431 [hep-ph]].
%  %%CITATION = ARXIV:1303.0431;%%
%  %3 citations counted in INSPIRE as of 02 Dec 2014
%  
%%\cite{Kutak:2004ym}
%\bibitem{Kutak:2004ym}
%  K.~Kutak and A.~M.~Stasto,
%  %``Unintegrated gluon distribution from modified BK equation,''
%  Eur.\ Phys.\ J.\ C {\bf 41} (2005) 343
%  [hep-ph/0408117].
%  %%CITATION = HEP-PH/0408117;%%
%  %72 citations counted in INSPIRE as of 02 Dec 2014
%  
%%\cite{Avsar:2010ia}
%\bibitem{Avsar:2010ia}
%  E.~Avsar and A.~M.~Stasto,
%  %``Non-linear evolution in CCFM: The Interplay between coherence and saturation,''
%  JHEP {\bf 1006} (2010) 112
%  [arXiv:1005.5153 [hep-ph]].
%  %%CITATION = ARXIV:1005.5153;%%
%  %21 citations counted in INSPIRE as of 02 Dec 2014
%
%%\cite{Hautmann:2013tba}
%\bibitem{Hautmann:2013tba}
%  F.~Hautmann and H.~Jung,
%  %``Transverse momentum dependent gluon density from DIS precision data,''
%  Nucl.\ Phys.\ B {\bf 883} (2014) 1
%  [arXiv:1312.7875 [hep-ph]].
%  %%CITATION = ARXIV:1312.7875;%%
%  %4 citations counted in INSPIRE as of 14 Jul 2014
  
%\cite{Kwiecinski:1996td}
\bibitem{Kwiecinski:1996td} 
  J.~Kwiecinski, A.~D.~Martin and P.~J.~Sutton,
  %``Constraints on gluon evolution at small x,''
  Z.\ Phys.\ C {\bf 71}, 585 (1996)
  [hep-ph/9602320].
  %%CITATION = HEP-PH/9602320;%%
  %113 citations counted in INSPIRE as of 02 dic 2014
  
  %\cite{Deak:2012mx}
\bibitem{Deak:2012mx}
  M.~Deak,
  %``Estimation of saturation and coherence effects in the KGBJS equation - a non-linear CCFM equation,''
  JHEP {\bf 1307} (2013) 087
  [arXiv:1209.6092 [hep-ph]];
  %%CITATION = ARXIV:1209.6092;%%
  %10 citations counted in INSPIRE as of 02 Dec 2014
%\cite{Kutak:2013kfa}
  K.~Kutak, W.~P\-laczek and D.~Toton,
  %``Numerical solution of the integral form of the resummed Balitsky-Kovchegov equation,''
  Acta Phys.\ Polon.\ B {\bf 44} (2013) 7,  1527
  [arXiv:1303.0431 [hep-ph]].
  %%CITATION = ARXIV:1303.0431;%%
  %3 citations counted in INSPIRE as of 02 Dec 2014
  
\end{thebibliography}



==> lowX/DeakHQ/content_DeakHQ.tex <==
\title{The heavy quark impact factor and single heavy quark production}
\author{$^a$Michal De\'ak, $^b$Grigorios Chachamis, $^a$Germ\'an Rodrigo}
\affiliation{
$^a$Instituto de F\'isica Corpuscular, CSIC, Universitat de Valencia, E-46071 Valencia, Spain\\
$^b$Instituto de F\'isica Te\'orica UAM, CSIC and Universidad Aut\'onoma de Madrid, 
E-28049 Madrid, Spain}

\maketitle

\section*{Motivation}
The developments within the Balitsky-Fadin-Kuraev-Lipatov (BFKL) framework
for the resummation of  high center-of-mass energy logarithms~\cite{BFKL} made possible the phenomenological 
analysis of high energy scattering 
processes within the $k_T$-factorization scheme. 
A key ingredient for studying high energy scattering processes within the
$k_T$-factorisation scheme is the impact factor.
The impact factors for gluons and massless quarks have been
calculated at NL$x$ accuracy. 
The bottom quark became a suitable probe for QCD physics whereas the the LHC experiments are very efficient in tagging the $b$-quark. In addition the LHC could be considered to be a $b$-factory.
Advantages connected with studying heavy quarks can be used to learn more about the small-$x$ physics.
The NL$x$ impact factor for a massive quark in the initial state has been 
calculated in Ref.~\cite{Ciafaloni:2000sq}.
We may apply mass corrections calculated 
in~\cite{Ciafaloni:2000sq} to calculate the cross section of 
single heavy quark production in proton-proton scattering at the LHC collision 
energies.

\section*{Single heavy quark production}
A good starting point for the solution of the above problem is to first
calculate the cross section without the mass corrections. We can focus on a
region of phase space where the mass corrections are relatively negligible, for
${\bf k}^2\gg m_{Q}^2$. We apply the scheme used in~\cite{Hentschinski:2012kr}. We replace the photon impact factor in~\cite{Hentschinski:2012kr} with the quark impact factor to obtain the heavy quark-proton scattering cross section $\sigma_{pQ}$. To obtain the $pp$ scattering cross section we have to convolute $\sigma_{pQ}$ with the bottom quark parton distribution function. Using the framework above, we have calculated the transversal momentum distribution of the final state $b$-quark and compared it with a similar calculation done with the Monte Carlo program {\sc Pythia}~\cite{Sjostrand:2014zea}. Both obtained cross sections agree well in the range of transversal momentum $30\;GeV<{\bf k}<140\;GeV$ and rapidity $2<y<2.4$.

\begin{thebibliography}{9}
\bibitem{BFKL}  
L.~N.~Lipatov, 
Sov.\ J.\ Nucl.\ Phys.\  {\bf 23} (1976) 338;
%%CITATION = YAFIA,23,642;%%
%
E.~A.~Kuraev, L.~N.~Lipatov, V.~S.~Fadin,
Phys.\ Lett.\  B {\bf 60} (1975) 50, 
%%CITATION = PHLTA,B60,50;%%
Sov.\ Phys.\ JETP {\bf 44} (1976) 443,
%%CITATION = ZETFA,71,840;%%
Sov.\ Phys.\ JETP {\bf 45} (1977) 199;
%%CITATION = ZETFA,72,377;%%
%
%Ia.~Ia.~Balitsky, L.~N.~Lipatov, 
%Sov.\ J.\ Nucl.\ Phys.\  {\bf 28} (1978) 822;
%%%CITATION = YAFIA,28,1597;%%
%%\cite{Fadin:1993qb}
%V.~S.~Fadin, L.~N.~Lipatov, Phys.\ Lett.\  B {\bf 429} (1998) 127 [hep-ph/9802290];
%%%CITATION = PHLTA,B429,127;%%
%%
%%\bibitem{Ciafaloni:1998gs}
% M.~Ciafaloni, G.~Camici, Phys.\ Lett.\  B {\bf 430} (1998) 349 [hep-ph/9803389].
%  %%CITATION = PHLTA,B430,349;%%


%\cite{Ciafaloni:1998hu}
\bibitem{Ciafaloni:1998hu} 
  M.~Ciafaloni and D.~Colferai,
  %``K factorization and impact factors at next-to-leading level,''
  Nucl.\ Phys.\ B {\bf 538}, 187 (1999)
  [hep-ph/9806350].
  %%CITATION = HEP-PH/9806350;%%
  
%  %\cite{Mueller:1986ey}
%\bibitem{Mueller:1986ey}
%  A.~H.~Mueller and H.~Navelet,
%  %``An Inclusive Minijet Cross-Section and the Bare Pomeron in QCD,''
%  Nucl.\ Phys.\ B {\bf 282} (1987) 727.
%  %%CITATION = NUPHA,B282,727;%%
%  %315 citations counted in INSPIRE as of 30 Jun 2013
%
%%\cite{Vera:2007kn}
%\bibitem{Vera:2007kn}
%  A.~Sabio Vera and F.~Schwennsen,
%  %``The Azimuthal decorrelation of jets widely separated in rapidity as a test of the BFKL kernel,''
%  Nucl.\ Phys.\ B {\bf 776} (2007) 170
%  [hep-ph/0702158 [HEP-PH]].
%  %%CITATION = HEP-PH/0702158;%%
%  %69 citations counted in INSPIRE as of 02 Jul 2013
%  
%\cite{Kwiecinski:2001nh}
\bibitem{Kwiecinski:2001nh}
  J.~Kwiecinski, A.~D.~Martin, L.~Motyka and J.~Outhwaite,
  %``Azimuthal decorrelation of forward and backward jets at the Tevatron,''
  Phys.\ Lett.\ B {\bf 514} (2001) 355
  [hep-ph/0105039].
  %%CITATION = HEP-PH/0105039;%%
  %17 citations counted in INSPIRE as of 02 Jul 2013

%\cite{Ciafaloni:2000sq}
\bibitem{Ciafaloni:2000sq}
  M.~Ciafaloni and G.~Rodrigo,
  %``Heavy quark impact factor at next-to-leading level,''
  JHEP {\bf 0005} (2000) 042
  [hep-ph/0004033];
  %%CITATION = HEP-PH/0004033;%%
  G.~Chachamis, M.~Deak and G.~Rodrigo,
  %``Heavy quark impact factor in kT-factorization,''
  JHEP {\bf 1312} (2013) 066
  [arXiv:1310.6611].
  %%CITATION = ARXIV:1310.6611;%%
  %3 citations counted in INSPIRE as of 28 Nov 2014
  
  %\cite{Hentschinski:2012kr}
\bibitem{Hentschinski:2012kr}
  M.~Hentschinski, A.~Sabio Vera and C.~Salas,
  %``The hard to soft Pomeron transition in small x DIS data using optimal renormalization,''
  Phys.\ Rev.\ Lett.\  {\bf 110} (2013) 041601
  [arXiv:1209.1353 [hep-ph]].
  %%CITATION = ARXIV:1209.1353;%%
  %23 citations counted in INSPIRE as of 18 Dec 2014

%\cite{Sjostrand:2014zea}
\bibitem{Sjostrand:2014zea}
  T.~Sj\"ostrand, S.~Ask, J.~R.~Christiansen, R.~Corke, N.~Desai, P.~Ilten, S.~Mrenna and S.~Prestel {\it et al.},
  %``An Introduction to PYTHIA 8.2,''
  arXiv:1410.3012 [hep-ph].
  %%CITATION = ARXIV:1410.3012;%%
  %6 citations counted in INSPIRE as of 18 Dec 2014

\end{thebibliography}



==> lowX/Ducloue/content_Ducloue.tex <==
\title{High-energy resummation effects in Mueller-Navelet jets production at the LHC}
\author{Bertrand Duclou\'e$^1$, Lech Szymanowski$^2$, Samuel Wallon$^{3,4}$}
\affiliation{$^1$Department of Physics, University of Jyv\"askyl\"a, P.O. Box 35, 40014 University of Jyv\"askyl\"a, Finland \\
             $^2$National Centre for Nuclear Research (NCBJ), Warsaw, Poland \\
             $^3$LPT, Universit{\'e} Paris-Sud, CNRS, 91405, Orsay, France \\
             $^4$UPMC Univ. Paris 06, Facult\'e de Physique, 4 place Jussieu, 75252 Paris Cedex 05, France}

\maketitle


The high energy limit of QCD, described by the Balitsky-Fadin-Kuraev-Lipatov (BFKL)
approach~\cite{Fadin:1975cb,Kuraev:1976ge,Kuraev:1977fs,Balitsky:1978ic}, has been the subject of many studies since four decades. One of the most promising processes to study these dynamics at hadron colliders was proposed by Mueller and Navelet~\cite{Mueller:1986ey}.
Consider two jets  separated by a large rapidity interval, i.e. each of them almost fly in the direction of the hadron ``close'' to it, and with similar transverse
momenta. Besides the cross-section, much information on the QCD high-energy resummation effects can be obtained when studying the azimuthal correlations of the two jets~\cite{DelDuca:1993mn,Stirling:1994zs}.
In a pure leading order (LO) collinear treatment, the two jets should be emitted back to back since there is no phase space for (untagged) emission between them. This simple picture is of course corrected by the inclusion of radiative corrections.
On the other hand, in the high-energy limit, the multiple emission of semi-hard gluons between these two jets is expected to modify dramatically this picture, leading to enhanced cross-sections and strong decorrelation effects. However, it is known that passing from a leading logarithmic (LL) to a next-to-leading-logarithmic (NLL) treatment in the BFKL framework can modify significantly this picture. 

Technically,
such a BFKL treatment involves two building blocks:
 the jet 
vertex, which describes the transition from an incoming parton to a jet,
and the Green's function, which describes the pomeron exchange between the vertices. A complete NLL BFKL analysis of Mueller-Navelet jets (for more details, see refs.~\cite{Ducloue:2013hia,Ducloue:2013bva}), including the NLL corrections both to the Green's function~\cite{Fadin:1998py,Ciafaloni:1998gs} and to
the jet vertex~\cite{Ciafaloni:1998kx,Ciafaloni:1998hu,Bartels:2001ge,Bartels:2002yj,Caporale:2011cc,Hentschinski:2011tz,Chachamis:2012cc}, showed that the NLL corrections to the jet vertex have a very large effect, of the same order of magnitude as the NLL corrections to the Green's function~\cite{Vera:2007kn,Marquet:2007xx}, leading to a lower cross-section and a much larger azimuthal correlation~\cite{Colferai:2010wu}. However, these results are very dependent on the choice
of the scales, especially the renormalization scale $\mu_R$ and the
factorization scale $\mu_F$, in particular in the case of realistic kinematical cuts for LHC experiments~\cite{Ducloue:2013hia}. This dependency can be reduced by using the Brodsky-Lepage-Mackenzie (BLM) prescription~\cite{Brodsky:1982gc}, adapted to the resummed perturbation theory \`a la BFKL~\cite{Brodsky:1998kn,Brodsky:2002ka}, to fix the renormalization scale. Such a full NLL BFKL analysis supplemented by the BLM scale fixing procedure has been performed~\cite{Ducloue:2013bva},
leading to a very satisfactory description of
the most recent LHC data extracted by the CMS collaboration
for the azimuthal correlations of Mueller-Navelet jets at a center-of-mass energy $\sqrt{s}=7$ TeV~\cite{CMS-PAS-FSQ-12-002}.
Recently, it was shown that energy-momentum non conservation should not affect this NLL BFKL analysis significantly~\cite{Ducloue:2014koa}.

In the very large center-of-mass energy of the LHC, the contributions
of partons with very small $x$ fraction of the protons are dominating, and their distributions are therefore enhanced. This is a typical situation where multipartonic scattering contributions could be sizable, in particular when dealing with small transverse momenta of the tagged jets (which hopefully will become accessible at CMS and ATLAS) for which the usual twist suppression is not valid~\cite{Diehl:2011yj}.
In such a situation, the cross-section gets an additional contribution where each jet is emitted by a separate BFKL chain.
The exchange of two BFKL ladders is presumably the dominant contribution for asymptotical values of $s$, and it would be of great interest to determine at which point it starts to be of the same order of magnitude as the exchange of a single ladder.
Thus, the study of this process with transverse momenta of the tagged jets as low as possible would be a great opportunity towards investigating the effect of 
multipartonic contributions at small $x$.


\begin{thebibliography}{9}

\providecommand{\href}[2]{#2}

\bibitem{Fadin:1975cb}
V.~S. Fadin, E.~A. Kuraev, and L.~N. Lipatov, {\it {On the {P}omeranchuk
  Singularity in Asymptotically Free Theories}},  {\em Phys. Lett.} {\bf B60}
  (1975) 50--52.

\bibitem{Kuraev:1976ge}
E.~A. Kuraev, L.~N. Lipatov, and V.~S. Fadin, {\it {Multi - Reggeon Processes
  in the {Y}ang-{M}ills Theory}},  {\em Sov. Phys. JETP} {\bf 44} (1976)
  443--450.

\bibitem{Kuraev:1977fs}
E.~A. Kuraev, L.~N. Lipatov, and V.~S. Fadin, {\it {The Pomeranchuk Singularity
  in Nonabelian Gauge Theories}},  {\em Sov. Phys. JETP} {\bf 45} (1977)
  199--204.

\bibitem{Balitsky:1978ic}
I.~I. Balitsky and L.~N. Lipatov, {\it {The Pomeranchuk Singularity in Quantum
  Chromodynamics}},  {\em Sov. J. Nucl. Phys.} {\bf 28} (1978) 822--829.

\bibitem{Mueller:1986ey}
A.~H. Mueller and H.~Navelet, {\it {An Inclusive Minijet Cross-Section and the
  Bare Pomeron in QCD}},  {\em Nucl. Phys.} {\bf B282} (1987) 727.

\bibitem{DelDuca:1993mn}
V.~Del~Duca and C.~R. Schmidt, {\it {Dijet production at large rapidity
  intervals}},  {\em Phys. Rev.} {\bf D49} (1994) 4510--4516,
  [\href{http://xxx.lanl.gov/abs/hep-ph/9311290}{{\tt hep-ph/9311290}}].

\bibitem{Stirling:1994zs}
W.~J. Stirling, {\it Production of jet pairs at large relative rapidity in
  hadron hadron collisions as a probe of the perturbative {P}omeron},  {\em
  Nucl. Phys.} {\bf B423} (1994) 56--79,
  [\href{http://xxx.lanl.gov/abs/hep-ph/9401266}{{\tt hep-ph/9401266}}].

\bibitem{Ducloue:2013hia}
B.~Duclou\'e, L.~Szymanowski, and S.~Wallon, {\it {Confronting Mueller-Navelet
  jets in NLL BFKL with LHC experiments at 7 TeV}},  {\em JHEP} {\bf 1305}
  (2013) 096, [\href{http://xxx.lanl.gov/abs/1302.7012}{{\tt
  arXiv:1302.7012}}].

\bibitem{Ducloue:2013bva}
B.~Duclou\'e, L.~Szymanowski, and S.~Wallon, {\it {Evidence for high-energy
  resummation effects in Mueller-Navelet jets at the LHC}},  {\em Phys. Rev.
  Lett.} {\bf 112} (2014) 082003,
  [\href{http://xxx.lanl.gov/abs/1309.3229}{{\tt arXiv:1309.3229}}].

\bibitem{Fadin:1998py}
V.~S. Fadin and L.~N. Lipatov, {\it {BFKL pomeron in the next-to-leading
  approximation}},  {\em Phys. Lett.} {\bf B429} (1998) 127--134,
  [\href{http://xxx.lanl.gov/abs/hep-ph/9802290}{{\tt hep-ph/9802290}}].

\bibitem{Ciafaloni:1998gs}
M.~Ciafaloni and G.~Camici, {\it {Energy scale(s) and next-to-leading BFKL
  equation}},  {\em Phys. Lett.} {\bf B430} (1998) 349--354,
  [\href{http://xxx.lanl.gov/abs/hep-ph/9803389}{{\tt hep-ph/9803389}}].

\bibitem{Ciafaloni:1998kx}
M.~Ciafaloni, {\it {Energy scale and coherence effects in small x equations}},
  {\em Phys. Lett.} {\bf B429} (1998) 363--368,
  [\href{http://xxx.lanl.gov/abs/hep-ph/9801322}{{\tt hep-ph/9801322}}].

\bibitem{Ciafaloni:1998hu}
M.~Ciafaloni and D.~Colferai, {\it {K factorization and impact factors at
  next-to-leading level}},  {\em Nucl. Phys.} {\bf B538} (1999) 187--214,
  [\href{http://xxx.lanl.gov/abs/hep-ph/9806350}{{\tt hep-ph/9806350}}].

\bibitem{Bartels:2001ge}
J.~Bartels, D.~Colferai, and G.~P. Vacca, {\it {The NLO jet vertex for
  Mueller-Navelet and forward jets: The quark part}},  {\em Eur. Phys. J.} {\bf
  C24} (2002) 83--99, [\href{http://xxx.lanl.gov/abs/hep-ph/0112283}{{\tt
  hep-ph/0112283}}].

\bibitem{Bartels:2002yj}
J.~Bartels, D.~Colferai, and G.~P. Vacca, {\it {The NLO jet vertex for
  Mueller-Navelet and forward jets: The gluon part}},  {\em Eur. Phys. J.} {\bf
  C29} (2003) 235--249, [\href{http://xxx.lanl.gov/abs/hep-ph/0206290}{{\tt
  hep-ph/0206290}}].

\bibitem{Caporale:2011cc}
F.~Caporale, D.~Y. Ivanov, B.~Murdaca, A.~Papa, and A.~Perri, {\it {The
  next-to-leading order jet vertex for Mueller-Navelet and forward jets
  revisited}},  {\em JHEP} {\bf 1202} (2012) 101,
  [\href{http://xxx.lanl.gov/abs/1112.3752}{{\tt arXiv:1112.3752}}].

\bibitem{Hentschinski:2011tz}
M.~Hentschinski and A.~Sabio~Vera, {\it {NLO jet vertex from Lipatov's QCD
  effective action}},  {\em Phys. Rev.} {\bf D85} (2012) 056006,
  [\href{http://xxx.lanl.gov/abs/1110.6741}{{\tt arXiv:1110.6741}}].

\bibitem{Chachamis:2012cc}
G.~Chachamis, M.~Hentschinski, J.~D. Madrigal, and A.~Sabio~Vera, {\it {NLO
  corrections to the gluon induced forward jet vertex from the high energy
  effective action}},  {\em Phys. Rev.} {\bf D87} (2013) 076009,
  [\href{http://xxx.lanl.gov/abs/1212.4992}{{\tt arXiv:1212.4992}}].

\bibitem{Vera:2007kn}
A.~Sabio~Vera and F.~Schwennsen, {\it The azimuthal decorrelation of jets
  widely separated in rapidity as a test of the {BFKL} kernel},  {\em Nucl.
  Phys.} {\bf B776} (2007) 170--186,
  [\href{http://xxx.lanl.gov/abs/hep-ph/0702158}{{\tt hep-ph/0702158}}].

\bibitem{Marquet:2007xx}
C.~Marquet and C.~Royon, {\it {Azimuthal decorrelation of Mueller-Navelet jets
  at the Tevatron and the LHC}},  {\em Phys. Rev.} {\bf D79} (2009) 034028,
  [\href{http://xxx.lanl.gov/abs/0704.3409}{{\tt arXiv:0704.3409}}].

\bibitem{Colferai:2010wu}
D.~Colferai, F.~Schwennsen, L.~Szymanowski, and S.~Wallon, {\it {Mueller
  Navelet jets at LHC - complete NLL BFKL calculation}},  {\em JHEP} {\bf 12}
  (2010) 026, [\href{http://xxx.lanl.gov/abs/1002.1365}{{\tt
  arXiv:1002.1365}}].

\bibitem{Brodsky:1982gc}
S.~J. Brodsky, G.~P. Lepage, and P.~B. Mackenzie, {\it {On the Elimination of
  Scale Ambiguities in Perturbative {Q}uantum {C}hromodynamics}},  {\em Phys.
  Rev.} {\bf D28} (1983) 228.

\bibitem{Brodsky:1998kn}
S.~J. Brodsky, V.~S. Fadin, V.~T. Kim, L.~N. Lipatov, and G.~B. Pivovarov, {\it
  The {{QCD}} pomeron with optimal renormalization},  {\em JETP Lett.} {\bf 70}
  (1999) 155--160, [\href{http://xxx.lanl.gov/abs/hep-ph/9901229}{{\tt
  hep-ph/9901229}}].

\bibitem{Brodsky:2002ka}
S.~J. Brodsky, V.~S. Fadin, V.~T. Kim, L.~N. Lipatov, and G.~B. Pivovarov, {\it
  High-energy {QCD} asymptotics of photon photon collisions},  {\em JETP Lett.}
  {\bf 76} (2002) 249--252, [\href{http://xxx.lanl.gov/abs/hep-ph/0207297}{{\tt
  hep-ph/0207297}}].

\bibitem{CMS-PAS-FSQ-12-002}
{CMS Collaboration}, {\it {Azimuthal angle decorrelations of jets widely
  separated in rapidity in pp collisions at $\sqrt{s}=7$ TeV}},  CMS Physics
  Analysis Summary CMS-PAS-FSQ-12-002, 2013.

\bibitem{Ducloue:2014koa}
B.~Duclou\'e, L.~Szymanowski, and S.~Wallon, {\it {Violation of
  energy–momentum conservation in Mueller-Navelet jets production}},  {\em
  Phys. Lett.} {\bf B738} (2014) 311--316,
  [\href{http://xxx.lanl.gov/abs/1407.6593}{{\tt arXiv:1407.6593}}].

\bibitem{Diehl:2011yj}
M.~Diehl, D.~Ostermeier, and A.~Schafer, {\it {Elements of a theory for
  multiparton interactions in QCD}},  {\em JHEP} {\bf 1203} (2012) 089,
  [\href{http://xxx.lanl.gov/abs/1111.0910}{{\tt arXiv:1111.0910}}].

\end{thebibliography}



==> lowX/Goerlich/content_Goerlich.tex <==
\title{Dijet production at HERA and tests of QCD factorisation}
\author{Lidia Goerlich\\on behalf of the H1 and ZEUS Collaborations }
\affiliation{Institute of Nuclear Physics\\Polish Academy of Sciences}

\maketitle

%\section{Open problems}
\section*{Exclusive dijet production in diffractive DIS}

The exclusive production of dijets in diffractive deep inelastic lepton-proton 
scattering has been measured by the ZEUS Collaboration 
for the first time at HERA \cite{ZEUS}.
Jets have been reconstructed in the virtual 
photon-Pomeron  centre-of-mass system frame using the exclusive 
$k_T$ algorithm. The cross section for the exclusive production of 
dijets is given as a function of the azimuthal angle $\phi$ between the plane defined
by exchanged photon and dijet system and the plane defined by the
incoming and scattered lepton momenta in the $\gamma^*$-Pomeron rest frame. 
The shape of the $\phi$ distribution is sensitive to the production mechanism
of diffractive exclusive dijets. The data favour fully perturbative calculations 
of the two-gluon exchange model over boson-gluon fusion mechanism, in which a partonic
structure of the Pomeron is assumed.

\section*{Tests of QCD factorisation}

In the framework of  QCD collinear factorisation the cross section for 
the diffractive DIS process factorises into universal diffractive 
parton distribution functions (DPDFs) and hard subrocess cross sections calculable 
within the perturbative approach. The universality of these DPDFs was sucessfully 
tested for hard diffractive DIS production.
% of dijet and charm.
However, the factorisation breaking was observed for hard processes in diffractive
hadron-hadron scattering where the predictions based on HERA DPDFs overestimate
the data, at Tevatron by about one order of magnitude. The factorisation breaking 
is usually explained 
in terms of multiple scattering effects, which occur in the presence
of beam remnants and lead to the destruction of the rapidity gap associated 
with the diffractive process. Rapidity gap survival effects can be investigated 
at HERA in hard diffractive dijet photoproduction. 

Diffractive dijet cross sections in photoproduction and in DIS
with a leading proton detected in the very forward proton spectrometer (VFPS) 
have been measured by H1 \cite{H1_01}. 
DIS measurements are complemented by measurements of dijet production with an
associated large rapidity gap (LRG) \cite{H1_02}. 
The cross sections for the dijet production  in diffractive DIS with VFPS  
and with LRG are found
to be well described by the NLO QCD predictions using the H12006 Fit-B DPDF set. 
These results confirm the validity of QCD factorisation in 
hard diffractive DIS.
  
Using the VFPS data the double ratio of measured to predicted cross sections in 
photoproduction to the corresponding ratio in DIS has been determined and 
its value is equal to $0.55 \pm 0.10(\rm data)+0.02(\rm theor.)$, with no significant
kinematic dependence. This result is consistent with previous H1 measurements based on the LRG method
and indicates that QCD factorisation may be broken in diffractive dijet photoproduction.
However, ZEUS does not observe factorisation breaking in diffractive photoproduced jets.

\begin{thebibliography}{9}
\bibitem{ZEUS}
  M. Guzik, Proceedings PoS (DIS2014) 070. 
%  M. Guzik (\emph{on behalf of the ZEUS Collaboration}), Proceedings PoS (DIS2014) 070. 
\bibitem{H1_01}
  R. Zlebcik, Proceedings PoS (DIS2014) 072. 
\bibitem{H1_02}
 V. Andreev et al. [H1 Collaboration], DESY 14-200. 
%\bibitem{lamport03}
 % Leslie Lamport, \emph{\LaTeX: a document preparation system}. Addison Wesley, Massachusetts, 2nd edition, 1994.

\end{thebibliography}



==> lowX/Hameren/content_Hameren.tex <==
\title{Compact expressions for off-shell amplitudes}
\author{Andreas van Hameren}
\affiliation{Institute of Nuclear Physics, Polish Academy of Sciences}

\maketitle

\newcommand{\lid}[2]{#1\!\cdot\!#2}
%
% These allow for the separation of the process-dependent ingredients, which are calculable perturbatively, from the universal ingredients, which must at least partly be determined from experimental data.
% %
% 
% The process dependent ingredients are given by {\em scattering amplitudes\/}.
% %
Within {\em collinear factorization\/}, the momenta of the particles and partons associated with the hard scattering amplitude are on-shell, and the amplitude is defined applying the Lehmann Symanzik Zimmermann reduction prescription on a connected Green function.
%
For a gauge theory like quantum chromo dynamics (QCD), this approach ensures the necessary gauge invariance.
%
For {\em high-energy factorization\/} or {\em $k_T$-factorization}~%
%\cite{Gribov:1984tu,Catani:1990eg,Collins:1991ty,Catani:1994sq},
\cite{Gribov:1984tu},
however, the initial-state momenta need to be off-shell, and the above approach cannot be applied directly.
%

There exist a few approaches in literature to define and calculate scattering amplitudes with off-shell partons.
%
One of them uses an effective action, which introduces new fields representing the off-shell partons with given longitudinal momentum associated with them~%
%\cite{Lipatov:1995pn,Antonov:2004hh}.
\cite{Lipatov:1995pn}.
%
They enter the QCD Lagrangian via terms similar to Wilson lines, ensuring gauge invariance of the eventual scattering amplitudes involving these fields.
%

In another approach~\cite{vanHameren:2012if}, which is more suitable for automated numerical implementations, the initial-state off-shell partons are replaced by auxiliary on-shell quarks, and auxiliary on-shell quarks or photons are added to the final state.
%
The on-shellness insures a gauge invariant definition of the amplitude, and the eikonal Feynman rules the auxiliary quarks turn out to follow lead to the same amplitudes as the the effective action approach.
%

In~\cite{Kotko:2014aba}, finally, a manifestly gauge invariant and constructive definition of scattering amplitudes with an arbitrary number of off-shell external gluons was presented, by considering matrix elements of Fourier transforms of straight infinite Wilson line operators associated with the off-shell external gluons.
%
In this work, it becomes particularly clear that the key to gauge invariance is the association of a {\em direction\/} $p^\mu$ with each off-shell external momentum~$k^\mu$, which satisfies~$\lid{p}{k}=0$.
%
With each direction, an eikonal line is associated.
%

Using the latter approach as a staring point, it has been demonstrated in~\cite{vanHameren:2014iua} how tree-level multi-gluon amplitudes with an arbitrary number of them off-shell can be calculated via Britto Cachazo Feng Witten (BCFW) recursion~%
%\cite{Britto:2004ap,Britto:2005fq}.
\cite{Britto:2004ap}.
%
The BCFW method leads to very compact expressions with relatively little effort for helicity amplitudes with only on-shell partons.
%
In~\cite{vanHameren:2014iua} a straightforward generalization of BCFW recursion has been established, allowing again for compact expressions with relatively little effort.
%
In particular, helicity amplitudes for up to $4$ gluons have been calculated with up to $3$ of them off-shell, and the MHV formulas have been shown to hold for arbitrary number of gluons with up to $2$ of them off-shell.
%
Further generalization to quarks and the calculation of all $5$-parton helicity amplitudes with up to $2$ of them off-shell is in progress.

{\small
\begin{thebibliography}{9}
\bibitem{Gribov:1984tu}
L.~Gribov, E.~Levin, and M.~Ryskin,   {\em
  Phys.Rept.} {\bf 100} (1983) 1--150.\\
%
%\bibitem{Catani:1990eg}
S.~Catani, M.~Ciafaloni, and F.~Hautmann,   {\em Nucl.Phys.} {\bf B366} (1991)
  135--188.\\
%
%\bibitem{Collins:1991ty}
J.~C. Collins and R.~K. Ellis,   {\em Nucl.Phys.} {\bf B360} (1991) 3--30.
%

\bibitem{Lipatov:1995pn}
L.~Lipatov,   {\em Nucl.Phys.} {\bf B452} (1995) 369--400.\\
%
%\bibitem{Antonov:2004hh}
E.~Antonov, L.~Lipatov, E.~Kuraev, and I.~Cherednikov,   {\em Nucl.Phys.} {\bf B721} (2005) 111--135.\\
%
%\bibitem{Lipatov:2000se}
L.~Lipatov and M.~Vyazovsky,   {\em Nucl.Phys.} {\bf B597} (2001) 399--409.

\bibitem{vanHameren:2012if}
A.~van Hameren, P.~Kotko, and K.~Kutak,   {\em JHEP} {\bf 1301} (2013) 078.\\
%
%\bibitem{vanHameren:2013csa}
A.~van Hameren, K.~Kutak, and T.~Salwa,   {\em Phys.Lett.} {\bf B727} (2013) 226--233.

\bibitem{Kotko:2014aba}
P.~Kotko,
  %``Wilson lines and gauge invariant off-shell amplitudes,''
  {\em JHEP} {\bf 1407} (2014) 128.

\bibitem{vanHameren:2014iua}
  A.~van Hameren,
  %``BCFW recursion for off-shell gluons,''
  {\em JHEP} {\bf 1407} (2014) 138.

\bibitem{Britto:2004ap}
R.~Britto, F.~Cachazo, and B.~Feng,   {\em Nucl.Phys.} {\bf B715} (2005) 499--522.\\
%
%\bibitem{Britto:2005fq}
R.~Britto, F.~Cachazo, B.~Feng, and E.~Witten,   {\em Phys.Rev.Lett.} {\bf 94}
  (2005) 181602.

\end{thebibliography}
}


==> lowX/Knutsson/content_Knutsson.tex <==
\title{Production of leading charged particles and leading charged-particle jets at small transverse momenta with the CMS detector}
\author{Albert Knutsson on behalf of the CMS collaboration}
\affiliation{Antwerpen University, Belgium}

\maketitle

\noindent Normalized cross-sections of leading charged particles and charged-particle jets are measured in proton-proton low pileup data at $\sqrt{s} = 8$ TeV, where "leading" refers to the single particle or single jet with the highest transverse momentum in each event, in data collected with the CMS detector at the CERN LHC. 
The particles and jets are measured, respectively, in pseudorapidity ranges of $|\eta|< 2.4$ and  $|\eta| < 1.9$ for
transverse momenta $p_{\mathrm{T}} > 0.8$~GeV and $p_{\mathrm{T}} > 1.0$~GeV. The measured yields integrated above a given minimum transverse 
momentum, $p_{\mathrm{T, min}}$, provide information of how parton-parton cross section calculations 
can be improved when used in low-$p_{\mathrm{T}}$
nonperturbative regimes. Comparison of data with predictions from models as implemented in various event generators shows that the measured observable is sensitive to key aspects in the transition between soft and hard QCD physics. The results are shown in Figure~\ref{fig:results}.
 \vspace{-0.2cm}
\begin{figure}[h!]
  \begin{center}
  \includegraphics[width=0.36\textwidth]{lowX/Knutsson/knutsson_fig1a.eps}
  \includegraphics[width=0.36\textwidth]{lowX/Knutsson/knutsson_fig1b.eps} \\
    \includegraphics[width=0.36\textwidth]{lowX/Knutsson/knutsson_fig2a.eps}
    \includegraphics[width=0.36\textwidth]{lowX/Knutsson/knutsson_fig2b.eps}
 \vspace{-0.6cm} { \caption{Normalised integrated $p_T$-distribution of the leading charged particle in $|\eta|<2.4$ (upper) and the leading charged jet in $|\eta|<1.9$ (lower). 
  The data are compared to different predictions from various {\sc Pythia}6 tunes (left) and various
Monte Carlo event generators (right).  The error bars indicate the statistical uncertainty and the shaded area the systematic uncertainty. The Monte Carlo curves for the leading particles and the leading jets are normalised to the measured value of $\sigma(p_{\mathrm{T\,leading~ch. particle}} > 9.0 \textrm{ GeV}) / \sigma_{vis}$ and $\sigma(p_{\mathrm{T\,leading~ch. particle}} > 14.3 \textrm{ GeV}) / \sigma_{vis}$, respectively, where $\sigma_{vis}$ is defined by the number of events with at least one charged particle with  $|\eta|<2.4$ and $p_t > 0.4$ GeV. }
 \label{fig:results}}
  \end{center}
\end{figure}

% \begin{thebibliography}{9}
% \bibitem{lamport94}
%  Leslie Lamport, \emph{\LaTeX: a document preparation system}. Addison Wesley, Massachusetts, 2nd edition, 1994.
% \end{thebibliography}



==> lowX/Kotko/content_Kotko.tex <==
\title{New results on forward jets within
High Energy Factorization}
\author{Piotr Kotko$^\dagger$}
\affiliation{\it Penn State University, University Park, PA 16802, USA}

\maketitle

\section*{High Energy Factorization and Off-shell Amplitudes}

\let\thefootnote\relax\footnote{$^\dagger$ in collaboration with A. van Hameren, K. Kutak and S. Sapeta}
In the High Energy Factorization (HEF) approach for forward particle production, a cross section 
is expressed as a convolution of unintegrated gluon density (UGD), collinear PDFs,
and off-shell gauge invariant tree-level partonic cross section. Generally, UGD undergoes BFKL-like evolution, possibly taking into account subleading corrections.
Construction of off-shell gauge invariant matrix elements is achieved by taking the Lipatov's effective action, or one of the
approaches \cite{vanHameren:2012if,vanHameren:2012uj} which are more suitable for a numerical calculation. In the present contribution we discussed one more approach based on the Wilson lines \cite{Kotko:2014aba},
which is more general and 
aims at constructing gauge invariant Green's functions with arbitrary number of off-shell legs. 
%It was implemented in a $\mathtt{form}$
%program $\mathtt{OGIME}$ (Off-shell Gauge Invariant Matrix Elements) devoted to calculate amplitudes analytically.

\section*{Forward jets at LHC}
Here we have concentrated on two recent studies within HEF: central-forward dijet production~\cite{vanHameren:2014ala} and $Z_0$+jet production at LHC. The sample results for the azimuthal decorrelations are shown in Fig.~1. The UGD that has been used here is the one described in \cite{Kutak:2012rf} and abbreviated here as KS. It utilizes BFKL type evolution with kinematic constraint, DGLAP corrections and nonlinear BK term. This UGD has been supplemented with a hard scale dependence via the Sudakov form factor as described in \cite{vanHameren:2014ala} (a similar model  
\cite{Kutak:2014wga} leads to similar results for the observables under study). This Sudakov-type resummation turns out to be important to have a reasonable agreement with the data. For the $Z_0$+jet production we recover correctly the normalized distributions, while the absolute cross sections are significantly smaller than the experimental ones, which may give a hint that MPIs should be incorporated in HEF.

\begin{figure}[h]
%  \begin{center}
\parbox{0.65\textwidth}{
%    \includegraphics[height=0.18\textheight]{lowX/Kotko/pp_dphi_7TeV_KSsud_vsCMS.eps}
%    \includegraphics[height=0.18\textheight]{lowX/Kotko/Z0jet_KSsud_dphi.eps}
        \includegraphics[height=0.18\textheight]{lowX/Kotko/kut2.eps}
    \includegraphics[height=0.18\textheight]{lowX/Kotko/kut1.eps}
}
%  \end{center}
%\vspace{-0.03\textheight}
\parbox{0.4\textwidth}{
  \caption{
  \small
Azimuthal decorrelations for forward-central dijets (left) and Z0+jet production (right). The theory uncertainty bands come from the scale variation.
  }
}
  \label{fig:fig1}
\end{figure}

\vspace{-0.02\textheight}

\begin{thebibliography}{9}
%\cite{vanHameren:2012if}
\bibitem{vanHameren:2012if} 
  A.~van Hameren, P.~Kotko and K.~Kutak,
  %``Helicity amplitudes for high-energy scattering,''
  JHEP {\bf 1301}, 078 (2013)
%  [arXiv:1211.0961 [hep-ph]].
%\cite{vanHameren:2012uj}
\bibitem{vanHameren:2012uj} 
  A.~van Hameren, P.~Kotko and K.~Kutak,
  %``Multi-gluon helicity amplitudes with one off-shell leg within high energy factorization,''
  JHEP {\bf 1212}, 029 (2012)
%  [arXiv:1207.3332 [hep-ph]].

%\cite{Kotko:2014aba}
\bibitem{Kotko:2014aba} 
  P.~Kotko,
  %``Wilson lines and gauge invariant off-shell amplitudes,''
  JHEP {\bf 1407}, 128 (2014)
%  [arXiv:1403.4824 [hep-ph]].

%\cite{vanHameren:2014ala}
\bibitem{vanHameren:2014ala} 
  A.~van Hameren, P.~Kotko, K.~Kutak and S.~Sapeta,
  %``Small-$x$ dynamics in forward-central dijet decorrelations at the LHC,''
  Phys.\ Lett.\ B {\bf 737}, 335 (2014)
%  [arXiv:1404.6204 [hep-ph]].

%\bibitem{Z0jet}
% A.~van Hameren, P.~Kotko, K.~Kutak,
% {\it in preparation}

%\cite{Kutak:2012rf}
\bibitem{Kutak:2012rf} 
  K.~Kutak and S.~Sapeta,
  %``Gluon saturation in dijet production in p-Pb collisions at Large Hadron Collider,''
  Phys.\ Rev.\ D {\bf 86}, 094043 (2012)
%  [arXiv:1205.5035 [hep-ph]].

%\cite{Kutak:2014wga}
\bibitem{Kutak:2014wga} 
  K.~Kutak,
  %``Hard scale dependent gluon density, saturation and forward-forward dijet production at the LHC,''
  arXiv:1409.3822 [hep-ph].


\end{thebibliography}



==> lowX/LYKASOV_MPI2014_Proc/contentLykasov.tex <==
\title{Transverse momentum dependent gluon density at low $x$}
\author{A.A. Grinyuk$^1$, A. V. Lipatov$^{1,2}$, \underline {G. I. Lykasov$^1$},   
 N. P. Zotov$^2$}
\affiliation{$^1$ Joint Institute for Nuclear Research -
  Dubna 141980, Moscow region, Russia\\
$^2$Skobeltsyn Institute of Nuclear Physics, 
     Lomonosov Moscow State University, 119991, Moscow, Russia \\}

\maketitle

%\section{Unintegrated gluon density}
We present results on the application of the transverse momentum ${\bf k}_T$ dependent
gluon density (TMD) at low $x$, which based on our previous study \cite{GLLZ:2013}.
We match this TMD at low transverse momenta $\mid {\bf k}_T\mid$ and starting scale $Q_0^2 = 1-2$~GeV$^2$
to the exact solution of the BFKL equation outside of the saturation region at large 
$\mid {\bf k}_T\mid$ obtained in \cite{Kovch:2000}. 
%which includes all multiple Pomeron exchanges and allows us to satisfy 
%the unitarization of the DIS cross section and the structure function $F_2$.
Then, to extend this TMD at higher $Q^2$ we use the Catani-Ciafoloni-Fiorani-Marchesini (CCFM) 
evolution equation solution. 
The inclusion of the CCFM evolution results in a large increase of the TMD magnitude. 
The use of new TMD allows us to describe satisfactorily the LHC data on the heavy flavour jet
production and especially the correlation between two $b$-jets produced in $pp$ collisions
at low $x$ and large $\mid {\bf k}_T\mid$. In Fig.1 (left) the rapidity $y$ distribution 
of $b$-jets produced in the $pp$ collision at $\sqrt{s}=$8 TeV is presented. The distribution over the
difference of the azimuthal angles $\Delta\phi$ between similar two $b$-jets is presented in Fig.1(right). 

\begin{figure}[h!]
\rotatebox{270}
%\begin{center}
{\epsfig{file=y_bjet_CMSe_17.12.14.eps,width=0.38\linewidth}}
%\hspace{0.5cm}
\rotatebox{270}
{\epsfig{file=dphi_bb_ATLASb_17.12.14.eps,width=0.38\linewidth}}
%\end{center}
 \caption{The $y$-distribution of $b$-jets produced in the $pp$ collision at $\sqrt{s}=$8 TeV
compared to the CMS data \cite{CMS} (left). The distribution over the difference of the azimuthal angles 
$\Delta\phi$ between similar two $b$-jets compared to the ATLAS data \cite{ATLAS} is presented on the right. 
The solid hystograms correspond to our new TMD, whereas the dashed ones correspond to the TMD 
suggested in \cite{Hannes} (set $A0$). 
}
\label{Fig_ybjet}
\end{figure}

%\section{Summary}
\begin{thebibliography}{9}
\bibitem{GLLZ:2013}
A.A.Grinyuk, A.V.Lipatov, G.I.Lykasov, N.P. Zotov,
Phys.Rev. D{\bf 87} (2013) 074017
\bibitem{Kovch:2000}
Yuri V.Kovchegov, Phys.Rev. D{\bf 61} (2000) 074018.
\bibitem{CMS}
CMS Collaboration, JHEP 1204, 084 (2012); arXiv:1202.4617 [hep-ex]
\bibitem{ATLAS}
ATLAS Collaboration, Eur.Phys.J. C 71, 1846 (2011); arXiv:1109.6833 [hep-ex]
\bibitem{Hannes}
H.~Jung, in Proceedings of 12$^{\rm th}$ International Workshop on Deep-Inelastic 
Scattering and Related Subjects (DIS'2004), Strbske Pleso, Slovakia, April 14-18, 
2004; arXiv:0411287 [hep-ph].
%  Leslie Lamport, \emph{\LaTeX: a document preparation system}. Addison Wesley, Massachusetts, 
%  2nd edition, 1994.
\end{thebibliography}



==> lowX/Martin/content_Martin.tex <==
\title{Report from the LHC Forward Physics Working Group}
\author{Timothy~A.~D.~Martin}
\affiliation{University of Warwick}

\maketitle

\section*{Introduction}
The LHC Forward Physics Working group brings together expertise from the ALICE, ATLAS, CMS, LHCb, LHCf and TOTEM collaboration along with theoretical colleagues involved in research at forward rapidity. A CERN yellow report covering forward physics topics will be released in early 2015 and outline a near term forward physics programme at the LHC. 

\section*{Forward Physics}
Forward physics topics span a range of cross sections from the many milibarn high energy $pp$ diffractive cross section - of importance to cosmic ray air-shower physics among others, to high mass and potentially exotic centrally produced states at small cross sections. The forward physics report covers both hard and soft diffractive, central exclusive and photon induced processes, cosmic ray and heavy ion physics along with processes sensitive to BFKL and saturation effects such as Mueller Navelet jets.

\section*{Forward Detectors}
The established forward proton tagging TOTEM experiment at CMS and ALFA group of ATLAS will operate in 2015 and beyond, continuing their primary remit of the measurement on the total cross section along with novel measurements of forward particle spectra.

Two new forward detector proposals, ATLAS Forward Physics and the CMS-TOTEM Precision Proton Spectrometer\cite{Albrow:1753795} are approved by their respective collaborations. These are designed to have a sensitivity of approximately $3\% < \xi < 12\%$ ($\xi$ is the fractional momentum loss of a driffractivly scattered proton) during standard LHC physics runs with squeezed beams ($\beta^* \sim 0.55$ m). This results in sensitivity to centrally produced systems with mass $M_X > 200$ GeV. The detectors will ultimately perform track reconstruction with 3D pixel detectors and integrate fast timing detectors based on time-to-digital chips or \v{C}erenkov photo-detectors. 10 ps timing resolution will allow for $\sigma_z = 2$ mm central vertex determination in a pile up environment.

Forward scintillator shower counters are being installed upstream and downstream of the ALICE, CMS and LHCb detectors. These will allow for the detection and hence study or veto of low mass proton dissociation in analyses of diffraction, rapidity gaps and central exclusive production. 
\section*{Outlook}
Improved proton tagging capabilities at the LHC will enable new studies of electroweak and QCD physics at high $Q^2$ with sensitivity to potential beyond Standard Model effects.

\begin{thebibliography}{9}
\bibitem{Albrow:1753795}
  CMS-TOTEM~Collaboration, \emph{CMS-TOTEM Precision Proton Spectrometer}. CERN-LHCC-2014-021. TOTEM-TDR-003. CMS-TDR-13, Sep 2014.
\end{thebibliography}

==> lowX/Pleskot/content.tex <==
\title{Studies of azimuthal decorrelation of dijets with a jet veto with ATLAS}
\author{Vojt\v{e}ch Pleskot on behalf of the ATLAS Collaboration}
\affiliation{Institute of Particle and Nuclear Physics\\Charles University in Prague}

\maketitle

\section{Open problems}

\begin{wrapfigure}{R}{0.5\textwidth}
  \centering
  \includegraphics[width=1.0\linewidth]{fig_05c.pdf}
  \caption{Ratio of the first two angular moments $\langle \cos(2\Delta \phi)\rangle / \langle \cos(\pi - \Delta \phi)\rangle$ measured using the inclusive dijet sample. Data are compared to several theoretical predictions.}
  \label{fig:moments_ratio}
\end{wrapfigure}

The next-to-leading-order QCD predictions provide a good description of the inclusive jet cross sections up to the highest reached jet energies~\cite{Aad:2014vwa, Aad:2013tea}.
For certain observables and in some regions of phase space higher-order contributions are important and must be resummed to all orders.
This is the case for dijet events with large rapidity separation of the two jets, $\Delta y$, and/or when a veto is applied on additional jets with $p_\mathrm{T} > Q_0$ produced in the rapidity interval between them; $Q_0$ is called a veto scale.
There are two available resummation approaches, BFKL and DGLAP.
BFKL resums the higher orders in terms of $\ln(1/x)$ while DGLAP does it in terms of $\ln(Q^2)$.
The goal of the presented measurement~\cite{Aad:2014pua} is to test theoretical predictions inspired by the above two approaches.
The DGLAP inspired procedure is implemented in POWHEG+PYTHIA~8 and POWHEG+HERWIG~6.5 Monte Carlo generators.
POWHEG~\cite{Nason:2004rx, Frixione:2007vw, Alioli:2010xd} provides a full NLO dijet calculation.
It is interfaced to PYTHIA~8~\cite{Sjostrand:2007gs} or HERWIG~6.5~\cite{Corcella:2000bw} to provide the parton shower.
The predictions based on BFKL are generated with HEJ~\cite{Andersen:2010ih, Andersen:2011hs} and HEJ+ARIADNE.
HEJ resums leading-logarithms relevant in the Mueller-Navelet limit.
ARIADNE~\cite{Lonnblad:1992tz} provides parton showers based on the colour-dipole cascade model.
The uncertainty of the HEJ+ARIADNE prediction is not available and only the statistical uncertainty is shown.

The described theoretical predictions are tested by ATLAS~\cite{Aad:2008zzm}.
Several observables are measured with the data samples recorded in 2010 and 2011 in proton-proton collisions at $7~\mathrm{TeV}$ centre-of-mass energy.
The 2010 data sample corresponds to $36.1 \pm 1.3~\mathrm{pb}^{-1}$ and was taken under low pile-up conditions.
The veto scale $Q_0$ is set to $20~\mathrm{GeV}$ and jets are accepted in the region $|y| < 4.4$.
The 2011 sample represents $4.5 \pm 0.1~\mathrm{fb}^{-1}$ and it is more affected by pile-up.
In this case $Q_0$ is set to $30~\mathrm{GeV}$ and jets are accepted if $|y| < 2.4$.
An additional requirement of $\Delta y > 1$ was used on the 2011 sample to enhance the events of interest.

Dijet events were selected if the (sub)leading jet $p_\mathrm{T}$ was higher than $60\ (50)~\mathrm{GeV}$.
The events were classified into two categories: the inclusive and gap dijet events.
An event contributes to the gap sample if there is no jet with $p_\mathrm{T} > Q_0$ in the rapidity interval between the two leading-$p_\mathrm{T}$ jets.

An interesting observable is the gap fraction, the ratio of the dijet cross sections measured using the gap and the inclusive samples.
It is exponentially suppressed as a function of $\Delta y$ and $\log(\bar{p}_\mathrm{T}/Q_0)$ where $\bar{p}_\mathrm{T}$ is the average $p_\mathrm{T}$ of the two leading jets.
There is a plateau at high $\Delta y$ and high $\bar{p}_\mathrm{T}$ that can be explained as an effect of steeply falling parton distribution functions and/or as a consequence of colour-singlet exchange processes.
A complementary observable is the mean multiplicity of jets with $p_\mathrm{T} > Q_0$ in the rapidity interval between the two jets.
POWHEG+PYTHIA~8 and HEJ+ARIADNE provide good description of both variables.
The prediction obtained with POWHEG+HERWIG~6.5 does not describe data very well.

The studied observable with the highest discrimination power between different predictions is the ratio of the first two angular moments: $\langle \cos(2\Delta \phi)\rangle / \langle \cos(\pi - \Delta \phi)\rangle$ where $\Delta \phi$ is the azimuthal separation of the two jets.
It is shown in Fig.~\ref{fig:moments_ratio}.
This observable is especially sensitive to the theoretical differences in the regions of low $\bar{p}_\mathrm{T}$ and high $\Delta y$.
HEJ+ARIADNE provides the best description of the ratio for the inclusive dijet sample; its performance is a bit poorer for the gap sample.
The double differential dijet cross section $\mathrm{d}^2 \sigma / \mathrm{d}\Delta \phi \mathrm{d}\Delta y$ is not well described by the predictions using HEJ.
It is quite well described by POWHEG+PYTHIA~8.

\section{Outlook}
No theoretical prediction describes data over the full phase space and for all observables.
Data can constrain parton-shower models because the experimental uncertainty is generally lower than the spread of the different predictions.
Theoretical predictions should be improved to decide about the presence or absence of BFKL effects or colour-singlet exchange processes.

\begin{thebibliography}{9}
\bibitem{Aad:2014vwa}
  ATLAS Collaboration, \emph{Measurement of the inclusive jet cross-section in proton-proton collisions at $\sqrt{s}=7$ TeV using 4.5 fb$^{-1}$ of data with the ATLAS detector}. arXiv:1410.8857, 2014.
%  @article{Aad:2014vwa,
%      author         = "Aad, Georges and others",
%      title          = "{Measurement of the inclusive jet cross-section in
%                        proton-proton collisions at $\sqrt{s}=7$ TeV using 4.5
%                        fb$^{-1}$ of data with the ATLAS detector}",
%      collaboration  = " ATLAS Collaboration",
%      year           = "2014",
%      eprint         = "1410.8857",
%      archivePrefix  = "arXiv",
%      primaryClass   = "hep-ex",
%      reportNumber   = "CERN-PH-EP-2014-155",
%      SLACcitation   = "%%CITATION = ARXIV:1410.8857;%%",
%}

\bibitem{Aad:2013tea}
  ATLAS Collaboration, \emph{Measurement of dijet cross sections in $pp$ collisions at 7 TeV centre-of-mass energy using the ATLAS detector}. JHEP 1405 (2014) 059.
%@article{Aad:2013tea,
%      author         = "Aad, Georges and others",
%      title          = "{Measurement of dijet cross sections in $pp$ collisions
%                        at 7 TeV centre-of-mass energy using the ATLAS detector}",
%      collaboration  = "ATLAS",
%      journal        = "JHEP",
%      volume         = "1405",
%      pages          = "059",
%      doi            = "10.1007/JHEP05(2014)059",
%      year           = "2014",
%      eprint         = "1312.3524",
%      archivePrefix  = "arXiv",
%      primaryClass   = "hep-ex",
%      reportNumber   = "CERN-PH-EP-2013-192",
%      SLACcitation   = "%%CITATION = ARXIV:1312.3524;%%",
%}
  
\bibitem{Aad:2014pua}
  ATLAS Collaboration, \emph{Measurements of jet vetoes and azimuthal decorrelations in dijet events produced in $pp$ collisions at $\sqrt{s}$ = 7 TeV using the ATLAS detector}. Eur.Phys.J. C74 (2014) 11, 3117.
%@article{Aad:2014pua,
%  author         = ``Aad, Georges and others'',
%  title          = ``{Measurements of jet vetoes and azimuthal decorrelations
%                     in dijet events produced in $pp$ collisions at $\sqrt{s}$
%                     = 7 TeV using the ATLAS detector}'',
%  collaboration  = ``ATLAS Collaboration'',
%  journal        = ``Eur.Phys.J.'',
%  number         = ``11'',
%  volume         = ``C74'',
%  pages          = ``3117'',
%  doi            = ``10.1140/epjc/s10052-014-3117-7'',
%  year           = ``2014'',
%  eprint         = ``1407.5756'',
%  archivePrefix  = ``arXiv'',
%  primaryClass   = ``hep-ex'',
%  reportNumber   = ``CERN-PH-EP-2014-132'',
%  SLACcitation   = ``%%CITATION = ARXIV:1407.5756;%%",
%}

\bibitem{Nason:2004rx}
  Nason, Paolo, \emph{A New method for combining NLO QCD with shower Monte Carlo algorithms}. JHEP 0411 (2004) 040.
%@article{Nason:2004rx,
%      author         = "Nason, Paolo",
%      title          = "{A New method for combining NLO QCD with shower Monte
%                        Carlo algorithms}",
%      journal        = "JHEP",
%      volume         = "0411",
%      pages          = "040",
%      doi            = "10.1088/1126-6708/2004/11/040",
%      year           = "2004",
%      eprint         = "hep-ph/0409146",
%      archivePrefix  = "arXiv",
%      primaryClass   = "hep-ph",
%      reportNumber   = "BICOCCA-FT-04-11",
%      SLACcitation   = "%%CITATION = HEP-PH/0409146;%%",
%}

\bibitem{Frixione:2007vw}
  Frixione, Stefano and others, \emph{Matching NLO QCD computations with Parton Shower simulations: the POWHEG method}. JHEP 0711 (2007) 070.
%@article{Frixione:2007vw,
%      author         = "Frixione, Stefano and Nason, Paolo and Oleari, Carlo",
%      title          = "{Matching NLO QCD computations with Parton Shower
%                        simulations: the POWHEG method}",
%      journal        = "JHEP",
%      volume         = "0711",
%      pages          = "070",
%      doi            = "10.1088/1126-6708/2007/11/070",
%      year           = "2007",
%      eprint         = "0709.2092",
%      archivePrefix  = "arXiv",
%      primaryClass   = "hep-ph",
%      reportNumber   = "BICOCCA-FT-07-9, GEF-TH-21-2007",
%      SLACcitation   = "%%CITATION = ARXIV:0709.2092;%%",
%}

\bibitem{Alioli:2010xd}
  Alioli, Simone and others, \emph{A general framework for implementing NLO calculations in shower Monte Carlo programs: the POWHEG BOX}. JHEP 1006 (2010) 043.
%@article{Alioli:2010xd,
%      author         = "Alioli, Simone and Nason, Paolo and Oleari, Carlo and Re,
%                        Emanuele",
%      title          = "{A general framework for implementing NLO calculations in
%                        shower Monte Carlo programs: the POWHEG BOX}",
%      journal        = "JHEP",
%      volume         = "1006",
%      pages          = "043",
%      doi            = "10.1007/JHEP06(2010)043",
%      year           = "2010",
%      eprint         = "1002.2581",
%      archivePrefix  = "arXiv",
%      primaryClass   = "hep-ph",
%      reportNumber   = "DESY-10-018, SFB-CPP-10-22, IPPP-10-11, DCPT-10-22",
%      SLACcitation   = "%%CITATION = ARXIV:1002.2581;%%",
%}

\bibitem{Sjostrand:2007gs}
  Sjostrand, Torbjorn and others, \emph{A Brief Introduction to PYTHIA 8.1}. Comput.Phys.Commun. 178 (2008) 852–867.
%@article{Sjostrand:2007gs,
%      author         = "Sjostrand, Torbjorn and Mrenna, Stephen and Skands, Peter
%                        Z.",
%      title          = "{A Brief Introduction to PYTHIA 8.1}",
%      journal        = "Comput.Phys.Commun.",
%      volume         = "178",
%      pages          = "852-867",
%      doi            = "10.1016/j.cpc.2008.01.036",
%      year           = "2008",
%      eprint         = "0710.3820",
%      archivePrefix  = "arXiv",
%      primaryClass   = "hep-ph",
%      reportNumber   = "CERN-LCGAPP-2007-04, LU-TP-07-28,
%                        FERMILAB-PUB-07-512-CD-T",
%      SLACcitation   = "%%CITATION = ARXIV:0710.3820;%%",
%}

\bibitem{Corcella:2000bw}
  Corcella, Gennaro and others, \emph{HERWIG 6: An Event generator for hadron emission reactions with interfering gluons (including supersymmetric processes)}. JHEP 0101 (2001) 010.
%@article{Corcella:2000bw,
%  author         = ``Corcella, G. and Knowles, I.G. and Marchesini, G. and
%  Moretti, S. and Odagiri, K. and others'',
%  title          = ``{HERWIG 6: An Event generator for hadron emission
%    reactions with interfering gluons (including
%    supersymmetric processes)}'',
%  journal        = ``JHEP'',
%  volume         = ``0101'',
%  pages          = ``010'',
%  doi            = ``10.1088/1126-6708/2001/01/010'',
%  year           = ``2001'',
%  eprint         = ``hep-ph/0011363'',
%  archivePrefix  = ``arXiv'',
%  primaryClass   = ``hep-ph'',
%  reportNumber   = ``CAVENDISH-HEP-99-03, CERN-TH-2000-284, RAL-TR-2000-048'',
%  SLACcitation   = ``%%CITATION = HEP-PH/0011363;%%",
%}

\bibitem{Andersen:2010ih}
  Andersen, Jeppe R. and others, \emph{High Energy Description of Processes with Multiple Hard Jets}. Nucl.Phys.Proc.Suppl. 205-206 (2010) 205–210.
%@article{Andersen:2010ih,
%  author         = ``Andersen, Jeppe R. and Smillie, Jennifer M.'',
%  title          = ``{High Energy Description of Processes with Multiple Hard
%    Jets}'',
%  journal        = ``Nucl.Phys.Proc.Suppl.'',
%  volume         = ``205-206'',
%  pages          = ``205-210'',
%  doi            = ``10.1016/j.nuclphysbps.2010.08.044'',
%  year           = ``2010'',
%  eprint         = ``1007.4449'',
%  archivePrefix  = ``arXiv'',
%  primaryClass   = ``hep-ph'',
%  reportNumber   = ``CERN-PH-TH-2010-167'',
%  SLACcitation   = ``%%CITATION = ARXIV:1007.4449;%%",
%}

\bibitem{Andersen:2011hs}
  Andersen, Jeppe R. and others, \emph{Multiple Jets at the LHC with High Energy Jets}. JHEP 1106 (2011) 010.
%@article{Andersen:2011hs,
%  author         = ``Andersen, Jeppe R. and Smillie, Jennifer M.'',
%  title          = ``{Multiple Jets at the LHC with High Energy Jets}'',
%  journal        = ``JHEP'',
%  volume         = ``1106'',
%  pages          = ``010'',
%  doi            = ``10.1007/JHEP06(2011)010'',
%  year           = ``2011'',
%  eprint         = ``1101.5394'',
%  archivePrefix  = ``arXiv'',
%  primaryClass   = ``hep-ph'',
%  reportNumber   = ``CP3-ORIGINS-2011-02, EDINBURGH-2011-03'',
%  SLACcitation   = ``%%CITATION = ARXIV:1101.5394;%%",
%}

\bibitem{Lonnblad:1992tz}
  Lonnblad, Leif, \emph{ARIADNE version 4: A Program for simulation of QCD cascades implementing the color dipole model}. Comput.Phys.Commun. 71 (1992) 15–31.
%@article{Lonnblad:1992tz,
%  author         = ``Lonnblad, Leif'',
%  title          = ``{ARIADNE version 4: A Program for simulation of QCD
%    cascades implementing the color dipole model}'',
%  journal        = ``Comput.Phys.Commun.'',
%  volume         = ``71'',
%  pages          = ``15-31'',
%  doi            = ``10.1016/0010-4655(92)90068-A'',
%  year           = ``1992'',
%  reportNumber   = ``DESY-92-046'',
%  SLACcitation   = ``%%CITATION = CPHCB,71,15;%%",
%}

\bibitem{Aad:2008zzm}
  ATLAS Collaboration, \emph{The ATLAS Experiment at the CERN Large Hadron Collider}. JINST 3 (2008) S08003.
%@article{Aad:2008zzm,
%      author         = "Aad, G. and others",
%      title          = "{The ATLAS Experiment at the CERN Large Hadron Collider}",
%      collaboration  = "ATLAS",
%      journal        = "JINST",
%      volume         = "3",
%      pages          = "S08003",
%      doi            = "10.1088/1748-0221/3/08/S08003",
%      year           = "2008",
%      SLACcitation   = "%%CITATION = JINST,3,S08003;%%",
%}

\end{thebibliography}



==> lowX/Pleskot/content_Pleskot.tex <==
\title{Studies of azimuthal decorrelation of dijets with a jet veto with ATLAS}
\author{Vojt\v{e}ch Pleskot}
\affiliation{Institute of Particle and Nuclear Physics\\Charles University in Prague}

\maketitle

\section*{Open problems}
The fixed-order next-to-leading QCD predictions provide good description of the inclusive jet cross sections up to the highest reached jet energies~\cite{Aad:2014vwa, Aad:2013tea}.
For certain observables and in some regions of phasespace higher order contributions are important and must be resummed to all orders.
It is the case of dijet events with large rapidity separation of the two jets, $\Delta y$, and/or when a veto is applied on additional jets with $p_\mathrm{T} > Q_0$ produced in the rapidity interval between them.
$Q_0$ is called a veto scale.
There are two available resummation approaches, BFKL and DGLAP.
BFKL resums the higher orders in terms of $\ln(1/x)$.
DGLAP does it in terms of $\ln(Q^2)$.
The goal of the presented measurement~\cite{Aad:2014pua} is to test theoretical predictions inspired by the above two approaches.
The DGLAP inspired predictions are POWHEG+Pythia 8 and POWHEG+Herwig 6.5.
POWHEG~\cite{Nason:2004rx, Frixione:2007vw, Alioli:2010xd} provides full NLO dijet calculation.
It is interfaced to Pythia 8~\cite{Sjostrand:2007gs} or Herwig 6.5~\cite{Corcella:2000bw} to provide the parton shower.
The predictions based on BFKL are HEJ~\cite{Andersen:2010ih, Andersen:2011hs} and HEJ+Ariadne.
HEJ resums leading-logarithms relevant in the Mueller-Navelet limit.
ARIADNE~\cite{Lonnblad:1992tz} provides parton showers based on the colour-dipole cascade model.

Several observables are measured with the data sample recorded by ATLAS in 2010 and 2011 in proton-proton collisions at $7~\mathrm{TeV}$ centre-of-mass energy.
The 2010 data sample corresponds to $36.1 \pm 1.3~\mathrm{pb}^{-1}$ and was taken under low pile-up conditions.
$Q_0$ is set to $20~\mathrm{GeV}$.
Jets with $|y| < 4.4$ are accepted.
The 2011 sample has $4.5 \pm 0.1~\mathrm{fb}^{-1}$ and it is more affected by pile-up.
$Q_0$ is set to $30~\mathrm{GeV}$ and jets are accepted if $|y| < 2.4$.
An additional requirement of $\Delta y > 1$ was used on the 2011 sample to enhance the events of interest.

Dijet events were selected if the (sub)leading jet $p_\mathrm{T}$ was higher than $60\ (50)~\mathrm{GeV}$.
The events were classified into two categories: the inclusive and gap dijet events.
An event contributes to the gap sample if there is no jet with $p_\mathrm{T} > Q_0$ in the rapidity interval between the two leading-$p_\mathrm{T}$ jets.

An interesting observable is the gap fraction, the ratio of the dijet cross sections measured on the gap and the inclusive samples.
It is exponentially suppressed as a function of $\Delta y$ and $\log(\bar{p}_\mathrm{T}/Q_0)$ where $\bar{p}_\mathrm{T}$ is the average $p_\mathrm{T}$ of the two leading jets.
There is a plateau at high $\Delta y$ and high $\bar{p}_\mathrm{T}$ that can be explained as an effect of steeply falling parton distribution functions and/or as a consequence of colour-singlet exchange processes.
Complementary observable is the mean multiplicity of jets with $p_\mathrm{T} > Q_0$ in the rapidity interval between the two jets.
POWHEG+Pythia 8 and HEJ+ARIADNE provide good description of both variables.
Herwig 6.5 worsens the POWHEG prediction with respect to Pythia 8.

The studied observable with the highest discrimination power between different predictions is the ratio of the first two angular moments: $\langle \cos(2\Delta \phi)\rangle / \langle \cos(\pi - \Delta \phi)\rangle$ where $\Delta \phi$ is the azimuthal separation of the two jets.
This observable is especially sensitive to the theoretical differences in the regions of low $\bar{p}_\mathrm{T}$ and high $\Delta y$.
HEJ+ARIADNE provides best description of the ratio on the inclusive dijet sample; its performance is a bit worsened on the gap sample.

The double differential dijet cross section $\mathrm{d}^2 \sigma / \mathrm{d}\Delta \phi \mathrm{d}\Delta y$ is not well described by the predictions using HEJ.
It is quite well described by POWHEG+Pythia 8.

\section*{Outlook}
No theoretical prediction describes data on the full phasespace and for all observables.
Data can constrain parton-shower models because the experimental uncertainty is generally lower than the spread of the different predictions.
Theoretical predictions should be improved to decide about the presence or absence of BFKL effects or colour-singlet exchange processes.

\begin{thebibliography}{9}
\bibitem{Aad:2014vwa}
  Aad, Georges and others, \emph{Measurement of the inclusive jet cross-section in proton-proton collisions at $\sqrt{s}=7$ TeV using 4.5 fb$^{-1}$ of data with the ATLAS detector}. arXiv:1410.8857, 2014.
%  @article{Aad:2014vwa,
%      author         = "Aad, Georges and others",
%      title          = "{Measurement of the inclusive jet cross-section in
%                        proton-proton collisions at $\sqrt{s}=7$ TeV using 4.5
%                        fb$^{-1}$ of data with the ATLAS detector}",
%      collaboration  = " ATLAS Collaboration",
%      year           = "2014",
%      eprint         = "1410.8857",
%      archivePrefix  = "arXiv",
%      primaryClass   = "hep-ex",
%      reportNumber   = "CERN-PH-EP-2014-155",
%      SLACcitation   = "%%CITATION = ARXIV:1410.8857;%%",
%}

\bibitem{Aad:2013tea}
  Aad, Georges and others, \emph{Measurement of dijet cross sections in $pp$ collisions at 7 TeV centre-of-mass energy using the ATLAS detector}. JHEP 1405 (2014) 059.
%@article{Aad:2013tea,
%      author         = "Aad, Georges and others",
%      title          = "{Measurement of dijet cross sections in $pp$ collisions
%                        at 7 TeV centre-of-mass energy using the ATLAS detector}",
%      collaboration  = "ATLAS",
%      journal        = "JHEP",
%      volume         = "1405",
%      pages          = "059",
%      doi            = "10.1007/JHEP05(2014)059",
%      year           = "2014",
%      eprint         = "1312.3524",
%      archivePrefix  = "arXiv",
%      primaryClass   = "hep-ex",
%      reportNumber   = "CERN-PH-EP-2013-192",
%      SLACcitation   = "%%CITATION = ARXIV:1312.3524;%%",
%}
  
\bibitem{Aad:2014pua}
  Aad, Georges and others, \emph{Measurements of jet vetoes and azimuthal decorrelations in dijet events produced in $pp$ collisions at $\sqrt{s}$ = 7 TeV using the ATLAS detector}. Eur.Phys.J. C74 (2014) 11, 3117.
%@article{Aad:2014pua,
%  author         = ``Aad, Georges and others'',
%  title          = ``{Measurements of jet vetoes and azimuthal decorrelations
%                     in dijet events produced in $pp$ collisions at $\sqrt{s}$
%                     = 7 TeV using the ATLAS detector}'',
%  collaboration  = ``ATLAS Collaboration'',
%  journal        = ``Eur.Phys.J.'',
%  number         = ``11'',
%  volume         = ``C74'',
%  pages          = ``3117'',
%  doi            = ``10.1140/epjc/s10052-014-3117-7'',
%  year           = ``2014'',
%  eprint         = ``1407.5756'',
%  archivePrefix  = ``arXiv'',
%  primaryClass   = ``hep-ex'',
%  reportNumber   = ``CERN-PH-EP-2014-132'',
%  SLACcitation   = ``%%CITATION = ARXIV:1407.5756;%%",
%}

\bibitem{Nason:2004rx}
  Nason, Paolo, \emph{A New method for combining NLO QCD with shower Monte Carlo algorithms}. JHEP 0411 (2004) 040.
%@article{Nason:2004rx,
%      author         = "Nason, Paolo",
%      title          = "{A New method for combining NLO QCD with shower Monte
%                        Carlo algorithms}",
%      journal        = "JHEP",
%      volume         = "0411",
%      pages          = "040",
%      doi            = "10.1088/1126-6708/2004/11/040",
%      year           = "2004",
%      eprint         = "hep-ph/0409146",
%      archivePrefix  = "arXiv",
%      primaryClass   = "hep-ph",
%      reportNumber   = "BICOCCA-FT-04-11",
%      SLACcitation   = "%%CITATION = HEP-PH/0409146;%%",
%}

\bibitem{Frixione:2007vw}
  Frixione, Stefano and others, \emph{Matching NLO QCD computations with Parton Shower simulations: the POWHEG method}. JHEP 0711 (2007) 070.
%@article{Frixione:2007vw,
%      author         = "Frixione, Stefano and Nason, Paolo and Oleari, Carlo",
%      title          = "{Matching NLO QCD computations with Parton Shower
%                        simulations: the POWHEG method}",
%      journal        = "JHEP",
%      volume         = "0711",
%      pages          = "070",
%      doi            = "10.1088/1126-6708/2007/11/070",
%      year           = "2007",
%      eprint         = "0709.2092",
%      archivePrefix  = "arXiv",
%      primaryClass   = "hep-ph",
%      reportNumber   = "BICOCCA-FT-07-9, GEF-TH-21-2007",
%      SLACcitation   = "%%CITATION = ARXIV:0709.2092;%%",
%}

\bibitem{Alioli:2010xd}
  Alioli, Simone and others, \emph{A general framework for implementing NLO calculations in shower Monte Carlo programs: the POWHEG BOX}. JHEP 1006 (2010) 043.
%@article{Alioli:2010xd,
%      author         = "Alioli, Simone and Nason, Paolo and Oleari, Carlo and Re,
%                        Emanuele",
%      title          = "{A general framework for implementing NLO calculations in
%                        shower Monte Carlo programs: the POWHEG BOX}",
%      journal        = "JHEP",
%      volume         = "1006",
%      pages          = "043",
%      doi            = "10.1007/JHEP06(2010)043",
%      year           = "2010",
%      eprint         = "1002.2581",
%      archivePrefix  = "arXiv",
%      primaryClass   = "hep-ph",
%      reportNumber   = "DESY-10-018, SFB-CPP-10-22, IPPP-10-11, DCPT-10-22",
%      SLACcitation   = "%%CITATION = ARXIV:1002.2581;%%",
%}

\bibitem{Sjostrand:2007gs}
  Sjostrand, Torbjorn and others, \emph{A Brief Introduction to PYTHIA 8.1}. Comput.Phys.Commun. 178 (2008) 852–867.
%@article{Sjostrand:2007gs,
%      author         = "Sjostrand, Torbjorn and Mrenna, Stephen and Skands, Peter
%                        Z.",
%      title          = "{A Brief Introduction to PYTHIA 8.1}",
%      journal        = "Comput.Phys.Commun.",
%      volume         = "178",
%      pages          = "852-867",
%      doi            = "10.1016/j.cpc.2008.01.036",
%      year           = "2008",
%      eprint         = "0710.3820",
%      archivePrefix  = "arXiv",
%      primaryClass   = "hep-ph",
%      reportNumber   = "CERN-LCGAPP-2007-04, LU-TP-07-28,
%                        FERMILAB-PUB-07-512-CD-T",
%      SLACcitation   = "%%CITATION = ARXIV:0710.3820;%%",
%}

\bibitem{Corcella:2000bw}
  Corcella, Gennaro and others, \emph{HERWIG 6: An Event generator for hadron emission reactions with interfering gluons (including supersymmetric processes)}. JHEP 0101 (2001) 010.
%@article{Corcella:2000bw,
%  author         = ``Corcella, G. and Knowles, I.G. and Marchesini, G. and
%  Moretti, S. and Odagiri, K. and others'',
%  title          = ``{HERWIG 6: An Event generator for hadron emission
%    reactions with interfering gluons (including
%    supersymmetric processes)}'',
%  journal        = ``JHEP'',
%  volume         = ``0101'',
%  pages          = ``010'',
%  doi            = ``10.1088/1126-6708/2001/01/010'',
%  year           = ``2001'',
%  eprint         = ``hep-ph/0011363'',
%  archivePrefix  = ``arXiv'',
%  primaryClass   = ``hep-ph'',
%  reportNumber   = ``CAVENDISH-HEP-99-03, CERN-TH-2000-284, RAL-TR-2000-048'',
%  SLACcitation   = ``%%CITATION = HEP-PH/0011363;%%",
%}

\bibitem{Andersen:2010ih}
  Andersen, Jeppe R. and others, \emph{High Energy Description of Processes with Multiple Hard Jets}. Nucl.Phys.Proc.Suppl. 205-206 (2010) 205–210.
%@article{Andersen:2010ih,
%  author         = ``Andersen, Jeppe R. and Smillie, Jennifer M.'',
%  title          = ``{High Energy Description of Processes with Multiple Hard
%    Jets}'',
%  journal        = ``Nucl.Phys.Proc.Suppl.'',
%  volume         = ``205-206'',
%  pages          = ``205-210'',
%  doi            = ``10.1016/j.nuclphysbps.2010.08.044'',
%  year           = ``2010'',
%  eprint         = ``1007.4449'',
%  archivePrefix  = ``arXiv'',
%  primaryClass   = ``hep-ph'',
%  reportNumber   = ``CERN-PH-TH-2010-167'',
%  SLACcitation   = ``%%CITATION = ARXIV:1007.4449;%%",
%}

\bibitem{Andersen:2011hs}
  Andersen, Jeppe R. and others, \emph{Multiple Jets at the LHC with High Energy Jets}. JHEP 1106 (2011) 010.
%@article{Andersen:2011hs,
%  author         = ``Andersen, Jeppe R. and Smillie, Jennifer M.'',
%  title          = ``{Multiple Jets at the LHC with High Energy Jets}'',
%  journal        = ``JHEP'',
%  volume         = ``1106'',
%  pages          = ``010'',
%  doi            = ``10.1007/JHEP06(2011)010'',
%  year           = ``2011'',
%  eprint         = ``1101.5394'',
%  archivePrefix  = ``arXiv'',
%  primaryClass   = ``hep-ph'',
%  reportNumber   = ``CP3-ORIGINS-2011-02, EDINBURGH-2011-03'',
%  SLACcitation   = ``%%CITATION = ARXIV:1101.5394;%%",
%}

\bibitem{Lonnblad:1992tz}
  Lonnblad, Leif, \emph{ARIADNE version 4: A Program for simulation of QCD cascades implementing the color dipole model}. Comput.Phys.Commun. 71 (1992) 15–31.
%@article{Lonnblad:1992tz,
%  author         = ``Lonnblad, Leif'',
%  title          = ``{ARIADNE version 4: A Program for simulation of QCD
%    cascades implementing the color dipole model}'',
%  journal        = ``Comput.Phys.Commun.'',
%  volume         = ``71'',
%  pages          = ``15-31'',
%  doi            = ``10.1016/0010-4655(92)90068-A'',
%  year           = ``1992'',
%  reportNumber   = ``DESY-92-046'',
%  SLACcitation   = ``%%CITATION = CPHCB,71,15;%%",
%}
\end{thebibliography}




==> lowX/Stebel/content_Stebel.tex <==
\title{Forward Drell-Yan cross-section beyond single scattering approximation}
\author{Tomasz Stebel, Leszek Motyka and Mariusz Sadzikowski}
\affiliation{M. Smoluchowski Institute of Physics, Jagiellonian University,\\
S. Lojasiewicz str.\ 11, 30-348 Krakow, Poland}

\maketitle

\section*{Open problems}

Forward Drell-Yan (DY) process at the LHC is a sensitive tool for investigating QCD effects at small Bjorken-$x$ ($x \simeq 10^{-6}$ and moderate energy scales). The LHCb experiment is expected to measure DY lepton-antilepton mass $M$ of about 2.5 GeV. In this kinematical domain higher twists of Operator Product Expansion (OPE) may introduce sizeable corrections to the leading twist approximation. 

In the standard description of the DY process an angular distribution of lepton pairs is described by four structure functions $W_L, \ W_T,\ W_{TT}, \ W_{LT}$. Higher twist analysis of forward the DY is based on the OPE of these functions. The power suppression in hard scale of higher twists is compensated by small-$x$ growing of matrix elements. In addition, combination $W_L-2 W_{TT}$ vanishes at leading twist-2 up to next-to-next-to-leading order of QCD corrections (this is known as the Lam-Tung relation). This makes from $W_L-2 W_{TT}$ a very promising observable for future experimental searches of higher twists. 

In the high energy limit in QCD, relevant for forward Drell-Yan process at the LHC, the scattering amplitudes may be efficiently computed using the $k_T$-factorization framework and the color dipole picture. In our approach we expressed structure functions $W_i$ as a Mellin convolutions $W_{i} \sim \int_C ds \ \tilde{\sigma} (-s) \hat{\Phi}_{i}(s)$ where $\tilde{\sigma}$ and $\hat{\Phi}_{i}$ are Mellin transforms of the dipole cross-section and an impact factor, respectively. Impact factors are calculated from perturbative QCD at the leading order and hence are universal (do not depend on the model) and their form is one of the main results of our calculations. On the other hand the cross-section $\tilde{\sigma}$ needs to be modeled. 

As a first step towards understanding the higher twist structure of the forward DY scattering we consider the simplest case of the eikonal dipole cross-section used in the Golec-Biernat--W\"{u}sthoff (GBW) approach. Using this cross-section we perform an explicit analytic twist decomposition of the forward DY structure functions. The GBW model provides an efficient description of the small-$x$ data. One should note however that up to now the data probe the proton structure efficiently only at the leading twist. Hence, current theoretical predictions of higher twist effects are uncertain. 

\section*{Outlook}

Since our results for the twist expansion of the forward DY structure functions are model dependent one needs also to provide dedicated predictions for the LHC within other reasonable schemes. Balitsky-Fadin-Kuraev-Lipatov (BFKL) and Balitsky-Kovchegov (BK) approximations obtained using small-$x$ resummations are the most promising ones. The next step in our program of theoretical analysis of the LHC higher twist will be a data oriented study containing numerical predictions for the higher twist corrections to forward DY within different models (such as GBW, BFKL, BK). 

For results, more detailed description and references see \cite{MSS}.



\begin{thebibliography}{9}
\bibitem{MSS}
L.~Motyka, M.~Sadzikowski and T.~Stebel, arXiv:1412.4675 [hep-ph].

\end{thebibliography}



==> lowX/content_Summary.tex <==
\title{Outlook on MPI and small-$x$ and diffraction}
\author{O. Kepka, P. van Mechelen, W. Sch\"afer, A. Sta\'sto}
\affiliation{}

\maketitle
%\section{Diffraction and small $x$}

In models of multiparticle production at high energies based on Pomeron exchanges,
multiple interactions and diffractive processes are part and parcel of the formalism.
While the former are related to diagrams with multiple cut Pomerons, diffractive processes,
or rapidity gap fluctuations, are described by the exchange of uncut Pomerons.

The perturbative QCD gluon ladder can be regarded as representing a cut Pomeron. 
In multipomeron exchange models, cut and uncut Pomerons enter with such combinatorial weights
(given by the AGK cutting rules), that the single particle inclusive cross section at central rapidities is just 
given by the contribution of a single cut Pomeron. All effects of multiple 
interactions/rescatterings cancel in this observable.

A similar cancellation of spectator interactions is 
also part of the standard hard scattering factorization theorems for inclusive hard processes. 
At small-$x$, there is not yet any coherent formalism available 
that would allow us to go to less inclusive observables, like for example multiple hard processes,
hard processes as a function of the underlying event multiplicity etc.

The search for novel QCD dynamics at low $x$ is centered around effects related to 
the transverse momentum of partons entering the hard scattering.  
Various observables have been proposed, such as the azimuthal balance of jets, 
the likelihood to produce additional jets within or outside the rapidity range covered by the 
leading dijet system, etc.  
Investigations using the LHC run 1 data have shown an intricate interplay between low $x$ effects and 
multiple partonic interactions.  
This points to the need for a unified theoretical approach including low $x$, 
transverse momentum dependent parton densities and multiple partonic interactions. 

Multiple interactions are also important for the understanding of diffractive events: here
the interaction of spectator partons in a diffractive process would fill the rapidity gaps.
One needs to know the probability that no additional interaction occurs -- the so-called
gap survival probability.
Lepton pair production with rapidity gaps is particularly interesting in this regard. 
Here the lepton-pair production via photon-photon fusion at ``Born-level'' is calculable from QED and 
proton structure functions. A deviation of the measurement from such a calculation may   
determine the probability that protons are transmitted through the interaction region intact. 
Such an analysis appears to be possible in the upcoming LHC run.

Another way to investigate the relation between rapidity gap survival and multiple partonic interactions is to measure 
the fraction of events with a (forward) rapidity gap w.r.t. inclusive events, as a function of (central) 
jet transverse momentum.  This is reminiscent of the study of the underlying event by looking at the activity 
transverse to a leading particle or jet as function of the particle or jet $p_{\rm T}$.  
For a fixed gap size, the fraction of events with a gap will decrease as function of $p_{\rm T}$ and 
it would be interesting to investigate whether phenomenological models for multiple 
partonic interaction can describe this behaviour well. 

The ATLAS and CMS collaborations will upgrade their detectors with forward proton taggers during the LHC run 2.  
Several upgrade stages are foreseen.  This will allow to tag diffractive events and measure the proton kinematics, 
even in the presence of pile-up and is thus a very attractive development 
for the study of hard diffractive processes with a small cross section. 

==> lowX/content_goerlich.tex <==
\title{Dijet production at HERA and tests of QCD factorisation}
\author{Lidia Goerlich\\on behalf of the H1 and ZEUS Collaborations }
\affiliation{Institute of Nuclear Physics\\Polish Academy of Sciences}

\maketitle

%\section{Open problems}
\section{Exclusive dijet production in diffractive DIS}

The exclusive production of dijets in diffractive deep inelastic lepton-proton 
scattering has been measured by the ZEUS Collaboration 
for the first time at HERA \cite{ZEUS}.
Jets have been reconstructed in the virtual 
photon-Pomeron  centre-of-mass system frame using the exclusive 
$k_T$ algorithm. The cross section for the exclusive production of 
dijets is given as a function of the azimuthal angle $\phi$ between the plane defined
by exchanged photon and dijet system and the plane defined by the
incoming and scattered lepton momenta in the $\gamma^*$-Pomeron rest frame. 
The shape of the $\phi$ distribution is sensitive to the production mechanism
of diffractive exclusive dijets. The data favour fully perturbative calculations 
of the two-gluon exchange model over boson-gluon fusion mechanism, in which a partonic
structure of the Pomeron is assumed.

\section{Tests of QCD factorisation}

In the framework of  QCD collinear factorisation the cross section for 
the diffractive DIS process factorises into universal diffractive 
parton distribution functions (DPDFs) and hard subrocess cross sections calculable 
within the perturbative approach. The universality of these DPDFs was sucessfully 
tested for hard diffractive DIS production.
% of dijet and charm.
However, the factorisation breaking was observed for hard processes in diffractive
hadron-hadron scattering where the predictions based on HERA DPDFs overestimate
the data, at Tevatron by about one order of magnitude. The factorisation breaking 
is usually explained 
in terms of multiple scattering effects, which occur in the presence
of beam remnants and lead to the destruction of the rapidity gap associated 
with the diffractive process. Rapidity gap survival effects can be investigated 
at HERA in hard diffractive dijet photoproduction. 

Diffractive dijet cross sections in photoproduction and in DIS
with a leading proton detected in the very forward proton spectrometer (VFPS) 
have been measured by H1 \cite{H1_01}. 
DIS measurements are complemented by measurements of dijet production with an
associated large rapidity gap (LRG) \cite{H1_02}. 
The cross sections for the dijet production  in diffractive DIS with VFPS  
and with LRG are found
to be well described by the NLO QCD predictions using the H12006 Fit-B DPDF set. 
These results confirm the validity of QCD factorisation in 
hard diffractive DIS.
  
Using the VFPS data the double ratio of measured to predicted cross sections in 
photoproduction to the corresponding ratio in DIS has been determined and 
its value is equal to $0.55 \pm 0.10(\rm data)+0.02(\rm theor.)$, with no significant
kinematic dependence. This result is consistent with previous H1 measurements based on the LRG method
and indicates that QCD factorisation may be broken in diffractive dijet photoproduction.
However, ZEUS does not observe factorisation breaking in diffractive photoproduced jets.

\begin{thebibliography}{9}
\bibitem{ZEUS}
  M. Guzik, Proceedings PoS (DIS2014) 070. 
%  M. Guzik (\emph{on behalf of the ZEUS Collaboration}), Proceedings PoS (DIS2014) 070. 
\bibitem{H1_01}
  R. Zlebcik, Proceedings PoS (DIS2014) 072. 
\bibitem{H1_02}
 V. Andreev et al. [H1 Collaboration], DESY 14-200. 
%\bibitem{lamport03}
 % Leslie Lamport, \emph{\LaTeX: a document preparation system}. Addison Wesley, Massachusetts, 2nd edition, 1994.

\end{thebibliography}


